A Survey on the Integration of NAND Flash Storage in the Design of File Systems and the Host Storage Software Stack

With the ever-increasing amount of data generate in the world, estimated to reach over 200 Zettabytes by 2025, pressure on efficient data storage systems is intensifying. The shift from HDD to flash-based SSD provides one of the most fundamental shifts in storage technology, increasing performance capabilities significantly. However, flash storage comes with different characteristics than prior HDD storage technology. Therefore, storage software was unsuitable for leveraging the capabilities of flash storage. As a result, a plethora of storage applications have been design to better integrate with flash storage and align with flash characteristics. In this literature study we evaluate the effect the introduction of flash storage has had on the design of file systems, which providing one of the most essential mechanisms for managing persistent storage. We analyze the mechanisms for effectively managing flash storage, managing overheads of introduced design requirements, and leverage the capabilities of flash storage. Numerous methods have been adopted in file systems, however prominently revolve around similar design decisions, adhering to the flash hardware constrains, and limiting software intervention. Future design of storage software remains prominent with the constant growth in flash-based storage devices and interfaces, providing an increasing possibility to enhance flash integration in the host storage software stack.

==> background.tex <==
\section{Background}\label{sec:background}
Flash storage has become ubiquitous with its increased performance capabilities over conventional storage, such as \as{hdd}, and with its decreasing cost it is increasing in adoption~\cite{daim2008forecasting,2008-Lee-Flash_in_enterprise_db}. This background section explains the high level concepts of how flash storage is constructed (\cref{sec:bg_flash_storage}), how performant storage devices are built with flash storage (\cref{sec:bg_flash_ssds}), and how these devices are managed to be integrated into host systems (\cref{sec:bg_ssd_internals,sec:flash_integration_separation,sec:ssd_host_interfaces}).

\subsection{Flash Storage}\label{sec:bg_flash_storage}
Flash storage is based on flash cells providing the persistent storage capabilities through programming of the cell and erasing to clear its content. These are constructed with a floating gate, which can hold an electrical charge, and a control gate, inside a complementary metal-oxide semiconductor (CMOS) transistor~\cite{parat2015floating}. \cref{fig:flash_cell} shows an overview of the organization of the floating and control gate in a flash cell. Oxide layers are used around the floating gate to provide insulation, resulting in trapping of electrons in the floating gate. Charging the floating gate with an electrical charge results in it dampening the electric field of the control gate, which requires a larger voltage to be applied to the control gate in order to become conductive~\cite{pavan1997flash}. Therefore, if the control gate does not become conductive at a certain voltage threshold, it means the floating gate is charged, which represents a logical 0. When the floating gate is not charged, the control gate becomes conductive at a lower voltage, indicating a logical 1. The current in the flash cell flows between the source and drain terminals. A single flash cell can therefore represent a single bit, with a logical 0 or 1. The current flowing between the terminals is managed by programming and erasing the floating gate. The charge of the floating gate after an erase operation is equivalent to a logical 1, and programming the flash cell can modify the charge to logical 0~\cite{jagmohan2010write}. A subsequent erase operation brings the charge back to a logical 1. 

\begin{figure}[!t]
    \center
    \includegraphics[width=0.3\textwidth]{figs/flash_cell.pdf}
    \label{fig:flash_cell}
    \caption{Overview of the construction of a flash cell.}
\end{figure}

Flash that stores a single bit value in a flash cell is called \af{slc}. The storage capacity of a flash cell can be increased by increasing the number of layers, by modifying the variability in the charging state of the floating. In order for a floating gate to represent two bits, its voltage must be able to represent 4 distinct states (as it is two bits $2^2=4$), based on which its logical value can be interpreted. Therefore, the voltage threshold is divided into regions to represent the values, such as no charge, low charge, medium charge, and a high charge. Available flash cell levels are \af{mlc}, \af{tlc}, \af{qlc}, and \af{plc}~\cite{2020-Ma-Flash_Memory_Bit_Errors}, which respectively increase the number of bits stored per flash cell by one. However, increasing number of cell levels results in slower access time~\cite{arpaci2018operating}, lower flash cell lifetime~\cite{mohan2010learned}, and introduced noise between cells due to the voltage differences, which in turn leads to increased bit errors~\cite{2015TaranalliFlashError,2020-Ma-Flash_Memory_Bit_Errors}. As the flash cell is programmed over time, the oxide layers erode, causing the flash cell to no longer be usable. For \as{slc} this value is typically 100K and decreases to 10K or less for \as{mlc}~\cite{2016-Schroeder-Flash_Reliability}.

There are various ways of packing flash cells in full storage devices. Firstly, organization of flash cells representing NOR gates. In NOR flash each individual flash cell is connected directly to the source line and the bit line, responsible for providing the connection to the source terminal of the cell and the drain terminal, respectively. Over the source terminal the charge for programming of reading the flash cell is applied, where the source drain of the flash cells is connected to the source line. The bit line is connected to the drain terminal in order to read the voltage that is applied from the source terminal. The connection to the source and bit line for each flash cell in NOR flash allows it to be byte addressable, however incurs a high erase latency, requires more space, and is therefore also more costly. Secondly, organization that depicts NAND gates, where several (typically 8) flash cells are connected in series from the source line to the bit line. This allows for a significantly higher density of flash cells to be packed, however makes the flash no longer byte addressable, but instead needs to be written and erased in a larger unit, referred to as a \textit{flash page}, which are typically 16KiB in modern flash storage. As NOR flash provides byte addressability and lower access latency, it is suitable for small persistent storage such as for system BIOS~\cite{2012-Lai-NOR_BIOS}, however for mass data storage NOR flash becomes costly compared to NAND flash. In addition to a higher cost, NOR flash has significantly higher erase latency than NAND flash~\cite{toshiba2006vs}, making it undesirable for large data storage.

NAND can also be stacked vertically in what is called 3-D NAND~\cite{micheloni2017array}, for a higher density, however such specifics are out of the scope of this survey. For this survey only a basic understanding of flash cells is required, as was explained. For more detailed information on functionality of flash cells, reports such as~\cite{bez2003introduction} and~\cite{compagnoni2017reviewing} can be consulted. We only focus on NAND based flash storage due to its increased benefits and adoption for large scale data storage systems, on which the file systems we evaluate are built.

\subsection{Flash SSDs}\label{sec:bg_flash_ssds}
Flash cells are grouped into \textit{pages}, depicting the unit of access (typically 16KiB). A flash page additional has a small extra space, called the \af{oob} area, which is utilized for \af{ecc} and small metadata. As the operation for erasing of a flash page is costly, multiple pages are grouped into a \textit{block} (typically several 256MiB), which is the unit of erase. Increasing the erase unit from individual pages to a block helps amortize the erase overheads. Pages within a block have to be written sequentially and prior to a page being overwritten, the entire block needs to be erased. A number of blocks are then grouped into a \textit{plane}, of which multiple planes are combined into a \textit{die}~\footnote{\textit{Dies} are also referred to as \textit{chips}, we use the terms interchangeably and mean the same entity.}. Lastly, numerous dies are combined into a single flash package. \cref{fig:ssd_architecture} shows a visual representation of a flash-based SSD architecture. The flash storage is organized a number of \textit{flash packages}.

\input{figs/ssd_architecture.tex}

In order to build fast storage devices, multiple flash packages are packed together into a \as{ssd}. While an \as{ssd} can be constructed with any solid state technology such as Optane~\cite{2019-Wu-Unwritten_Contract_Optane,2020-Yang-Optane_3DXpoint}, we focus purely on NAND flash based SSDs. The SSD contains a controller, which is responsible for processing requests, managing data buffers, and contains the NAND flash controller that manages the flash packages. An additional \af{ram} buffer, most commonly in the form of \af{dram}, is present on the device for maintaining address mappings (discussed in \cref{sec:bg_ssd_internals}). Lastly, an \as{ssd} contain the host interface that provides the means to connect to the storage to the host system over connection interfaces such as \af{sata} and \af{pcie}, and defining standards such as \af{ahci} and \af{nvme}~\cite{landsman2013ahci} (discussed in \cref{sec:ssd_host_interfaces}). Depending on the chosen connection protocol for the storage media, throughput and achievable performance is limited by it, where the newest \as{pcie} protocol achieves the highest throughput and lower latency compared to SATA~\cite{2013-Eshghi-SSD}.

However, based on a study on a Samsung \as{ssd}, the bandwidth of NAND flash \af{io} buses, connecting the flash to the flash controller, is limited to 32MB/s because of physical restrictions, and 40MB/s with interleaving in dies~\cite{2008-Agrawal-Design-Tradeoff-SSD}. A write operation to flash storage firstly writes the data to a data register, from which the data in the register is then programmed into the flash page. Because the programming operation takes longer than loading of data, these operations can be interleaved, such that while a page is being programmed, data of another write operation is loaded~\cite{kim2011parameter}. This avoids stalling whenever a page programming finishes and data needs to be loaded again. Interleaving is similar to the concept of CPU pipelining~\cite{tanenbaum2016structured-pipelinining}. In order to increase performance, parallelism is utilized on the different flash entities in the \as{ssd}~\cite{chen2011essential}. Depending on the hardware configurations, the different types of parallelism are referred to as \textit{channel-level parallelism}, where requests are distributed individually across the flash channels, \textit{package-level parallelism} where flash packages on the same channel are accessed in parallel, \textit{chip-level parallelism} where flash packages with multiple dies access the dies in parallel, and \textit{plane-level parallelism} where the same operation can be run on multiple planes, in the same die, in parallel. 

There are several additional performance optimizations for accessing flash storage. Other than accessing a flash entity in parallel and interleaving, flash packages can be accessed synchronously with a single request queue through \textit{ganging}~\cite{2008-Agrawal-Design-Tradeoff-SSD}. Flash packages within a gang share the same control bus from the flash controller, however can utilize different data buses, thus allowing a single command request queue with multiple data buses to provide the resulting data. Therefore, requests that require data from multiple pages can be split among a gang from a single request queue, and provide the data on different buses, avoiding the bottleneck of a single data bus. With the increased parallelism on a flash \as{ssd}, the process of accessing multiple blocks simultaneously across different chips and planes is referred to as \textit{clustered blocks}~\cite{kim2011parameter}. Accessing flash storage in units of clustered blocks allows exploiting a higher level of the flash performance.

\subsection{SSD Internals}\label{sec:bg_ssd_internals}
With the complexity of flash-based storage devices, an \as{ssd} ships with firmware, containing the \as{ftl}, that hides the flash management idiosyncrasies from the host system, exposing a conventional sector/page addressable storage device (just as a \as{hdd}). The \as{ftl} is responsible for aligning \as{io}s to the device constraints, such that pages are written sequentially and a block is erased prior to a page being overwritten. For achieving this, the \as{ftl} maintains a mapping of pages and their state, such that it can identify which pages in a block are valid and which have been overwritten. Different implementations of an \as{ftl} can utilize different mapping levels, such as block mappings or custom units. For a detailed explanation of FTL mapping algorithms consult \cite{chung2009FTL_survey} and \cite{2009-Gupta-DFTL}.

A naive FTL design is to maintain a fully associative mapping of each \af{lba} to \af{pba}~\cite{2009-Gupta-DFTL}, referred to as \af{l2p} mapping, and inversely \af{p2l} mapping. These mappings are maintained in a \textit{mapping table}, which is kept in the \as{ram} of the flash device for faster accesses. For consistency the mapping table is also maintained in the persistent flash storage, where on startup time of the devices the mapping table is reconstructed in the device \as{ram}~\cite{chen2009understanding,2008-Agrawal-Design-Tradeoff-SSD}. With this, the SSD can provide seemingly in-place updates by simply writing data to a free page and invalidating the overwritten data. Over time this generates an increasing number of invalid pages within blocks, requiring to run \af{gc} to read out still valid pages in the block and move these pages to a free block on the SSD, followed by erasing the original block. An additional requirement for performing \as{gc} is the need for extra space, such that the \as{ftl} can move valid pages to a free space before erasing the block. This extra space is called the \af{ops}, and typically ranges between 10-28\% of the device capacity. Due to the limited life of flash cells~\cite{mohan2010learned,2016-Schroeder-Flash_Reliability}, the FTL has to additionally ensure even wear across the device, such that no particular region of the flash storage is burnt out quicker than other regions. This process is referred to as \af{wl}. While SSDs are not the only method for utilizing flash storage, embedded devices, such as mobile and IoT devices, directly attached flash chips on the motherboard. This avoids the internal management from the \as{ftl} (discussed in detail in \cref{sec:bg_ssd_internals}) which is required with SSDs, allowing embedded devices to have direct control over the flash storage.

\subsection{Additional Flash Integrations}\label{sec:flash_integration_separation}
\begin{figure*}[!t]
    \centering
    \subfloat[]{\includegraphics[width=0.33\textwidth]{figs/flash_integration_ssd.pdf}\label{fig:flash_integration_ssd}}\hfill
    \subfloat[]{\includegraphics[width=0.33\textwidth]{figs/flash_integration_custom.pdf}\label{fig:flash_integration_custom}}\hfill
    \subfloat[]{\includegraphics[width=0.33\textwidth]{figs/flash_integration_embedded.pdf}\label{fig:flash_integration_embedded}}
    \caption{Integration of flash storage into host systems with (a) showing a conventional \as{ssd} with a \as{ftl} on the storage device, (b) a custom flash integration, through interfaces such as \as{ocssd}, custom \as{ftl}, custom device drivers, and multi-stream SSD and (c) flash storage on embedded systems with direct management for flash from the file system.}
    \label{fig:flash_integrations}
\end{figure*}

\as{ssd} is not the only integration of flash storage into full storage devices. \cref{fig:flash_integrations} shows three integration levels for flash, where \cref{fig:flash_integration_ssd} depicts the conventional integration with an \as{ssd}. \cref{fig:flash_integration_custom} shows a custom integration of flash storage, under which classification several types of devices fall. Particularly in this literature study we classify custom flash integration as either \af{ocssd}~\cite{2019-Lu-Sync_IO_OCSSD,bjorling2017lightnvm}, devices with custom firmware or \as{ftl}, and multi-stream SSD~\cite{bhimani2017enhancing,kang2014multi}. The main benefit of such a setup is that the flash characteristics are no longer hidden behind the device, giving the host an increasing level of possible management for the flash. \as{ocssd} is a type of \as{ssd} that exposes the device geometry to the host, allowing the host to manage device parallelism and allocation. Similarly, with custom firmware and \as{ftl} it is commonly the case that the device exposes more information and control of the underlying flash storage to the host. While such a device allows increased data management for the host software, it comes at increased complexity for managing the device constraints. Lastly, \cref{fig:flash_integration_embedded} shows flash integration at the embedded level, such as is commonly used in mobile devices and \af{iot} devices. In embedded flash configuration the flash chip is commonly directly attached to the motherboard, giving the host system full control over the underlying flash storage. Throughout this literature study we group file system design and mechanisms based on these three integration levels, as different levels of integration allow different degrees of flash management and ranging possibility for flash integration.

\subsection{Host Interfaces and Storage Protocols}\label{sec:ssd_host_interfaces}
Storage systems were largely relying on slow storage media, such as \as{hdd}, for which many of the legacy protocols and interfaces such as \af{scsi}, \af{sas}, \af{ata}, \af{sata}, and \af{ahci} were design for. However, the arrival of faster storage devices, including flash based storage, made the legacy protocols the bottleneck for performance~\cite{walker2012comparison}. \as{scsi} provides the standards for the physical connection of host systems to peripheral components, such as external storage including disk and tape, allowing to connect multiple devices at the same time. \as{sas} allows to increase the number of attached devices, compared to SCSI, up to 65535. \as{ata} is the interface for connecting the host system bus to the attached storage device. \as{sata} is the successor of ATA, which provides higher transfer speeds for attached devices. \as{ahci} is the standard defining the interface to communicate with \as{sata} attached devices. 

In order to integrate storage devices with \as{ahci} and \as{sata}, such that the host can communicate to the device, a \af{hba} or integrated chip on the storage device is required. These serve the purpose to provide the translation between the host bus and the storage subsystem interconnect~\cite{walker2012comparison}. As an \as{ssd} provides significantly higher speeds, and the storage interconnect becomes the bottleneck, efforts led to the development of the \af{pcie} interconnect, an extension of on \af{pci}, specifically designed to provide lower latency and increased throughput compared to \as{sata}. However, \as{ahci} storage controller connected over the \as{pcie} interconnect is still a bottleneck for the entire system with the required interconnect translation. Therefore, \af{nvme} was designed, specifically for fast SSD devices. It allows to directly connect storage devices over \as{pcie}, without the need for a \as{hba}.

An additional benefit of \as{nvme} is that the storage device can be partitioned into multiple logical extents, called namespaces, of which each can have its own \as{io} channels, allowing to exploit the internal device parallelism~\cite{walker2012comparison}. Contrary to \as{sata}, which had a single request queue in which \as{io} requests is inserted and sequentialized, \as{nvme} utilizes a \af{sq} and a \af{cq}. Requests are placed in the SQ, which allows up to 64K outstanding requests and up to 64K different \as{io} queues, and upon completion of a request the \as{nvme} controller places the result in the \as{cq} and writes to a doorbell register (called the completion queue head doorbell) to notify the host of completion for the request. Additionally, on submission of a command by the host the submission queue tail doorbell is written to announce a new request. The increased parallelism of \as{nvme} allows to better exploit \as{ssd} performance, and removes the single point of failure and contention in storage systems~\cite{xu2015performance}. Performance comparison of \as{sata} and \as{nvme} show that \as{nvme} \as{ssd} can achieve 8x higher performance than \as{sata} \as{ssd}~\cite{xu2015performance}.


==> bak/custom_integration.tex <==
\section{Custom Flash Integration}
Different types of flash-based storage devices allow for varying levels of flash management for the file system. With OCSSD, the device geometry of the underlying flash storage is exposed to the file system, allowing for specific data placement and optimizations. Multi-streamed SSDs can leverage the stream hint for the FTL to leverage increased parallelism and better data placement. Custom FTLs further extend this concept by giving the file system developers advanced interfaces and exposing distinct flash characteristics, allowing the file system to better manage data and optimize for the flash characteristics. Custom device drivers similarly allow increased device management. 

This section evaluates such storage devices, giving the host file system more flash management responsibility. We analyze the various file system implementations at this integration level, evaluating the additional flash integration modifications, which are not possible at the SSD level integration. Thus, we evaluate what additional benefits the deeper integration of custom flash devices can provide, and how file systems deal with these. We do not repeat the concepts that are discussed in the SSD integration, as they are all also applicable at this integration, instead we look only at the enhancement made by this integration on the concepts and new concepts made possible by the integration level. Table~\ref{tab:custom_integration_comparison} shows a comparison of the file systems evaluated in this section, indicating which flash challenges the particular proposed file system incorporates. Note, not all file systems in the table are discussed in the text, if they did not contribute a mechanism that is not already discussed.

\begin{table*}[!ht]
    \centering
     \begin{tabular}{||p{19mm}||p{8mm}|p{12mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||} \hline & & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
         File \newline System & Year & Type & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        Kawaguchi et al.\cite{kawaguchi1995flash} & 1995 & CD & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        DFS\cite{josephson2011direct} & 2011 & CD & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        DualFS\cite{2020-Wu-DualFS} & 2020 & OCSSD & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
        \hline
         Ext4Stream\cite{2018-Rho-Fstream} & 2018 & MS-SSD & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
         XFStream\cite{2018-Rho-Fstream} & 2018 & MS-SSD & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
         SSDFS\cite{dubeyko2019ssdfs} & 2019 & OCSSD & \xmark & \cmark & WA \& SA & \cmark & \xmark & \xmark & \xmark \\
        \hline
         RFS\cite{lee2014refactored} & 2014 & CSC & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark \\
        \hline
         StageFS\cite{2019-Lu-Sync_IO_OCSSD} & 2019 & OCSSD & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \cmark \\
        \hline
         ALFS\cite{2016-Lee-AMF} & 2016 & CFTL & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
        \hline
         OrcFS\cite{2018-Yoo-OrcFS} & 2018 & CFW & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark \\
        \hline
        ParaFS~\cite{2016-Zhang-ParaFS} & 2016 & CFTL & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        % From here on papers added from original FS Design Considerations classification
         NBFS\cite{2021-Qin-Atomic_Writes} (based on F2FS) & 2021 & OCSSD & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \cmark \\
        \hline
    \end{tabular}
    \caption{Evaluated file systems for flash-based storage with custom FTL, OCSSD, custom device driver, and multi-streamed SSD under the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. The type column indicates if the file system is built on OCSSD, custom FTL (abbreviation C-FTL), custom driver (abbreviation CD), custom storage controller (abbreviation CSC), custom FTL (CFTL), custom firmware (CFW), or multi-streamed SSD (abbreviation MS-SSD). If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented.}
    \label{tab:custom_integration_comparison}
\end{table*}

\subsection{Read/Write Asymmetry}
The close integration of flash storage to the host software, compared to SSD integration, provides the host with more knowledge of the underlying flash characteristics, allowing for more tailored data placement and algorithm integration. The close integration further allows to integrate and possible eliminate the FTL. Kawaguchi et al.~\cite{kawaguchi1995flash} provide one of the first file systems for flash, which is integrated into the flash storage driver, taking full control over flash. Similarly, integrating the file system at an enhanced level, DFS~\cite{josephson2011direct} implements a direct file system on an optimized virtual flash storage (VFS). By combining the FTL with a flash virtualization layer, which similarly to virtual memory exposes the flash as a large addressable space as a block device. Therefore, it still relies on logical addressing, which the virtual layer translates, making it backward compatible, however exposing a 64-bit logical address space. Such a layer allows to match the physical flash characteristics such as the flash erase unit to the virtual addressing, better matching flash properties compared to exposing flash as a linear address space. 

The enhanced interface of flash management allows DFS to leave block allocation for file system data and metadata, hiding latency for flash erasure, and providing consistency operations. To account for read/write asymmetry, DFS implements a lazy LRU caching policy, which implements a bloom filter to identify if blocks are present in cache (similar to MLB caching, see Section~\ref{sec:ssd_rw_asym}). However, on a cache miss is the data block only copied into the user memory, and not the cache. Only on the second miss is the data cached in LRU policy, allowing the cache to only contain the frequently accessed data.

Some modern flash devices allow the host to switch the cell level of underlying flash blocks (e.g., switching MLC to SLC)~\cite{2020-Wu-DualFS,li2019accelerating}. This provides the benefit that a lower cell level, representing less bits, has a lower read, write, and erase latency, thus providing the flash with a higher performance than with a larger cell level configuration~\cite{2020-Wu-DualFS}. This switching between flash modes is referred to as \textit{flash dual mode}, which however comes at the cost of being able to store less data in the same amount of flash as the block is only able to store half the data, in the example of switching from MLC to SLC. DualFS~\cite{2020-Wu-DualFS} utilizes the flash dual mode feature to provide a dynamically sized SLC area, alongside the remaining MLC area, to accelerate the performance of critical I/O requests. By evaluating the I/O queue depth of I/O requests, DualFS determines the criticality of the incoming request, and maps it to the SLC area for increased performance. It further profiles incoming request based on the hotness and allocates hot data into the SLC mode for lower request latency.

StageFS~\cite{2019-Lu-Sync_IO_OCSSD} overcomes the lower write performance of flash by utilizing multiple stages for file system updates. Firstly, writes are written into the first stage, called the \textit{file system staging area}. Writes to the staging area are completed in a \textit{persistence-efficient} way, which matches the write updates to the operations more optimal for flash, which are smaller fine-fine grained updates~\cite{2013-Lu-Flash_Lifetime_Reduce_With_WA} in a log structured fashion~\cite{2015-Changman-f2fs}. Secondly, writes are then regrouped, based on the file system structure and hot/cold identification, and are written to the \textit{file system image} second stage based on the group assignment in parallel over the flash parallel units (solving \textbf{FC4}). The staging area allows to write synchronous I/O directly to the staging log with optimal flash write characteristics, lowering completion latency (solving \textbf{FC7}), followed by better grouping of data when writing from the staging to the file system area.

\subsection{Garbage Collection}
Similar to the SSD integration, grouping of data based on its access frequency is a commonly used approach to mitigate GC overheads. However, the deeper integration allows to better map the hot/cold data area to specific regions on the flash, independent of the FTL intervention as with the SSD integration. Such a separation is implemented by Fstream~\cite{2018-Rho-Fstream}, which modify ext4~\cite{cao2007ext4} and xfs~\cite{sweeney1996scalability} to map different operations to different streams on a stream SSD. Ext4Stream, the modified ext4 to support streams, maps different metadata operations to different streams, including the journal writes for consistency, the inode writes, as well as different streams for the directory blocks and the bitmaps (inode and block). Furthermore, it utilizes different streams that can be created for different files and for different file extensions. The goal of such streams is to map particular files, such as LOG files for key-value stores for example to a particular stream, separating its access patterns from that of other files and file system data. Similarly, the modified XFStream utilizes different streams for the log, inodes, and specific files.

The close integration to flash allows the file system to maintain closer control, allowing specific garbage collection mechanisms to enhance the GC overhead. For this, SSDFS~\cite{dubeyko2019ssdfs} manages the storage with segments, which are mapping to a number of \textit{physical erase blocks} (PEB). Each PEB is a multiple of the flash erase unit, aligning data writing and GC to the physical unit. In order to improve on GC overheads, SSDFS employs PEB self-migration, which relies on each PEB having an associated clean PEB that upon updates can be migrated to. Furthermore, incorporating hot/cold data grouping into this scheme allows to that groups into PEBs, such that during an update all hot data can be moved to the associated PEB, invalidating the prior original PEB which can then be erased without requiring to run GC.

A different approach to mitigate GC overheads is to design the GC procedure such that accesses do not suffer from high tail latency when GC is running. TTFlash~\cite{2017-Yan-Tiny_tail} achieves this through several mechanisms. It implements \textit{plane-blocking GC}, which limits any resources that are blocking I/Os to only the affected planes on the flash. However, this leads to blocking of requests to the GC affected planes. Therefore, TTFlash implements \textit{rotating GC} that only runs at most one GC operation on a \textit{plane group}, which are planes in parallel channels allowing planes to be accessed in parallel. This ensures that a plane group is never blocked for more than a single GC operation, implying that any request will not be blocked by more than one GC operation. Additionally, with the presence of capacitors on the flash device, which can flush the memory buffers (at least parts of the buffers if not using expensive capacitors that can flush the entire device memory), GC affected write operations buffers blocked writes in memory and flushes at a later point, allowing to complete the I/O without waiting for GC to complete. TTFlash refers to this mechanism as \textit{GC-tolerant flush}.

The garbage collection cost of foreground cleaning in F2FS can take up to several seconds~\cite{2018-Yoo-OrcFS}, as it is not a preemptive task. Implementing preemptive scheduling in Kernel file systems is challenging as during the preemption the Kernel has to store the file system state to continue after higher priority tasks have finished, however there can be modified metadata from the garbage collection. OrcFS~\cite{2018-Yoo-OrcFS} implements \textit{quasi preemptive segment cleaning} (QPSC), which sets a maximum time interval $T_{max}$ (default of 100ms). After cleaning a segment it checks if the timer has expired, and if so it checks if outstanding writes are present from the host. If there are outstanding writes the locks are released and the write is executed, and if there are no outstanding writes the next segment can be cleaned and the timer is reset. This allows any host write command to not encounter a segment cleaning overhead higher than $T_{max}$.

ParaFS~\cite{2016-Zhang-ParaFS} coordinates the file system garbage collection with the garbage collection in the FTL, reducing the migration times and Overprovisioning space for GC. The file system runs greedy garbage collection on its log structure to free segments, and the FTL runs cost-benefit cleaning on the space that is being erased by the file system. Therefore, space management and garbage collection are completed by the file system, and the erasing of physical blocks is completed by the FTL. This allows to better manage GC overheads at the file system level, and avoids duplicate operations from the file system and FTL GC.

\subsection{I/O Amplification}
While write amplification can already be significantly reduced by avoiding unnecessary garbage collection through the prior discussed mechanisms, a major contributing factor in write amplification is the modification of pointers, which only require several bytes, however on an update at least a full flash page is required to be written, or in the cases of LFS an inode block needs to be written, which can comprise of multiple flash pages. One approach at solving this is employed in OFTL~\cite{2013-Lu-Flash_Lifetime_Reduce_With_WA}, an object-based FTL implementation, that utilizes \textit{backpointer-assisted lazy indexing}. It relies on inversely indexing the associated metadata to objects in the data page itself. The metadata page then contains a reverse index to the object, thus on a data update avoiding to rewrite the object metadata page, reducing write amplification. While the implementation focuses on object-based mapping, the concept can be applied to file system management. However, in order to avoid increased scan times on failure recover, after power failure, where only one page is updated, thus requiring to scan the entire region, the updated pages are tracked to indicate the most recently updated valid page. The tracking is then periodically included in the checkpointing to ensure consistency, which OFTL refers to as the \textit{updating window}.

Similar to file systems at SSD integration, file system at the custom flash integration also employ on data compression, which allows to decrease the space amplification, as well as using inline data for small files. Inline data writes the content into the inode, utilizing the inode space which would be otherwise written at the allocation unit without data, and avoiding the extra allocation to write the data. SSDFS~\cite{dubeyko2019ssdfs} incorporates all these concepts, and additionally includes delta-encoding to only write changes on data updates, instead of writing the entire new data, as well as deduplication.

A similar goal of file systems is to reduce the amount of memory that is required for the mapping table to maintain the logical-to-physical mappings. A common solution is to increase the granularity of the mapping table (e.g., block-level mapping instead of page-level mapping), requiring less mappings. However, this comes at the cost of having a larger allocation unit, and if a host write is smaller than the allocation unit it causes write amplification due to the partial flash page write when the flash page size and the file system allocation unit (block size) are not identical~\cite{2018-Yoo-OrcFS,lee2007log}. OrcFS~\cite{2018-Yoo-OrcFS,lee2007log} implements \textit{block patching} to solve this issue, which takes write requests that are smaller than the flash page size and pads the remaining space with dummy data to align the write request to flash page size. This mechanism avoids copying data if a flash page is partially written and the next LBA (in the same flash page) is written, which would trigger a copy of all LBAs in the flash page followed by writing the LBA of the new write. For instance, a flash page contains 4 LBAs, if LBAs 1-3 are written by one request and a second request to LBA 4 is issued, it cannot fill the flash page as it has already been written, therefore requiring to copy LBAs 1-3, add the new write to LBA 4 to it, and write the 4 LBAs to a new flash page. Adding of dummy data to fill pages reduces the write amplification of copying LBAs, however it still adds write amplification to fill the flash page.

\subsection{Flash Parallelism}
The hardware organization of flash allows to address flash dies and channels in parallel, which FTLs commonly do to increase performance. Architectures utilizing multiple flash chips also allow these to be addressed in parallel. At the SSD integration, the FTL commonly stripes data across the parallel units, which is hidden from the host, as the FTL controls the physical data mapping. SSDFS~\cite{dubeyko2019ssdfs} utilizes the closer integration to map data allocation of segments to PEBs, which are aligned to the physical erase unit, and additionally the allocated PEBS can be split over the available parallel unit. Therefore, utilizing PEBs over the parallel unit (e.g., flash channels) allows to stripe writes into a segment over the varying channels, increasing the device parallelism. In order to achieve this, I/O requests have to be large enough such that they can be striped across the channel and fill the PEBs mapped to the segment. SSDFS, utilizes aggressive merging of I/O requests to achieve the larger I/Os that can be striped across the parallel units.

Co-designing the FTL and the file system allows to remove uncoordinated duplicate work, and coordinate the flash management. To this end, Lee et al.~\cite{lee2014refactored} present a redesigned I/O architecture, called REDO, which avoids the duplicate operations from file system and FTL by implemented the new framework directly as the storage controller, and building the refactored file system (RFS) on top of the new controller interface. By combining the file system operations with the storage controller, the file system is responsible for running GC and managing the storage, which is made possible by REDO giving it direct access to the storage the file system managing logical-to-physical mappings. REDO implements the bad block management and wear leveling. The file system is based on LFS, and thus is also organized in segments. However, logical segments are mapped directly to physical segments, where pages in the logical segment are mapped to the physical pages across the flash channels. This firstly allows to utilize the device parallelism with the flash channels and secondly avoids to maintain a logical-to-physical mapping table for pages, as it only requires segment mappings which contain numerous pages. Similarly, OrcFS~\cite{2018-Yoo-OrcFS} implements its file system allocation unit as a \textit{superblock} (not to be confused with the file system superblock), which represents a set of flash blocks. These flash blocks are then split over the parallel units of the flash storage, such as the flash channels, allowing increased parallelism.

Exploiting the flash parallelism relies on utilizing the parallel unit, such as the flash channels. However, there are several methods that these can be utilized, as mentioned earlier in OrcFS, striping superblocks across the flash channels can utilize the channels and increases parallelism. The large allocation unit however introduces increased garbage collection overheads. Furthermore, block-level striping has lower performance than page-level striping~\cite{2016-Zhang-ParaFS}. Therefore, ParaFS~\cite{2016-Zhang-ParaFS} implements a 2-D allocation scheme, with page-level striping over the flash channels, where striping is also based on the data hotness, hence having a 2-dimensional allocation scheme. Different groups are assigned for the hotness levels, where writes are issued to the corresponding hotness group.

\subsection{Wear Leveling}
With the importance of ensuring that flash cells are utilized evenly, and no particular area burns out faster than others, devices ensure even wear across the device. At the SSD integration this is responsibility of the FTL, where the file system has little control over the physical mapping of data. With custom integration that can provide more possibility for higher software levels to manage physical mappings, there is an increased responsibility to manage wear leveling. Particular to the file system implementations that utilize the flash dual mode, which causes the lower cell level area (e.g., SLC area) to burn out quicker than the higher cell level area, due to writing the same amount of data, but not being able to storage the same amount. Therefore, DualFS~\cite{2020-Wu-DualFS} implements a \textit{write budget} in order to ensure that writes to the SLC area are not burning out, incorporating the write budget in the SLC area admission which decides if data should be written to the SLC or MLC area, resorting to writing data to the MLC area if necessary to avoid burning out the flash in the SLC area.

\subsection{Software Stack}
Similar to prior discussed file systems at SSD integration level, several file systems with close flash integration also minimize the software stack through various mechanisms. In particular, closer integration to the flash storage allows to remove parts of the redundancy present in the conventional software stack, where the FTL does independent data management and operations, uncoordinated with the file system and software layers above the storage device. At the SSD integration level a significant amount of duplicate work is done by the file system and the flash storage. LFS requires to run garbage collection to free space in its log, and the FTL similarly requires to run garbage collection on the flash to free erase blocks. Stacking multiple layers with uncoordinated operations on top of each other, such as a log-based file system and a log-based FTL, generates duplicate work, which in turn leads to significant performance impacts~\cite{2014-yang-dont_stack_log_on_log}. Co-designing of the FTL and file system has shown benefits of reduced memory requirements for logical-to-physical mappings, and increased channel parallelism through file system information~\cite{2013-Qiu-Codesign_FTL_FS}.

Therefore, merging operations of the file system with the FTL can provide performance gains, which are not possible at the SSD integration level, but at the custom flash integration level. DualFS~\cite{2020-Wu-DualFS} utilizes the custom integration with OCSSD to merge the garbage collection of the file system with that of the FTL, and present this scheme as \textit{global garbage collection}. Similar to file systems at SSD integration, avoiding Kernel intervention in the I/O path can minimize I/O overheads. Direct accesses file systems, including DFS~\cite{josephson2011direct}, avoid such an I/O path and provide direct access to the underlying storage.

A different approach taken by Lee at al.~\cite{2016-Lee-AMF} is to modify the block interface with the flash characteristics, moving responsibility directly to the file system, or other application built on top of it. The resulting interface called \textit{application managed flash} (AMF) exposes a block interface that does not allow overwriting unless an explicit erase is issued for the blocks. This matches the flash requirement that prior to overwriting data it has to be erased. The interface is implemented as a custom FTL, called AFTL, and the authors built a file system (ALFS) with this new interface. This avoids the duplicate garbage collection of the FTL and the file system, as the garbage collection of the ALFS erases blocks during garbage collection, informing the FTL to erase the physical block.

\subsection{I/O Scheduling}
Similar to the scheduler merging I/O requests in the I/O path for SSDs, custom flash integration incorporates the concept of merging similarly. The VFS layer on top of which DFS~\cite{josephson2011direct} is built, can merge all incoming requests, as virtualized storage can map logical to physical addresses similar to virtual memory, merging incoming block writes is achieved when the VFS decides on the physical mapping. A further issue of the I/O path are the overheads of the operating system and file system. Moneta-D~\cite{caulfield2012providing}, based on the original Moneta project~\cite{caulfield2010moneta}, implements this by bypassing the file and operating system, and providing \textit{channels} to the storage for each process. Channels are virtual interfaces to the storage area for the accessed region, and ensure that correct permissions are enforced for each process, which allows bypassing the file and operating system permission checks. Permission checks are instead enforced at the hardware level, only giving access to valid processes. Once permissions are established for a channel, an emulated in memory register is written to execute commands on the storage area. Commands are executed over DMA on the channel. With a user-space library, against which application can be linked, are the library calls replaced to go to the Moneta-D driver, instead of through the file system and Kernel, thus allowing to minimize the software stack and avoid overheads (solving \textbf{FC6}).

ALFS~\cite{2016-Lee-AMF}, which is built on a custom FTL which does not allow overwrites, but rather requires the application to issue an erase before blocks can be overwritten, exploits the flash parallelism by mapping consecutive segments to the flash channels and utilizing different I/O queues for each flash channel. Each flash channel has a separate I/O queue, upon which I/O requests are sorted when issued to the flash controller. This striping of segment data allows exploiting the flash parallelism, resulting in higher performance, and furthermore handles I/Os arriving in random order, due to possible rescheduling in the Kernel block layer. As I/Os are sorted per channel, such that for instance writes at page 0 go to channel 1, writes at page 1 go to channel 2, and so forth, they can be assigned to the correct channel independent of the arrival order. Furthermore, AFTL utilizes multiple segments in parallel, where data grouping and checkpointing can use different channels. 

Similarly, ParaFS~\cite{2016-Zhang-ParaFS} implements \textit{parallelism-aware scheduling}, which also maintains different I/O queues for each channel. However, it extends this concept by using a \textit{dispatching phase} and a \textit{request scheduling phase}. The dispatching phase optimizes write I/Os with a scheduling to the respective channels based on the utilization of the channel, such that the least utilized channels receives more requests. All requests are assigned a weight, which indicates their priority in the queue, where read requests weight is lower than that of write requests, because of the asymmetric performance of flash storage. During the request scheduling phase the scheduler assigns slices the read and write/erase operations in the individual queues, such that if the time from the slice of a read operation is up and the queue contains no other read requests, a write or erase is scheduled, based on a fairness formula that incorporates the amount of free space in the block and concurrently active erase operations on other channels. This allows to minimize the erase operations on the flash, giving always free channels to utilize and maintain a fair schedule between write and erase operations.

Qin et al.~\cite{2021-Qin-Atomic_Writes} argue that I/O ordering limits from utilizing the parallelism of flash devices. Especially as the Linux block layer does not guarantee particular ordering, flags such as \textit{forced unit access (FUA)}, indicating that I/O completion is signaled upon arrival of data on the storage, and \textit{PREFLUSH}, which before completing the request flushes the volatile caches, have to be set in order to ensure a specific ordering~\cite{2021-Qin-Atomic_Writes}. With file systems, the I/O of metadata and data has a particular ordering, such that metadata can only point to data that exists, needing to ensure that data is written prior to metadata. Removing of I/O ordering allows to eliminate this need and better utilize the flash parallelism. Utilizing the OOB area on flash pages, the file system developed by Qin et al., called NBFS, maintains versioning in order to identify out of order updates. Furthermore, updates are done using atomic writes (discussed in Section~\ref{sec:failure_consistency}). The issuing of \textit{FUA} requests further implies that its I/Os cannot be merged in the scheduler~\cite{2021-Qin-Atomic_Writes}, implying that if a smaller than flash page size \textit{FUA} I/O request is issued, it is padded to the page size, causing write amplification. NBFS solves this with its atomic writes that imply that the \textit{FUA} request does not immediately have to be written to the flash, but instead wait for all data blocks to arrive, which are then used to fill the pages, allowing to reduce the write amplification (\textbf{FC3}).


==> bak/embedded_integration.tex <==
\section{Embedded Flash Integration}
The last group of flash-based storage systems is the embedded systems, which give the file system full control over the underlying flash storage. This allows the file system to fully manage the storage, however comes at the cost of increased complexity. This section evaluates the file systems for flash-based embedded systems, analyzing how different file systems solve the particular design challenges of flash, leveraging the direct management of flash media. Again, we only discuss concepts that are not mentioned in the prior integration levels or methods of which further optimization is possible as a result of the embedded flash integration. Table~\ref{tab:embedded_integration_comparison} shows a comparison of the various file systems discussed in this section, evaluating the flash challenge(s) that a file system addresses. Note, also not all file systems in the table are discussed in this section if they do not contribute any new methods not already discussed.

\begin{table*}[!ht]
    \centering
    \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
        \hline 
        & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
        File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        CFFS\cite{2006-Lim-NAND_fs} & 2006 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
        \hline
        UBIFS\cite{hunter2008brief} & 2008 & \cmark & \cmark & SA & \xmark & \cmark & \xmark & \xmark \\
        \hline
        FlexFS\cite{2009-Sungjin-FlexFS} & 2009 & \cmark & \cmark & WA & \xmark & \cmark & \xmark & \xmark \\
        \hline
        ScaleFFS\cite{2008-Jung-ScaleFFS} & 2008 & \cmark & \xmark & WA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        JFFS\footnote{focusing on JFFS V2}\cite{woodhouse2001jffs} & 2001 & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark \\
        \hline
        EnFFiS\cite{park2013enffis} & 2013 & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark \\
        \hline
        FlogFS\cite{nahill2015flogfs} & 2015 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        RFS\cite{schildt2012contiki} & 2012 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
        \hline
        F2FS + SAC\cite{2015-Park-Suspend_Aware_cleaning-F2FS} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        NANDFS\cite{2009-Zuck-NANDFS} & 2009 & \cmark & \cmark & WA & \xmark & \cmark & \xmark & \xmark \\
        \hline
        NAMU\cite{2009-Park-Multimedia_NAND_Fs} & 2009 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
        \hline
        LeCramFS\cite{2007-Hyun-LeCramFS} & 2007 & \cmark & \xmark & SA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        F2FS + FPC\cite{2021-Ji-F2FS_compression} & 2021 & \cmark & \cmark & SA & \cmark & \xmark & \xmark & \xmark \\
        \hline
        NAFS\cite{2011-Park-Multi_NAND} & 2011 & \cmark & \xmark & WA & \cmark & \cmark & \xmark & \xmark \\
        \hline
        YAFFS\cite{manning2010yaffs,aleph2001yaffs,manning2002yaffs} & 2010\footnote{references include all YAFFS publications, however we focus on YAFFS2} & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        % From here on papers added from original FS Design Considerations classification
        LogFS\cite{engel2005logfs} & 2005 & \xmark & \cmark & SA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        DFFS\cite{2008-Kim-DFFS} & 2008 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        RFFS\cite{park2006flash} & 2006 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        F2FS + ARS\cite{2020-Yang-F2FS_Framentation} & 2020 & \cmark & \cmark & WA \& RA & \cmark & \xmark & \xmark & \xmark \\
        \hline
        F2FS + RM-IPU\cite{2022-Lee-F2FS_Address_Remapping} & 2022 & \cmark & \cmark & WA \& RA & \cmark & \xmark & \xmark & \xmark \\
        \hline
        DeFFS\cite{2011-Lim-DeFFS} & 2011 & \cmark & \xmark & WA & \xmark & \xmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Evaluated file systems for embedded systems with flash storage under the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented. Continued in Table~\ref{tab:embedded_integration_comparison_cont}.}
    \label{tab:embedded_integration_comparison}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
        \hline 
        & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
        File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        O1FS\cite{2014-Hyunchan-O1FS} & 2014 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        ELOFS\cite{2022-Zhang-ELOFS,2020-Zhang-LOFFS} & 2022 & \xmark & \cmark & WA & \cmark & \cmark & \xmark & \xmark \\
        \hline
        MNFS\cite{kim2006mnfs} & 2006 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        Coffee FS\cite{2009-Tsiftes-Coffee_FS} & 2009 & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Table~\ref{tab:embedded_integration_comparison} continued.}
    \label{tab:embedded_integration_comparison_cont}
\end{table*}

\subsection{Read/Write Asymmetry}
With the lower integration level and increased flash management responsibility comes increased complexity. Similar to DualFS~\cite{2020-Wu-DualFS}, which implemented a dynamically reconfigurable file system for dual-flash mode (switching of the flash cell level such as MLC to SLC), flexfs\cite{2009-Sungjin-FlexFS}, it implements a similar mechanism for increased performance on the SLC area. The drawback of such a design is that data is required to be moved from the SLC area to the MLC area as it has a lower write lifetime, and is aimed at the for critical I/O requests that require lower completion latency, which in turn causes \textit{data migration overheads}. To solve this, FlexFS implements several migration techniques that aim to hide the overheads for the data migration from the host. The first technique revolves around \textit{background migration}, which pushes the migration to happen when the system is idle. The second technique is \textit{dynamic allocation}, which writes non-critical requests to the MLC area, saving on flash degradation in the SLC area, as well as avoiding future data migration. The dynamic allocator functions based on measurements of prior system idle times from I/O requests, to predict current idle time, and if sufficient idle time is predicted in order to complete data migration, the data is written to the SLC, and otherwise part of the data, depending on required migration and idle time, is written to the MLC area. The last technique, \textit{locality-aware data management}, takes into account the hotness of data, and the dynamic allocator attempts to migrate only cold data from the SLC area.

NAFS~\cite{2011-Park-Multi_NAND} implements a file system which utilizes multiple NAND chips, by representing them as a storage array to the file system in order to simplify the management of the different chips, where parallelism is utilized by striping I/O across the different chips (\textbf{FC4}). In order to incorporate the asymmetric flash performance, it further implements a \textit{double list cache}, containing a clean list with only clean pages for caching of data, and a second dirty list for writing of modified pages and to prefetch of pages based on the access patters, only containing dirty pages. Prefetching is striped across the NAND chips, increasing read performance, and minimizing cache misses from the lists. The benefit of two separate lists is that firstly it allows to cache write operations and avoid small writes to the flash device, and secondly it prefetches data into the clean list in order to minimize cache misses.

\subsection{Garbage Collection}
A major challenge of flash-based storage is the performance impacts of garbage collection. At points where the device has to move valid pages in blocks to a free space, and erase the old block, application performance becomes unpredictable and can encounter significantly higher tail latency. There are several approaches for file systems to utilize in order to minimize the required garbage collection. While we discuss these methods in the context of file systems, they are applicable to the majority of applications utilizing flash storage.

Similar to prior discussed file systems, UBIFS~\cite{hunter2008brief}, which is built on the unsorted block images (UBI)~\cite{gleixner2006ubi}. UBI implements the management of the flash storage, including allocation and wear leveling. In order for UBIFS to decrease the garbage collection overheads, it firstly utilizes inline metadata where file data and metadata are stored together. Secondly similar to existing file systems, it utilizes a log where updates are initially written to, before writing to the on-flash index structure, avoiding small writes.

A different approach to reducing the garbage collection overheads for the file system is by adding a level of indirection. As Butler Lampson mentioned in his famous quote from 1972 (which was originally stated by David Wheeler), ``Any problem in computer science can be solved with another level of indirection``~\cite{lampson1993principles}. For this, NANDFS~\cite{2009-Zuck-NANDFS} implements a \textit{sequencing layer} on top of which the file system is built, which handles block allocation, garbage collection, wear leveling, and the logical-to-physical flash mapping. The sequencing layer implements the block allocation as immutable storage, therefore when file system data is updated, it cannot overwrite, and simply marks the data as obsolete. The new updated data is written in a newly allocated block, however the sequencing layer implements the logical-to-physical mapping, with a mapping table, such that the logical block address to the new data is the same as the old logical block address, avoiding the updating of data addresses in the file system metadata. This implies that the file system does less writing by eliminating metadata updates, but it also does not run any garbage collection.

\subsubsection{Data Grouping}
Similar to discussed file systems, grouping of data is also beneficial for embedded devices to minimize garbage collection. Similar to how F2FS assigns a temperature to the data, the Core Flash File System (CFFS)~\cite{2006-Lim-NAND_fs}, which is an earlier flash-based file system, differentiates between hotness of metadata to data. Given that metadata is more likely to be updated frequently, separating metadata from data improves on required garbage collection. Specifically, since metadata is often updated even if the data is not updated, for example in scenarios where the file attributes (access time, permissions, etc.) are updated or the file is moved. With CFFS being a file system for embedded devices, there is more control over the flash storage, as it has direct flash access without an FTL, it separates metadata and data in distinct blocks (the flash erase unit). However, this can quickly lead to uneven wear across the flash, since metadata blocks are erased more frequently, which CFFS solves by switching metadata and data blocks after an erase, such that an erased metadata block becomes a free data block.

\subsubsection{Garbage Collection Policies}
On embedded devices, and in particular mobile devices, in order to save energy the device suspends all threads when not needed (e.g., when the mobile screen is turned off). This implies that all file system threads are also suspended, which means the file system cannot run the background garbage collection during these inactive sessions. Therefore, \textit{suspend aware cleaning}~\cite{2015-Park-Suspend_Aware_cleaning-F2FS} (we abbreviate it as SAC) is an addition to LFS, which utilizes the slack time, which is the time between the suspend initiation (e.g., turning off the mobile device screen) and the suspending of the file system threads. It uses this slack time to run background garbage collection, however it does not write any data on the flash storage, but instead selects a victim block and brings the still valid pages in the page cache and marks these as dirty, resulting in all pages in the victim block to be dirty, which allows it to be erased. This process is referred to as \textit{virtual segment cleaning}, which however is not run every time the screen is turned off, but rather based on the device utilization, which is called \textit{utilization based segment cleaning}. Similarly, file-aware garbage collection (FaGC)~\cite{yan2014efficient} is an optimization to garbage collection policies, which maintains an update frequency table (UTF) for each logical block address of a file, in order to to group valid pages in the victim block based on the access frequency when these are copied to a new block during garbage collection. This is similar to grouping hot and cold data, but at the level of garbage collection for LBAs in a file, and therefore allows to minimize the GC overheads.

The application domain of embedded devices is often particular to specific workloads and files. This allows file systems to optimize for a particular domain, such as multimedia content. NAMU~\cite{2009-Park-Multimedia_NAND_Fs} showcases a file system that, similar to other file systems, also manages flash in a number of segments, however these are aligned to match the characteristics of large files, and in particular multimedia content. The main benefit of large file mappings, aside of lower memory usage from fewer address mappings, the possible optimization in garbage collection. Given that multimedia files are rarely modified, and if removed, all file segments are erased in one unit, garbage collection in NAMU is done at the granularity of files. During garbage collection, NAMU selects a victim file with the smallest erase count, which is maintained for each file, and the erasure of large files allows freeing up significantly more space. 

\subsection{I/O Amplification}
While write operations are the major cause of flash cells burning out, read operations also pay a toll on the flash. The assumption that read operations can be issued indefinitely without interfering with the flash cells is flawed, as the current flash technology utilizes flash gates that are only capable of holding very few electrons (determining the charge of the gate) due to their size~\cite{lu2009future,shin2005non}. This makes the cells increasingly susceptible to \textit{read disturbance}~\cite{2015-Liu-Read_leveling}, requiring frequent rewriting to ensure the charge stays consistent. In order to control read disturbance, Liu et al.~\cite{2015-Liu-Read_leveling} propose to include in the FTL read-leveling mechanisms. While the discussion is aimed at FTL implementations, the ideas are applicable to file systems in embedded flash integration, which control physical mappings. Read-hot data is isolated from other data pages by placing the hot pages into \textit{shadow blocks}, which contain no valid data (i.e., they can be invalid blocks). However, this requires to identify the read-hot pages, where a tracking of read counters for each page would require significant resources. Therefore, a \textit{second-chance monitoring strategy} is used, which initially tracks the reads for a particular block, and upon reaching a threshold indicating the block contains read-hot pages, the individual pages in the block are tracked on read counters. Finally, pages reaching a threshold are then copied to the shadow blocks, thus avoiding the tracking of read counters for individual pages and only copying hot pages into the shadow blocks. While this strategy requires copying of read-hot pages to shadow blocks, it minimizes read disturbance which in turn minimizes the write amplification it causes.

Similar to SSD integration, an effective method to reduce space amplification is to utilize compression. LeCramFS~\cite{2007-Hyun-LeCramFS} (short for less crammed FS) is such a read-only file system with compression for embedded devices. However, unlike other existing file systems, which utilize a memory buffer for decompression, to read the data, decompress it, followed by writing the uncompressed data to a memory space, LeCramFS does not utilize a decompression buffer, avoiding copying overheads. It achieves this by using \textit{page boundary alignment} (PBA), in which the block with the compressed data is aligned to the page, such that compressed data does not share pages. Conventionally, compressed data blocks are allocated directly after prior blocks, even if the prior page is not fully utilized, resulting in blocks sharing the same pages. This requires the reading of all the compressed data into the device cache, separating the compressed data, followed by decompressing the desired part. Aligning compressed data to the page unit allows to directly bring the desired data into the device cache and decompressing it, avoiding an extra copy to separate the requested part. 

In order to avoid wasting space if the page is not fully utilized from a single compression, LeCramFS implements a partial compression which fits part of data as a separate compressed part, and the remaining data is compressed in the next free region. The difference from this and conventional compression is that partial compression splits the data and compresses it separately into the available space, avoiding that the entire compressed data spans across page boundaries. Similar compression is applied to F2FS~\cite{2021-Ji-F2FS_compression} for mobile devices, where \textit{file pattern-guided compression} (FPC) selects the compression method for files based on how compressible they are. For instance SQLite journals are rarely read and can be easily compressed, generic files can be compressed with inline metadata, and binaries can be compressed using specific compression methods.

\subsection{Flash Parallelism}
While IoT devices such as microcontrollers commonly only contain a small amount of flash, such as a single flash chip, limiting the possible parallelism that can be exploited, parallelism on more resource available embedded devices can be utilized. NAFS~\cite{2011-Park-Multi_NAND} utilizes the flash parallelism by striping I/O across multiple flash chips. Similarly, YAFFS~\cite{manning2010yaffs,aleph2001yaffs,manning2002yaffs} allocates data in units of \textit{chunks}, which can be a single page, however in the presence of multiple NAND chips, a chunk can be mapped to multiple pages, with a single page from each chip being in a chunk. This results in I/Os being striped across the flash chips.

\subsection{Wear Leveling}
\ntytodo{add papers here? several that have checkmark on WL in table}

\subsection{Software Stack}
The largest benefit of embedded flash is the possible reduction of layers in the software stack. The direct control over the flash storage allows to remove the FTL, and optimize flash management at the file system level, which in turn allows to incorporate the file system knowledge of data into the data placement and flash management. JFFS~\cite{woodhouse2001jffs} is a well known file system for embedded devices, which particularly argues for removing the redundant layers of the FTL and file system, and include all flash management in the file system level.

\ntytodo{can we extend this? it's mostly embedded so directly on flash anyways, also JFFS doesn't really minimize the stack, just argue for it, maybe drop this section during refactor?}


==> bak/fc_intro.tex <==
\section{Flash Integration Organization}
\ntytodo{coordinate this section}
With conventional SSDs, the FTL has full control over the underlying flash media. As a result, the possibility for file systems to fully incorporate each flash challenge is limited. However, particular design decisions in the file system aid the performance of the FTL and help leverage the flash characteristics. Therefore, this section covers the file systems that are particularly built on conventional flash-based SSDs (recall Figure~\ref{fig:flash_integration_ssd}), with an FTL exposing a conventional block interface. Table~\ref{tab:ssd_integration_comparison} shows a comparison of all file systems meeting this criteria, evaluating if the file system provides novel methods for handling of certain flash characteristics. As all file systems are log-structured file systems, which is a write optimized data structure due to its append only nature, which further inherently provides basic wear leveling by writing everything sequentially, the WL column is only marked on file systems that further extend this mechanism with additional novel methods.

\begin{table*}[!t]
    \centering
    \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
        \hline 
        & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
        File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        F2FS\cite{2015-Changman-f2fs} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        F2FS + SCJ\cite{2021-Gwak-SCJ} & 2021 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        SFS\cite{2012-Min-SFS} & 2014 & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        ReconFS\cite{2014-Lu-ReconFS} & 2014 & \xmark & \xmark & WA \& SA & \cmark & \xmark & \xmark & \xmark \\
        \hline
        URFS\cite{2020-Tu-URFS} & 2020 & \cmark & \cmark & WA & \xmark & \xmark & \cmark & \cmark \\
        \hline
        EvFS\cite{2019-Yoshimura-EvFS} & 2020 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
        \hline
        BetrFS\cite{2022-Jiao-BetrFS} & 2022 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        CSA-FS\cite{huang2013improve} & 2013 & \cmark & \xmark & SA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        DashFS\cite{2019-Liu-fs_as_process} & 2019 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
        \hline
        DevFS\cite{2018-Kannan-DevFS} & 2018 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        % From here on papers added from original FS Design Considerations classification
        Max\cite{2021-Liao-Max} & 2021 & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark \\
        \hline
        SpanFS\cite{2015-Kang-SpanFS} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark \\
        \hline
        exF2FS\cite{2022-Oh-exF2FS} & 2022 & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Evaluated file systems for flash-based SSD integration (with conventional FTL) and the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. As the majority of file systems are LFS-based designs, the table indicates if the file system employs a novel method in addition to what is required of LFS. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented.}
    \label{tab:ssd_integration_comparison}
\end{table*}

\textbf{Custom Flash Integration-Level.} Different types of flash-based storage devices allow for varying levels of flash management for the file system. With OCSSD, the device geometry of the underlying flash storage is exposed to the file system, allowing for specific data placement and optimizations. Multi-streamed SSDs can leverage the stream hint for the FTL to leverage increased parallelism and better data placement. Custom FTLs further extend this concept by giving the file system developers advanced interfaces and exposing distinct flash characteristics, allowing the file system to better manage data and optimize for the flash characteristics. Custom device drivers similarly allow increased device management. 

This section evaluates such storage devices, giving the host file system more flash management responsibility. We analyze the various file system implementations at this integration level, evaluating the additional flash integration modifications, which are not possible at the SSD level integration. Thus, we evaluate what additional benefits the deeper integration of custom flash devices can provide, and how file systems deal with these. We do not repeat the concepts that are discussed in the SSD integration, as they are all also applicable at this integration, instead we look only at the enhancement made by this integration on the concepts and new concepts made possible by the integration level. Table~\ref{tab:custom_integration_comparison} shows a comparison of the file systems evaluated in this section, indicating which flash challenges the particular proposed file system incorporates. Note, not all file systems in the table are discussed in the text, if they did not contribute a mechanism that is not already discussed.

\begin{table*}[!ht]
    \centering
     \begin{tabular}{||p{19mm}||p{8mm}|p{12mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||} \hline & & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
         File \newline System & Year & Type & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        Kawaguchi et al.\cite{kawaguchi1995flash} & 1995 & CD & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        DFS\cite{josephson2011direct} & 2011 & CD & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        DualFS\cite{2020-Wu-DualFS} & 2020 & OCSSD & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
        \hline
         Ext4Stream\cite{2018-Rho-Fstream} & 2018 & MS-SSD & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
         XFStream\cite{2018-Rho-Fstream} & 2018 & MS-SSD & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
         SSDFS\cite{dubeyko2019ssdfs} & 2019 & OCSSD & \xmark & \cmark & WA \& SA & \cmark & \xmark & \xmark & \xmark \\
        \hline
         RFS\cite{lee2014refactored} & 2014 & CSC & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark \\
        \hline
         StageFS\cite{2019-Lu-Sync_IO_OCSSD} & 2019 & OCSSD & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \cmark \\
        \hline
         ALFS\cite{2016-Lee-AMF} & 2016 & CFTL & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
        \hline
         OrcFS\cite{2018-Yoo-OrcFS} & 2018 & CFW & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark \\
        \hline
        ParaFS~\cite{2016-Zhang-ParaFS} & 2016 & CFTL & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        % From here on papers added from original FS Design Considerations classification
         NBFS\cite{2021-Qin-Atomic_Writes} (based on F2FS) & 2021 & OCSSD & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \cmark \\
        \hline
    \end{tabular}
    \caption{Evaluated file systems for flash-based storage with custom FTL, OCSSD, custom device driver, and multi-streamed SSD under the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. The type column indicates if the file system is built on OCSSD, custom FTL (abbreviation C-FTL), custom driver (abbreviation CD), custom storage controller (abbreviation CSC), custom FTL (CFTL), custom firmware (CFW), or multi-streamed SSD (abbreviation MS-SSD). If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented.}
    \label{tab:custom_integration_comparison}
\end{table*}

\textbf{Embedded Flash Integration-Level.} The last group of flash-based storage systems is the embedded systems, which give the file system full control over the underlying flash storage. This allows the file system to fully manage the storage, however comes at the cost of increased complexity. This section evaluates the file systems for flash-based embedded systems, analyzing how different file systems solve the particular design challenges of flash, leveraging the direct management of flash media. Again, we only discuss concepts that are not mentioned in the prior integration levels or methods of which further optimization is possible as a result of the embedded flash integration. Table~\ref{tab:embedded_integration_comparison} shows a comparison of the various file systems discussed in this section, evaluating the flash challenge(s) that a file system addresses. Note, also not all file systems in the table are discussed in this section if they do not contribute any new methods not already discussed.

\begin{table*}[!ht]
    \centering
    \begin{threeparttable}
        \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
            \hline 
            & & \multicolumn{7}{|c||}{Flash Challenge} \\
            \hline
            File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
            \hline
            \hline
            CFFS\cite{2006-Lim-NAND_fs} & 2006 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
            \hline
            UBIFS\cite{hunter2008brief} & 2008 & \cmark & \cmark & SA & \xmark & \cmark & \xmark & \xmark \\
            \hline
            FlexFS\cite{2009-Sungjin-FlexFS} & 2009 & \cmark & \cmark & WA & \xmark & \cmark & \xmark & \xmark \\
            \hline
            ScaleFFS\cite{2008-Jung-ScaleFFS} & 2008 & \cmark & \xmark & WA & \xmark & \xmark & \xmark & \xmark \\
            \hline
            JFFS\tnote{†}\cite{woodhouse2001jffs} & 2001 & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark \\
            \hline
            EnFFiS\cite{park2013enffis} & 2013 & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark \\
            \hline
            FlogFS\cite{nahill2015flogfs} & 2015 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
            \hline
            RFS\cite{schildt2012contiki} & 2012 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
            \hline
            F2FS + SAC\cite{2015-Park-Suspend_Aware_cleaning-F2FS} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
            \hline
            NANDFS\cite{2009-Zuck-NANDFS} & 2009 & \cmark & \cmark & WA & \xmark & \cmark & \xmark & \xmark \\
            \hline
            NAMU\cite{2009-Park-Multimedia_NAND_Fs} & 2009 & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
            \hline
            LeCramFS\cite{2007-Hyun-LeCramFS} & 2007 & \cmark & \xmark & SA & \xmark & \xmark & \xmark & \xmark \\
            \hline
            F2FS + FPC\cite{2021-Ji-F2FS_compression} & 2021 & \cmark & \cmark & SA & \cmark & \xmark & \xmark & \xmark \\
            \hline
            NAFS\cite{2011-Park-Multi_NAND} & 2011 & \cmark & \xmark & WA & \cmark & \cmark & \xmark & \xmark \\
            \hline
            YAFFS\cite{manning2010yaffs,aleph2001yaffs,manning2002yaffs}\tnote{‡} & 2010 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
            \hline
            % From here on papers added from original FS Design Considerations classification
            LogFS\cite{engel2005logfs} & 2005 & \xmark & \cmark & SA & \xmark & \xmark & \xmark & \xmark \\
            \hline
            DFFS\cite{2008-Kim-DFFS} & 2008 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
            \hline
            RFFS\cite{park2006flash} & 2006 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
            \hline
            F2FS + ARS\cite{2020-Yang-F2FS_Framentation} & 2020 & \cmark & \cmark & WA \& RA & \cmark & \xmark & \xmark & \xmark \\
            \hline
            F2FS + RM-IPU\cite{2022-Lee-F2FS_Address_Remapping} & 2022 & \cmark & \cmark & WA \& RA & \cmark & \xmark & \xmark & \xmark \\
            \hline
        \end{tabular}
        \begin{tablenotes}
            \item[†] Focusing on JFFS V2.
            \item[‡] References include all YAFFS publications, however we focus on YAFFS2.
        \end{tablenotes}
    \end{threeparttable}
    \caption{Evaluated file systems for embedded systems with flash storage under the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented. Continued in Table~\ref{tab:embedded_integration_comparison_cont}.}
    \label{tab:embedded_integration_comparison}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
        \hline 
        & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
        File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        DeFFS\cite{2011-Lim-DeFFS} & 2011 & \cmark & \xmark & WA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        O1FS\cite{2014-Hyunchan-O1FS} & 2014 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        ELOFS\cite{2022-Zhang-ELOFS,2020-Zhang-LOFFS} & 2022 & \xmark & \cmark & WA & \cmark & \cmark & \xmark & \xmark \\
        \hline
        MNFS\cite{kim2006mnfs} & 2006 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        Coffee FS\cite{2009-Tsiftes-Coffee_FS} & 2009 & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Table~\ref{tab:embedded_integration_comparison} continued.}
    \label{tab:embedded_integration_comparison_cont}
\end{table*}



==> bak/lfs.tex <==
\subsection{Log-Structured File Systems}
A ubiquitous approach of managing persistent storage devices is with file systems, providing the familiar file and directory interface for organizing storage. While there exist a plethora of different file systems, they largely rely on similar concepts, albeit often using different data structures and naming. The lack of in-place updates on flash pages, making sequential writes a requirement, makes \af{lfs}~\cite{1992-Rosenblum-LFS,2006-Konishi-Linux_LFS,seltzer1993implementation} a suitable file system design. Originally designed to minimize random writes on HDDs, and thus minimize arm movements on the disk, LFS have been around for several years. The design of log-structured file systems revolves around writing data as a log, appending new data sequentially on the storage device. Similar to the \as{ftl}, as data is being updated in a \as{lfs}, the log contains an increasing amount of no longer needed data, requiring \as{gc} to be freed and regain the used space.

In \as{lfs}, due to the convention coming from the block interface for \as{hdd} integration, storage is addressed in \textit{sectors}, typically 512B or 4KiB, representing the smallest unit of I/O on the device. File systems then divide the storage space in a number of \textit{blocks}, commonly 4KiB, which consists of at least one up to multiple sectors. Blocks are the unit in which file systems allocate space for files. Next, we discuss the design of the de facto standard \as{lfs} for flash storage devices, F2FS~\cite{2015-Changman-f2fs}.

\subsection{F2FS - Flash Friendly File System}
The most widely adopted \as{lfs} for flash storage is F2FS~\cite{2015-Changman-f2fs}. With it being the de facto standard of flash file systems, a large number of file systems are based on its design. In F2FS, the data space is divided into \textit{segments} (typically 4KiB), presenting the smallest writable unit in the file system in which data space is allocated. Segments are then grouped into \textit{sections}, representing the erase unit of F2FS at which it runs victim selection during \as{gc}. Furthermore, the section size is aligned to the flash erase unit, to amortize overheads and avoid unnecessary copying data with \as{ftl} garbage collection.

To minimize the garbage collection overheads, F2FS groups data based on the modification frequency. It achieves this by assigning a temperature (hold/warm/cold) to the data blocks, and pre-defines classifications for direct node blocks, as these are frequently modified, and indirect node blocks are classified as cold, as these are not frequently modified. To further extend this mechanism, F2FS maintains six different logging zones for the different temperature assignments (hot/warm/cold for nodes and file data). In F2FS \as{gc} is commonly referred to as \textit{cleaning}, and is run periodically (called \textit{background cleaning}) or when space is needed (called \textit{foreground cleaning}). The cleaning policies implemented in F2FS are greedy~\cite{2010-Bux-Greedy_GC,kawaguchi1995flash} and cost-benefit~\cite{kawaguchi1995flash,1992-Rosenblum-LFS,wu1994envy}, which are used for foreground and background cleaning respectively.

\begin{figure}[!t] 
    \centering
    \includegraphics[width=0.49\textwidth]{figs/f2fs-inode.pdf}
    \caption{The \as{inode} structure of F2FS, figure retrieved from F2FS~\cite{2015-Changman-f2fs}.}
    \label{fig:f2fs-inode}
\end{figure}

Data in file systems is managed through an \af{inode}. \cref{fig:f2fs-inode} shows the inode of F2FS. It contains all information of a file, including the file specific metadata on creation time, access permissions, file name, and more. For identifying the data blocks of the associated file, inodes contain a fixed number of direct pointers to the addresses of the file data. Since inodes are allocated in blocks, they can often contain inline data of the file, if the file data fits in the available space of the inode. To be able to locate larger files, inodes utilize \textit{multi-level indexing}, where indirect pointers point to blocks containing further pointers to more data blocks. There are several levels of indirection, where a \textit{single indirect} pointer points to one block containing pointers to the blocks which contain the data. For example, with a block size of 4KiB and 4B addresses, a single indirect pointer can store 1024 addresses, which each point to 4KiB of data, giving an addressable space of $4KiB*1024=4MiB$ (plus the number of direct pointers in the inode). Increasing the level of indirection further increases the maximum file size of the file system, where nowadays file systems most commonly provide up to three levels of indirect pointers, allowing in the example of 4KiB block size and 4B addresses, a maximum file size of $4KiB*(1024+1024^2+1024^3)=4TiB$ (plus the number of direct pointers). While multi-level indexing is a popular implementation in file systems, other solutions such as \textit{extents} exist, utilizing a single pointer to a contiguous number of blocks for the file. This approach decreases the metadata size by requiring only a single pointer, however it is more difficult of finding contiguous number of blocks for allocating space for the file.

File systems commonly utilize tree-based indexing data structures in order to achieve a worst case time complexity of $\mathcal{O}(\log{}n)$ for locating of inodes or other metadata, compared to a log based approach requiring to scan the entire log, corresponding to $\mathcal{O}(n)$ worst case time complexity. However, a tree-based data structure introduces the Wandering Tree Problem~\cite{bityutskiy2005jffs3}, where if a leaf node is modified by changing it to point to new data, thus requiring a new entry at the end of the log, its parent node also requires to change the pointer to the changed node. This parent node then also requires to be updated, propagating the changes all the way up the tree to the root node. Therefore, F2FS manages metadata for segment allocations in a \af{nat}. It divides allocated blocks into three types; \textit{inode blocks} that contain the metadata for the file from the \as{inode}, \textit{direct pointer node blocks} containing the \as{lba} of the data, and \textit{indirect node blocks} containing the identifier of the associated direct pointer node block, which is unique for each direct node. Therefore, a change in a data block requires the direct node block to be updated, to point to the new \as{lba} of the data, and a change in the NAT to point the indirect node block to the new direct node block, solving the wandering tree problem. 

To avoid metadata updates being written directly after a change, F2FS uses the \af{lmu} to buffer metadata and node block updates in memory before being flushed to the flash storage. A similar policy is the \af{libu}~\cite{oh2010optimizations}, in which only the block node updates are buffered in memory before being flushed. Additional data structures for metadata in F2FS include the \af{sit} for information on the segment usage and the bitmap to identify valid and invalid blocks, and a \as{ssa} which includes further information on segments such as the information on owners of data and node blocks. Note that F2FS requires randomly writable space for metadata, as it is not written in the log, delegating data management to the \as{ftl}. 

Given that file systems are written in units of blocks, smaller I/Os arising from minor file challenges, such as microwrites, are undesirable due to the added \as{wa}. Therefore, file systems employ \textit{write buffering} by caching the changes in memory, and writing to storage when needed. However, this comes at the drawback that if the system crashes, the data cached in memory is lost. For this file systems provide the possibility to directly write to storage with \textit{direct I/O} or to explicitly flush caches to the storage device with an \textit{fsync()} call. To provide failure recovery in the case of system crashes or power loss, file systems commonly employ methods such as \textit{journaling}, in which operations are logged in a journal in addition to being written to the storage. Therefore, if the system crashes replaying the journal will result in reaching the prior valid file system before the system failure. File systems with this journaling feature are referred to as \textit{journaling file systems}. 

A similar approach with less overheads is using \af{cow}, commonly also referred to as \textit{shadow paging}, in which a copy of the original data is made on writing, and the copy is modified. Only upon successful completion is the metadata, pointing to the valid data block, changed to present the new copy. This can additionally be done atomically and simplifies the crash recovery, as the metadata state will always be valid, such that if the copy was written but the metadata points to the old data, the write did not complete successfully and thus the original data is the valid data. While there exist more implementations for ensuring crash recovery and consistency, journaling and \as{cow} are among the most utilized approaches. F2FS utilizes \textit{checkpointing}, in which metadata including the file system status, bitmaps, inode lists, and the segment summary, are written to the \as{cp} region periodically. During a checkpoint, all data in page cache is flushed to storage and a \textit{checkpoint pack} is written, containing the metadata (\as{nat} and segment information bitmaps). 

In the case of a system crash or power loss, the file system can recover the state from the latest checkpoint, referred to as \textit{roll-back recovery} since the latest changes which are not in the checkpoint are reverted. In order to recover the latest changes, the host must call \textit{fsync()} to ensure that metadata and data are flushed from memory to the device. This recovery is referred \textit{roll-forward recovery} since it recovers the state past the latest stable checkpoint. F2FS can only guarantee roll-forward recovery with \textit{fsync()}.

While F2FS utilizes a log-structured approach, under increased concurrency such a log becomes a bottleneck. Therefore, to provide increased performance, F2FS can switch between a single sequentially written log (\textit{normal logging}) to \textit{threaded logging}, where data is written in dirty segments instead of the log. However, while this approach provides increased logging capacity for concurrent access and avoids garbage collection, it incurs random writing. Given that during file system \as{gc}, block addresses are modified, as the cleaning moves still valid blocks to free space, however the metadata is not directly updated due to the \as{lmu} policy, F2FS is required to create a checkpoint after each segment cleaning. 


==> bak/ssd_integration.tex <==
\section{SSD Flash Integration}\label{sec:ssd_integration_evaluation}
With conventional SSDs, the FTL has full control over the underlying flash media. As a result, the possibility for file systems to fully incorporate each flash challenge is limited. However, particular design decisions in the file system aid the performance of the FTL and help leverage the flash characteristics. Therefore, this section covers the file systems that are particularly built on conventional flash-based SSDs (recall Figure~\ref{fig:flash_integration_ssd}), with an FTL exposing a conventional block interface. Table~\ref{tab:ssd_integration_comparison} shows a comparison of all file systems meeting this criteria, evaluating if the file system provides novel methods for handling of certain flash characteristics. As all file systems are log-structured file systems, which is a write optimized data structure due to its append only nature, which further inherently provides basic wear leveling by writing everything sequentially, the WL column is only marked on file systems that further extend this mechanism with additional novel methods.

\begin{table*}[!t]
    \centering
    \begin{tabular}{||p{15mm}||p{8mm}|p{15mm}|p{5mm}|p{20mm}|p{15mm}|p{5mm}|p{15mm}|p{15mm}||}
        \hline 
        & & \multicolumn{7}{|c||}{Flash Challenge} \\
        \hline
        File \newline System & Year & Read/Write \newline Asymmetry & GC & I/O \newline Amplification & Flash \newline Parallelism & WL & Software \newline Stack & I/O \newline Scheduling \\
        \hline
        \hline
        F2FS\cite{2015-Changman-f2fs} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        F2FS + SCJ\cite{2021-Gwak-SCJ} & 2021 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        SFS\cite{2012-Min-SFS} & 2014 & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
        \hline
        ReconFS\cite{2014-Lu-ReconFS} & 2014 & \xmark & \xmark & WA \& SA & \cmark & \xmark & \xmark & \xmark \\
        \hline
        URFS\cite{2020-Tu-URFS} & 2020 & \cmark & \cmark & WA & \xmark & \xmark & \cmark & \cmark \\
        \hline
        EvFS\cite{2019-Yoshimura-EvFS} & 2020 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
        \hline
        BetrFS\cite{2022-Jiao-BetrFS} & 2022 & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
        \hline
        CSA-FS\cite{huang2013improve} & 2013 & \cmark & \xmark & SA & \xmark & \xmark & \xmark & \xmark \\
        \hline
        DashFS\cite{2019-Liu-fs_as_process} & 2019 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
        \hline
        DevFS\cite{2018-Kannan-DevFS} & 2018 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark \\
        \hline
        % From here on papers added from original FS Design Considerations classification
        Max\cite{2021-Liao-Max} & 2021 & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark \\
        \hline
        SpanFS\cite{2015-Kang-SpanFS} & 2015 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark \\
        \hline
        exF2FS\cite{2022-Oh-exF2FS} & 2022 & \cmark & \cmark & WA & \cmark & \xmark & \xmark & \xmark \\
        \hline
    \end{tabular}
    \caption{Evaluated file systems for flash-based SSD integration (with conventional FTL) and the flash challenges (Section~\ref{sec:opt_flash}) the file system solves. A \cmark\hspace{0.5mm} indicates that a file system implements a mechanism to handle the particular flash challenge, however it does not indicate to what extent it is handled or how successful it is handled. If a file system does not have a name and/or it is an extension on an existing file system, the authors' names are used as the file system name. As the majority of file systems are LFS-based designs, the table indicates if the file system employs a novel method in addition to what is required of LFS. For instance, the GC column contains a \xmark\hspace{0.5mm} if the file system simply implements greedy or cost-benefit GC, and a \cmark\hspace{0.5mm} if a new GC policy or new mechanisms of managing GC are presented.}
    \label{tab:ssd_integration_comparison}
\end{table*}

\subsection{Read/Write Asymmetry}\label{sec:ssd_rw_asym}
The characteristic of flash having lower write than read performance requires that data structures for flash are write optimized. Such data structures which are optimized for write operations are referred to as \textit{write optimized indexes} (WOI). With the addition of the missing support for in-place updates on flash, the best suiting data structure for flash-based file systems is a log-based structure. As a result, all file systems discussed in this section are LFS. The nature of a LFS being append only writes accounts for the lower write performance on flash. 

However, file systems should further avoid small writes, referred to as microwrites. Particularly, as file systems write in units of blocks, which commonly are 4KiB, small writes require a full unit to be filled. The majority of file systems provide the possibility for inline data in inodes, such that the inode data, which is written regardless, has a small capacity to include data. However, this still requires that for small files inodes are directly written to flash. Therefore, several schemes that involve buffering and caching of data in memory, before flushing to the flash storage, provide increased write performance, and additionally increase overall performance.

While buffering of I/O prior to flushing to flash storage provides performance gains, buffers are often limited in size and are much smaller than the persistent storage, therefore numerous buffering and eviction algorithms exists, in particular algorithms designed for flash storage characteristics. Clean first least recently used (CFLRU)~\cite{park2006cflru} is an extension on the LRU algorithm. It splits the buffer into two segments, one as the working region in which recently accessed pages reside, which are managed in most recently used (MRU) fashion, therefore depicting the frequently accessed pages. The second region, called the clean-first region contains the less commonly accessed pages in LRU fashion. On eviction (e.g., when writing a new page and freeing space in the buffer), it first attempts to evict a clean page, rather than a dirty page from the clean-first region, as this does not require a flush of the dirty data to the flash storage, and only resorts to evicting dirty pages as last resort. Flash aware buffer (FAB)~\cite{jo2006fab} is another buffering mechanism particular to flash. It organizes pages in blocks and upon eviction flushes entire blocks to the flash storage, issuing larger I/Os and aligning better to the flash erase unit. 

Similar to write optimized indexes, \textit{write optimized dictionaries} (WODs) provide increased write performance. These are implemented through data structures such as LSM trees~\cite{sears2012blsm} and $\text{B}^\varepsilon$-Trees (a write optimized version of the B-Tree). BetrFS~\cite{2022-Jiao-BetrFS} (not the original BetrFS file system but an updated, flash-optimized version) implements such a $\text{B}^\varepsilon$ as the metadata storage for indexing data. It is implemented in the Linux Kernel as a key-value store, based on TokuDB~\cite{tokudb}, which exposes a key-value addressable interface. The benefit of $\text{B}^\varepsilon$-Trees is that the nodes have a larger (2-4MiB) sequentially written log, batching updates into larger units and thus avoiding small updates. Updates are placed in the leaf nodes. Initially all updates go into the root node message log, which when full gets flushed to its child nodes, similar to the internals of LSM tree compaction. Updates are cached in the VFS page cache , and are flushed to the $\text{B}^\varepsilon$-Tree. While WODs provide optimized write performance by batching updates, read requests require reading an entire node (2-4MiB), causing small read requests to suffer from significant read amplification (\textbf{FC2}).

With the lower write performance on flash storage, CSA-FS~\cite{huang2013improve} aims to reduce the write traffic on the device by utilizing deduplication (in detail discussed in Section~\ref{sec:deduplication}). Storage often contains duplicate data (e.g., archival copies of data, or backup copies). However, this requires additional space for the same data. Therefore, CSA-FS implements deduplicaiton by calculating the MD5 digest (MD5 is a hash function applied to the input) and looks up the result in a hash table which provides the corresponding LBA of the block. If it already exists and the user requested a new file with it, the new inode simply uses the given LBA from the hash table, instead of duplicating the data again. Furthermore, for reducing the writes of semantic data (superblock, descriptors, bitmaps, and tables), CSA-FS uses delta-encoding (discussed in detail in Section~\ref{sec:compression_encoding}) for updates. Delta-encoding finds the difference of the data and its original data, storing only the changes that are made instead of the entire new data. Both of these mechanisms, deduplication and delta-encoding reduce the amount of data that is written, which in turn provides a longer lifetime of the flash storage (\textbf{FC5}) and enhances space amplification by minimizing data that is written (\textbf{FC3}).

\subsection{Garbage Collection}
A significant challenge of flash storage is the garbage collection overheads. While the FTL is running garbage collection, the file system can experience significant performance drops and suffer from high and unpredictable tail latency. While the FTL is in control of managing the garbage collection, there are methods for improving the GC required by minimizing the amount of data that is being invalidated, and thus lowering the required erasing. URFS~\cite{2020-Tu-URFS} aligns the data allocation unit for large files to the erase unit, allowing files to be erased as a single unit, limiting required GC. However, as the erase unit of flash can be several MBs, this is only applicable to large files.

\subsubsection{Data Grouping}
Similar to F2FS, an effective method for this is the grouping of data based on the access frequency. This grouping allows to separate the hot data, which is frequently accessed and overwritten from cold data, which is infrequently modified. In the scenario where hot and cold data is not separated and resident in the same block, the frequently modified hot data will repeatedly invalidate the block, which will cause the garbage collection to have to move the valid data to a new free space. This cold data is then again resident in a block with hot data, which will be invalidated, requiring to move the cold data again. This constitutes to significant garbage collection, where cold data is constantly moved. Jung et al.~\cite{jung2010process} propose a novel hot/cold data grouping, which unlike simplistic data grouping that classifies based on the access frequency, that further periodically classifies based on the process ID.

SFS~\cite{2012-Min-SFS} implements such a data grouping to separate hot and cold data into different segments, by utilizing an eager data grouping on writing during segment cleaning. Emphasizing that lazily grouping data on segment cleaning fails to account for the asymmetric write performance of SSDs, SFS utilizes a comprehensive grouping classification mechanism. SFS assigns a hotness to blocks and to groups, which represent a collection of blocks with similar temperature. Using an \textit{iterative segment quantization} algorithm, based on k-means clustering~\cite{hartigan1979algorithm}, SFS partitions the segments into a number of groups to which blocks are assigned based on the quantization model, that finds the center of groups through iterative search as the data in segments and their hotness changes. Such a model allows to provide a better distribution of hotness in the particular data.

Shafaei et al.~\cite{2016-Shafaei-WA_extent_temp} identify that the majority of hot/cold data grouping methods fail to account for the accuracy in the hot/cold grouping mechanism, as well as relying on an individual classification of each LBA, making the management of increasingly larger flash storage difficult. Therefore, an extent-based temperature identification mechanism is proposed, based on the density-based stream clustering problem~\cite{jia2008grid,chen2007density,forestiero2013single,isaksson2012sostream}, which is a common approach of classification in artificial intelligence and stream processing, however has not been applied to storage before. The density-based stream clustering groups/clusters data in a one dimensional space. Applying this method to storage, the one-dimensional space is the range of LBAs, and extent-based clustering splits the available space into a number of extents for a group cluster. Initially, the entire space is a single extent and is expanded and merged (merging of extents with the same group classification) as writes occur. Such a grouping allows a more detailed grouping, compared to hot/cold grouping, reducing possible garbage collection penalties. 

Numerous additional hot/cold grouping schemes exist, such as request size-based prediction scheme~\cite{chang2008hybrid}, which bases its classification on the sector size of the request. This classification is based on the assumption that write requests follow a bi-modal distribution, large number of small requests and a large number of very large requests, incorporating the tendency of file systems to incur a large number of metadata updates. A table-based classification model~\cite{hsieh2005efficient} is another mechanism that maintains a history of accesses for each LBA, allowing precise access frequency modeling for individual LBAs. This however comes at a high overhead cost, as an entry for each LBA is needed, which becomes increasingly expensive as flash storage grows. Another mechanism is the two-level LRU classification~\cite{chang2002adaptive}, which maintains two LRU lists, of which an initial LBA access stores the LBA in the first list, and a subsequent access moves it to the next list, which is referred to as the hot list. Therefore, only LBAs in the hot list are considered to be frequently accessed. 

Multiple bloom filters (MBF)~\cite{jagmohan2010write,park2011hot} uses bloom filters to identify if an LBA is hot. Bloom filters rely on a hash function that, given an input such as the LBA, provide an output which is mapped to a bit array, and sets the bit to true. Therefore, if an LBA is accessed applying the hash function sets the respective bit in the array to true, and checking if an LBA is hot simply applies the hash function and checks if the bit is set. However, depending on the length of the array, multiple LBAs can map to the same bit location, as proven by the pigeonhole principle~\cite{ajtai1994complexity}, resulting in false positive hotness classifications for LBAs. To avoid frequent false positive classifications, MBF utilizes multiple bloom filters. Similar to MBF, Kuo et al.~\cite{kuo2006configurability} present a hot data identification method by using multiple hash functions and a hash table. Upon a write, the LBA is hashed by multiple hash function and a counter for each has function is incremented in a hash table. To check if an LBA is hot, the LBA is hashed and a configured $H$ most significant bits of the resulting hash table indicate if that the LBA is hot if they are non-zero. Multiple hash functions are used for the same reason multiple bloom filters are used in MBF, to avoid false positive classifications. Lee and Kim~\cite{2013-Lee-data_grouping_empirical_study} provide a study into comparing performance of two-level LRU, MBF, and dynamic data clustering (DAC, which are similar to the density-based stream clustering by Shafaei et al.~\cite{2016-Shafaei-WA_extent_temp}). The authors show that on the evaluated synthetic workloads DAC clustering provides the highest reduction in write amplification factor.

Instead of grouping data based on an assigned temperature, indicating the access frequency, Chakraborttii and Litz~\cite{2021-Chakraborttii-DT_LBA} propose a temporal convolutional network that predicts the \textit{death-time} of LBAs. This allows to more optimally group data based on the death-time of individual LBAs. Grouping related death-time LBA reduces the required garbage collection, as blocks containing LBAs with similar death-times are erased together, which in turn reduces the write amplification (\textbf{FC2}).

\subsubsection{Garbage Collection Policies}
While data grouping provides benefits of co-locating data based on their update likelihood, an additional essential part of garbage collection is the policy of victim selection for segments to clean. Since during garbage collection a segment to clean is required to be selected, where all still valid data in the segment is moved to a free space, selecting a victim becomes non-trivial. The common existing policies for garbage collection are greedy~\cite{2010-Bux-Greedy_GC,kawaguchi1995flash} and cost-benefit~\cite{kawaguchi1995flash,1992-Rosenblum-LFS,wu1994envy}. However, with the prior established data grouping, both of these policies fail to fully account for the hotness of groups in the victim selection.

Greedy victim selection selects the segment with the lowest utilization, whereas the cost-benefit policy selects the segment with the best cost/benefit ratio, calculated as, with $u$ being the utilization of the segment~\cite{1992-Rosenblum-LFS}
\begin{equation}
    \text{cost-benefit}=\frac{\text{free space generated}}{\text{cost}}=\frac{(1-u)*\text{age}}{1+u}
\end{equation}
where the cost is based on reading the segment (equivalent to cost 1) + writing the data in the segment (equivalent to its utilization). SFS~\cite{2012-Min-SFS} proposes the \textit{cost-hotness} policy to account for the hotness of segments instead of the segment age, better incorporating the data grouping into victim selection. Similar to the cost-benefit policy, the cost-hotness is calculated as
\begin{equation}
    \text{cost-hotness}=\frac{\text{free space generated}}{\text{cost}*\text{segment hotness}}=\frac{(1-u)*\text{age}}{2u*h}
\end{equation}
where the cost considers reading and writing the valid blocks (equivalent to $2u$) with the segment hotness. A further garbage collection policy that is based on the cost-benefit policy, is the \textit{cost-age-time} (CAT) policy~\cite{chiang1999cleaning}. It extends cost-benefit by including an erase count for each block, improving wear leveling (\textbf{FC5}).

Customizable victim selection algorithms, such as the \textit{$d$-Choice} algorithm~\cite{van2013mean}, which combines greedy selection with random selection. The tunable parameter $d$ defines the number of blocks to be selected randomly out of the $N$ total blocks. Therefore, configuring $d=1$ results in fully random victim selection, as a single block is randomly selected from the total blocks, providing effective wear leveling through randomness~\cite{2015-Yang-algebric_WA_modeling}. Configuring $d\rightarrow \infty$ selects a larger subsets of blocks to use greedy selection on, such that $d=N$ is equivalent to fully greedy victim selection, allowing to provide the lowest cleaning latency. Configuration of $d$ thus allows to define the tradeoff between wear leveling and performance. An evaluation by Yang and Zhu~\cite{2015-Yang-algebric_WA_modeling} of the algorithm shows the significance of the number of hotness tiers which are utilized and the configuration of the $d$ parameter, where a large number of hotness tiers can significantly increase the write amplification during garbage collection. 

A further drawback of segment cleaning with LFS, in particular F2FS, is that the modification of metadata during segment cleaning requires a checkpoint to be created after each segment clean. This constitutes to a significant overhead for the segment cleaning process. To avoid the excessive checkpointing after segment cleaning, \textit{segment cleaning journaling} SCJ~\cite{2021-Gwak-SCJ} adds support to F2FS to journal metadata updates made during segment cleaning, instead of creating a checkpoint. This journal is stored in a journal area, which delays the updating of the original metadata until the journal becomes large enough or the checkpointing time interval is reached. However, metadata still points to old invalid data blocks (referred to as pre-invalid blocks), which requires that data only be invalidated once the metadata is updated by the segment cleaning journal. Therefore, SCJ implements an adaptive checkpointing that evaluates the cost of checkpointing to flush the metadata updates and the accumulation of pre-invalid blocks, and checkpoints if its cost is lower. 

\subsection{I/O Amplification}
As the main cause of write amplification is the incurred garbage collection, mechanisms to reduce garbage collection consequently reduce the write amplification. However, additional mechanisms exist to reduce the write amplification. In particular, as the smallest unit of write in flash storage is a single page, smaller writes still require to write a full page, filling up unused space and writing more than was intended, which causes space and write amplification. While the majority of file systems aim to align inodes to the size of flash pages, such that space amplification can be avoided. File systems, such as ReconFS~\cite{2014-Lu-ReconFS} have much smaller inode size, equal to 128B, allowing to place numerous inodes in a single flash page. With such an inode size, writing each inode change directly would require to fill the flash page with unnecessary data, therefore, ReconFS implements a \textit{metadata persistent log}, in which metadata changes are logged and compacted to align with pages, and are only written back to the storage when evicted or checkpointed, in order for the file system to remain consistent.

\subsection{Flash Parallelism}
As host software has no direct access to flash storage with SSDs, the FTL implements and manages all device-level parallelism. The possibility for the host to utilize flash parallelism comes from aiding the FTL in providing large enough I/Os such that the FTL can stripe data across flash chips and channels. This combining of resources for striping of data is referred to as \textit{clustered blocks/pages}~\cite{2012-Kim-clustered_blocks}. Furthermore, clustered blocks are also erased as one, allowing for write I/Os that are aligned to a multiple of the clustered block size to invalidate blocks in parallel, helping to amortize overheads.

SFS~\cite{2012-Min-SFS} takes advantage of the achieved device-level parallelism with clustered blocks by aligning segments to a multiple of the clustered block size. During garbage collection SFS ensures that cleaning of segments which do not have enough blocks to fill the clustered block size is delayed until enough data is present. Increasing device parallelism can further be achieved by mapping operations to individual resources. DevFS~\cite{2018-Kannan-DevFS}, a direct access user-space file system, maps I/O queues to individual files, allowing concurrent file operations to submit I/Os concurrently without interfering on the I/O queue.

\subsection{Wear Leveling}
Garbage collection and the selection of garbage collection policy are major contributing factors to burning out of flash cells~\cite{2016-Verschoren-GC_impact_WL}. While file systems commonly aim to provide even wear over the flash device, especially during file system garbage collection with LFS, at the SSD integration level there is limited possibility of ensuring even wear, since the FTL makes the final decision on physical write addresses, and it also attempts to ensure even wear. However, as seen with earlier discussed file systems such as CSA-FS~\cite{huang2013improve}, flash lifetime can further be prolonged by minimizing the data write traffic through mechanisms such as deduplication and delta-encoding.

% per process stream pattern recognition to improve wear on ssd\cite{wang2013exploit} - NO ACCESS TO PAPER ON IEEE

\subsection{Minimizing the Software Stack with User-Space File Systems}
With SSDs providing significantly lower access latency, the overheads of the I/O stack on the storage becomes a major contributing factor in the performance~\cite{foong2010towards,seppanen2010high,vasudevan2012using}. Any added interrupt on the I/O path can cause significant delays~\cite{2014-Shin-OS_IO_Path}. Especially with the Kernel involvement requiring to possibly do context switches, the majority of time can be spent in the I/O stack rather than the storage retrieving the data. Therefore, research has aimed at minimizing the I/O stack and avoiding costly mechanisms.

A major contribution of this is the design of user-space file systems. These file systems run only in the user-space, as opposed to commonly used file systems (e.g., F2FS) running in Kernel space. Further benefiting from easier development, increased reliability and security by avoiding Kernel bugs and vulnerabilities, and increased portability~\cite{2015-Tarasov-User_space_fs_practicality}. The most commonly framework for building user-space libraries is FUSE~\cite{szeredi2010fuse}, however it is implemented over a Kernel module, allowing to export virtual file systems into the Kernel. However, FUSE based file systems suffer significant performance penalties, requiring more CPU cycles that file systems in Kernel space, because of it need to copy memory between user space and kernel space and overheads from the way FUSE handles requests~\cite{2019-Vangoor-Fuse_performance,vangoor2017fuse}. Furthermore, FUSE suffers from context switching~\cite{vangoor2017fuse,2019-Vangoor-Fuse_performance,rajgarhia2010performance} and inter-process communication (IPC) with the FUSE kernel module~\cite{zhu2018direct}. An existing file system in the Linux Kernel called ZUFS (zero-copy user-mode file system)~\cite{2019-Harrosh-zufs}, which is aimed at persistent memories but applicable to other devices, provides a lockless, zero-copy, user-space file system, which completes I/O requests by requesting exact data locations instead of copying data into the own address space.

A similar framework for building user-space applications with direct access to storage devices is NVMeDirect~\cite{2016-Kim-NVMe_Direct}. However, it also relies on a Kernel driver to provide enhanced I/O policies. SPDK~\cite{2017-Yang-SPDK} is another framework for building user-space storage applications, however it provides the mechanisms to bypass the Kernel and submit I/O directly to the device, by implementing a user-space driver for the storage device. Such a framework allows to build high performance storage applications in user-space, which eliminate the overheads coming from the Kernel I/O stack. Borge et al.~\cite{2019-Borge-SSD_read_variability} show with a case study on HDFS performance with SSD, that in order to leverage the capabilities of flash SSDs, direct I/O and increased parallel requests with buffered I/O are needed. 

File system as processes (FSP)~\cite{2019-Liu-fs_as_process} provides a storage architecture design for user-space file systems. The emphasis of FSP is to scale with the arrival of faster storage, and similarly to other user-space frameworks, minimize the software stack. For this it bases development on running file systems as processes, providing safer metadata integrity, data sharing coordination, and consistency control, as the process running the file system is in control of everything, instead of trusting libraries. Furthermore, FSP relies on IPC for fast communication, which unlike FUSE has a low overhead since it does not require context switching. Inter-core message passing comes at a low overhead and cache-to-cache transfers on multi-core systems can complete in double digit cycles~\cite{soares2010flexsc}. DashFS~\cite{2019-Liu-fs_as_process} is built with FSP, providing a safe user-space file system with isolation of different user processes, and efficient IPC.

URFS~\cite{2020-Tu-URFS} provides increased concurrency performance by implementing a multi-process shared cache in memory. This mechanism helps avoid contention on the storage device, and further avoids Kernel interaction. In order to guarantee permissions are valid, URFS implements an \textit{access control list} (ACL). Through the shared memory, it avoids the Kernel having to copy memory for every process, limiting Kernel overheads. A similar user-space file system that implements a shared cache for process is EvFS~\cite{2019-Yoshimura-EvFS}, which is SPDK-based. While this file system can also support multiple readers/writers in the page cache, it only supports these for a single user process. User-space frameworks often provide capabilities to either expose the storage device as a block device, which the user-space application then accesses, or build a custom block device module (e.g., with SPDK which also has default driver modules such as NVMe). For NVMe devices that support NVMe controller memory buffer management, the file system can manage parts of the device memory. DevFS~\cite{2018-Kannan-DevFS} utilize such an integration to manage the device memory for file metadata and I/O queues.

Lastly, specific operating systems, such as Arrakis~\cite{peter2014towards,peter2015arrakis}, which exposes storage devices as virtualized storage and allows user-space I/O requests to bypass their kernel. However, it requires the Kernel to be updated to enforce storage protection, which makes detailed discussion of its methods out of the scope of this literature study.  

\subsection{I/O Scheduling}
Given that particular I/O patterns can have degrading affects on the SSD performance, such as mixing read and write operations, as they share resources on the device, including the mapping table and ECC engine, and furthermore possibility invalidating the cached data in the SSD RAM. Similarly, mixing I/O operations with different block sizes can result in increased fragmentation~\cite{2020-Tu-URFS}. As the Linux Kernel relies on a submission and completion queue for I/O, user-space frameworks such as SPDK and NVMeDirect provide more flexibility for user-space file systems to design different queues, depending on the requirements. URFS~\cite{2020-Tu-URFS} utilizes this possibility to create adaptive queues that can better optimize I/O submissions to the device. Based on the workload characteristics URFS dynamically creates flexible I/O queues (e.g., group by size, read/write operation) to increase SSD performance. In addition to better utilizing SSD performance, this mechanism also enhances dealing with the read/write asymmetry of flash (\textbf{FC1}).

Conventionally I/O requests are submitted asynchronously, where the application submits the I/O to the Kernel, which then submits it to the device and waits for an interrupt from the storage device when the I/O has completed. While this allows the application to continue different work and frees the CPU, it was originally designed for slow storage devices, where I/O completion takes significant time. Especially, as the Kernel asynchronous block I/O layer adds a substantial overhead, with fast storage devices, such as NVMe SSD, polling provides better performance. With polling, the I/O is submitted synchronously, avoiding the Kernel asynchronous block I/O layer, and spin-waits for the I/O to complete. Faster storage devices can complete I/O requests significantly faster, where the overheads of spin-waiting are lower than the overheads of asynchronous I/O. Furthermore, a large penalty of asynchronous I/O is the need for context switching, when interrupts happen, as well as causing cache and translation lookaside buffer (TLB) pollution~\cite{yang2012poll}. Yang et al.~\cite{yang2012poll} provide a quantitative comparison of asynchronous and synchronous, interrupt and polling, I/O scheduling.

With the possibility for asynchronous I/O to merge and reorder requests, the Linux Kernel implements several schedulers, such as \textit{NOOP}, \textit{deadline}, and \textit{CFQ}~\cite{sun2014exploring,pratt2004workload,moallem2008study,heger2010linux}. NOOP being the least intrusive scheduler only merges I/O request, but does not reorder them, which is beneficial on devices such as OCSSD and ZNS that require consecutive LBAs. Son et al.~\cite{2015-Son-Optimizing_FS} showcase the benefits of merging random write requests, regardless of contiguity of the LBAs, in order to better enhance performance with fast storage devices. Deadline adds to NOOP by utilizing merging and reordering, however also applies a deadline for each I/O request to ensure requests are submitted to the device eventually. Two separate queues, one for read requests and an additional one for write requests are utilized, which are both ordered by the deadline of the request. Another scheduler variant of deadline exists, called \textit{mq-deadline}, which is aimed at multi-queue devices, such as NVMe SSD. CFQ (completely fair queueing) implements a round-robin based queue that assigns time slices to each in order to prevent starvation and provide fairness. While these are some of the common schedulers in the Linux Kernel, various more schedulers exist~\cite{2019-ubuntu_wiki_io_schedulers}.

Such scheduling configuration begs the question on which scheduler is best suited for file systems on flash storage. Sun et al.~\cite{sun2014exploring} provide a study into several possible scheduler configurations for file systems on SSD, with an emphasis on incorporating the storage energy consumption, however we do not discuss energy consumption aspects in this literature review. Yu et al.~\cite{yu2014optimizing} present similar study of the I/O path and block I/O system optimizations, however over SCSI and SATA instead of NVMe, which is why we do not include its details here. Nonetheless, several of the findings are applicable to all applications submitting I/O to storage devices. The merging of read I/O requests in synchronous I/O provides beneficial performance gains, and similarly the merging of write I/Os in asynchronous I/O shows performance gains. However, optimal I/O scheduling for storage devices is an obstacle that has yet to be overcome.


==> conclusion.tex <==
\section{Conclusion}
The move from \as{hdd} to flash \as{ssd}, has been one of the most fundamental shifts in the storage hierarchy. The increased performance of flash \as{ssd} over \as{hdd}, capable of achieving single several GB/s bandwidth with millions of \as{iops}, however required adaptations in the software stack, changing the design of file systems and storage software to integrate with these devices. In this literature study we evaluate the current state of file systems for flash storage devices, how these file systems design to align with introduced flash characteristics, and how the integration of flash storage into file system design has affected storage stack design.

Iterating the considered research objectives for this literature study, the main findings show that \textbf{(RQ1)} NAND flash storage has influenced file system design particular in the aspects of no in-place updates and requiring erasing of flash blocks prior to rewriting data. Resulting file system design has largely focused on \as{lfs}, aligning with the sequential write requirement of the storage, however introducing complexity through required \as{gc} and effective \as{wl} across the flash. We present numerous effective methods, showing that dealing with \as{gc} through efficient \as{gc} policies, write buffering, reducing write traffic, and effective data grouping techniques is a widely adopted and research field. Numerous file systems present different approaches and policies. Furthermore, the increased performance of flash storage is largely dependent on exploiting the internal parallelism, of which favored methods involve data striping across parallel flash units and increasing the parallelism. An additional major change is the reduction of the software stack, which was originally designed for slower storage devices (\as{hdd}), and is showing its shortcomings in integrating flash storage and providing and scalable and performant storage systems. User-space file systems, bypassing a significant amount of the software stack layers are increasingly popular adoption for eliminating software stack layers.

The main challenges of integrating with NAND flash storage \textbf{(RQ2)} revolve around dealing with introduced \as{gc} overheads, limiting its introduced \as{io} amplifications, exploiting the possible parallelism capabilities of flash storage, and lowering the storage software stack overheads. We showcase the different methods adopted by flash file systems for dealing with these challenges, evaluating developments of the past decades on how to effectively integrate flash storage in storage software design. While we emphasize the design for file systems, the majority of the evaluated methods are applicable to the larger spectrum of storage software. We therefore include methods from \as{ftl} design, which have not yet been adopted by file system designers, providing the possible methods for future flash optimized file system design.

Given the increasing rise in adoption for flash storage, and the introduction of new flash-based storage devices and interfaces, future implications of flash storage \textbf{(RQ3)} provide a promising ground of better integrating the flash storage with software, leveraging the increased performance capabilities further. Through new interfaces exposing a larger amount of flash characteristics, the host software gets an increasing level of possibility to design application specific flash management, integrating the application design with flash management. Future storage software developments are likely to continue integrating the closer integration of flash storage into host storage software design, optimizing the flash utilizing for full leveraging of flash performance. We envision the semantic gap between storage hardware and software to slowly decrease over time, allowing to build more performant, efficient, reliable, and responsible storage systems. Such efforts align with the grand challenges of future storage~\cite{2022-compsys-manifesto}, particularly with increasing demand of systems due to the digitalization of the world, and the push towards a more sustainable future. 


==> discussion.tex <==
\section{Discussion}
With the multitude of methods for dealing with flash integration, there are several that are of key concern. In particular, \as{gc} and mechanisms of dealing with \as{gc} have shown to be applicable, and enhance other flash integration challenges. However, there is no panacea for solving all flash integration challenges. Incorporating a particular mechanism causes difficulty of integration with other flash challenges. Especially, depending on the level of integration of flash storage, there is limited possibility of integrating particular mechanisms. Therefore, the closer integration is largely necessary in order to more optimally integrate flash, however coming ad the additional flash management complexity. Resulting in finding of the tradeoff between the level of management from the file system, or host software, where a higher level of management allows the application to more optimally be designed for the flash, and the required complexity and applicability of the file system. Generic file systems working on numerous integration levels, require more generic interface management, limiting the customizability of it. 

While we discussed methods for integrating flash at the file system and software level, there exist other flash-based storage devices and interfaces that can provide adapted integration for host software. Such include a flash design that allows multi-write coding of the flash pages in order to reduce erasing and garbage collection~\cite{jagmohan2010write}. With multi-write coding, the bits in a flash page can be reprogrammed, without a required erase, to a bit value higher than it currently is. As an erase on a flash page resets the bits to a 1, any bit that is set to a 0 can be set to a 1 without requiring to erase the entire flash page. Similar flexible storage interfaces such as \as{ocssd}, and Prism-SSD~\cite{2022-Shen-PrismSSD} provide increased possibility for flash management. Such interfaces aim at reducing the mismatch between storage devices and their interfaces, which allow to better integrate flash characteristics, and the devised flash integration challenges, into file system and storage software design.

\section{Future Predictions}
Clear trends in the storage community are becoming apparent, focusing on eliminating the hiding of flash management idiosyncrasies, and exposing its characteristics to the host. Therefore, allowing the host to integrate and optimize the software for its access patterns with increased knowledge of the underlying storage device characteristics~\cite{bjorling2017lightnvm,2012-asplos-moneta,kang2014multi,bhimani2017enhancing,2010-Josephson-DFS,2021-Bjorling-ZNS}. As stated in the CompSys Manifesto~\cite{2022-compsys-manifesto}, ''the grand challenge in storage systems is to combine heterogeneous storage layers, leveraging their programmability and capabilities to deliver a new class of cost, data, and performance efficiency for all kinds of applications''. Reducing the semantic gap between storage hardware and software must be a driving concern in future storage system design, leveraging the existing hardware capabilities and enhancing integration for more efficient, effective, sustainable, and reliable storage systems.

The recent addition of \af{zns} \as{ssd}~\cite{2021-Bjorling-ZNS,2022-Tehrany-Understanding_ZNS}, standardized in the \as{nvme} 2.0 specification~\cite{2022-nvme-spec}, similarly provides host the control over \as{gc} management on the storage device, and matches the interface to the underlying flash characteristics. It exposes flash storage through a number of \textit{zones} which must be written sequentially, and must be erased prior to being overwritten~\cite{2021-ZNS-ZBD_docs}. Leveraging such device interfaces allows the file system development to partially take control of on-device operations. In addition to eliminating duplicate work of file system and \as{gc} on the device, where the increased coordination provides better performance capabilities, the higher-level control of the file system allows it to apply its data knowledge, such as particular grouping based on file characteristics, without a significant increase in complexity through the zone interface of \as{zns} \as{ssd}. Such integration presents a well defined interface aimed at eliminating the interface mismatch between flash storage and storage software, leaving a plethora of possibility for storage software to enhance flash integration. Exposing more storage device control to the host system, particularly in the configuration of \as{zns}, allows not only data placement to be better integrated into storage software, but furthermore allows to to fully utilize the parallel units of the storage device. With \as{zns} devices, the parallelism unit of the storage device is clearly defined~\cite{2022-Bae-ZNS_Parallelism}, and can be leveraged by the storage software.

With \as{zns} having been a recent proposal at the time of writing, file system support is limited. F2FS provides capabilities to run on \as{zns} \as{ssd}~\cite{2021-Bjorling-ZNS}, however requires an additional randomly writable device for its metadata. ZenFS~\cite{2021-Bjorling-ZNS,2022-zenfs-git} is a domain specific file system for \as{zns} that provides the backend for the RocksDB key-value store. Therefore, currently there does not exist a purely \as{zns} based file system, which we envision to be a prospect of future developments in storage. We imagine likewise interfaces to appear, exposing an increasing level of flash hardware characteristics to the host software in order to better coordinate and integrate the storage. Similarly, we envision future efforts to aim at further decreasing the semantic gap between storage hardware and software, and leverage a higher degree of coordination across storage software/hardware layers. Similarly, the gain in popularity of user-space based applications, as we discussed in \cref{sec:user_space_fs}, presents prominent possibility for future development and limiting Kernel involvement, which has become an increasing overhead in the software stack. Therefore, we furthermore picture an increase in user-space applications, and particularly file systems.



==> failure.tex <==
\section{Failure Consistent Operations}\label{sec:failure_consistency}
An important aspect of file systems is to ensure that in the case of power failure or system crashes, the file system state and its data remain in a consistent state, and can be recovered upon a subsequent mount. Most commonly used mechanisms for ensuring this are journaling, CoW, and checkpointing. However, journaling suffers from having to write data twice, once for the metadata log and again for the data log, to ensure full consistency~\cite{pillai2017application,xu2016nova}, also referred to as the double-write problem~\cite{2018-Kannan-DevFS}. Therefore, file systems commonly only provide metadata consistency by logging only the metadata. Furthermore, power failure is a concern with flash storage, as it has capacitors that can flush parts of the on-device memory buffers, unless more expensive capacitors are used that can flush the entirety of the memory buffers. In the case of power failure, partially written data or metadata updates can result in the file system being in an inconsistent state.

While checkpointing, \as{cow}, and other consistency mechanisms aim to handle these failures and provide recovery after failure, other methods exist for providing interfaces that eliminate partial operations. Particularly, the design of flash storage, such as the available \as{oob} space of pages, provides beneficial options for such implementations. \cref{tab:consistency} depicts the methods for ensuring failure consistency with flash storage, and the file systems implementing such methods.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        Atomic Writes (\cref{sec:atomic_writes}) & \cite{2021-Qin-Atomic_Writes,cheon2017exploiting,f2fs-atomic-write} \\
        \hline
        Transactions (\cref{sec:transactions}) & \cite{2022-Oh-exF2FS} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Failure consistency mechanisms to for flash storage, and the respective file systems that implement a particular mechanism.}
    \label{tab:consistency}
\end{table}


% Nowhere else are these mentioned, removed prior section on mount time
% O1FS~\cite{2014-Hyunchan-O1FS} decreases the crash recovery time, when remounting a file system, by dividing the storage space into working areas, where all file system data is going into one working area at a time. This implies that superblock and additional metadata is duplicated for each working area, however on a system crash it requires only to check the latest working area and recover the file system from it. This allows to significantly decrease the required complexity for recovering from the system crash, due to the smaller region that is required to be scanned. A similar decrease of recovery time at mount time for LFS is achieved by recording file system states for faster metadata checks, which is presented by Wu et al.~\cite{wu2006efficient}. It relies on maintaining an in-memory record, called the \textit{log record manager}, of the file system records, including the important data structures to the file system. When persisting the log records onto flash, the file system can upon remounting more quickly check the log records to reconstruct the file system state, with the present data structures in the log record, instead of reconstructing them.

\subsection{Atomic Writes}\label{sec:atomic_writes}
A possible method for ensuring that operations are not completed partially is through atomic writes. This is important to file systems as an update of data requires its respective metadata to also be updated. Failure of one should result in the other not being completed. A variety of flash devices support atomic writes through mechanisms such as in \as{ftl}~\cite{ouyang2011beyond} and through user-programmable \as{ssd}~\cite{Seshadri-2014-Willow}, however it can also be implemented in the file system itself. F2FS supports multi-block atomic writing, which allows updating multiple file system blocks in a single \textit{ioctl} command~\cite{2021-Qin-Atomic_Writes,cheon2017exploiting,f2fs-atomic-write}. ReconFS~\cite{2014-Lu-ReconFS} provides multi-page atomicity by using a flag in each page to indicate if it is valid. This is achieved by writing a 1 in the head of the last flash page of the metadata updated, and all other pages have a 0 in the head. Therefore, in the case of power failure, when the file system is reconstructed, any metadata pages in between two pages with a 1 in the head (depicting two ending page updates) are valid pages, and in the case when the log has no page with the flag set to 1, the update failed and all pages after the last 1 flag are invalid. 

Similarly, Qin et al.~\cite{2021-Qin-Atomic_Writes} showcase the utilization of the \as{oob} area on flash with \as{ocssd} in order to store metadata for ensuring data integrity in the No-Barrier File System (NBFS), which is extending F2FS. The file system uses \af{dnchain} to ensure consistency measurements. \as{dnchain} is a linked list of all the blocks in an atomic operation, which are stored through a pointer in the \as{oob} space, thus representing a linked list of pointers in an atomic operation. The last block in the \as{dnchain} points to itself to indicate the end of the linked list and the atomic operation. Furthermore, each block contains a checkpoint version, allowing the recovery after a failure to traverse the \as{dnchain} and identify if an invalid checkpoint version number is present, which indicates a failed atomic operation. As the initial writing of journal or \as{cow} is done in memory and later flushed to the flash storage, mechanisms such as failure-atomic \textit{msync()}~\cite{park2013failure}, provide atomicity in such operations.

\subsection{Transactions}\label{sec:transactions}
A similar approach for ensuring consistency is to use transactions, enforcing an ``all-or-nothing`` mechanism that either writes all data or no data at all if there are any failures during the transaction. Transactional support can stem from transactional block devices, such as TxFlash (Transactional Flash)~\cite{prabhakaran2008transactional} LightTX with embedded transaction support in the flash storage FTL~\cite{2013-Lu-LightTX,lu2015high}, and similar block device implementations that expose transaction support~\cite{huang2012bvssd,kang2013x,2013-Coburn-SSD_Txs}. Additions to file systems can similarly implement transactions for block devices without transaction support. exF2FS~\cite{2022-Oh-exF2FS} is an extension on F2FS that provides it with support for transactions. In order to support transactions, exF2FS implements several features. Firstly, with transactions relying on either all updates being present or no updates at all, the \as{gc} policy is adapted such that the \as{gc} module cannot reclaim flash pages that contain data from a transaction that is in progress. If such a page is garbage collected without the transaction having finished, it can be recovered and thus violates the all-or-nothing mechanism. 

For this, exF2FS implements \textit{shadow garbage collection}, which prohibits the \as{gc} module from using pages involved in pending transactions. Secondly, in order to provide large scale transactions with multiple exF2FS maintains \textit{transaction file groups}, which are kernel objects that identify the set of files involved in a transaction. Lastly, it implements \textit{stealing}, which allows dirty pages of pending transactions to be committed to the flash storage, however do not allow it to be garbage collected until the transaction completed. This mechanism is referred to as \textit{delayed invalidation and relocation record}, and the process of allowing dirty pages to be evicted in uncommited transactions is referred to as \textit{stealing}~\cite{2022-Oh-exF2FS}.

\subsection{Flash Failures}
Flash failures are another important aspect of file systems on how they manage and recover from these failures. A study into file system reliability showed that 16\% of injected faults resulted in an unmountable file system, which furthermore was not fixable by a file system checker~\cite{2020-Jaffer-SSD_Errors}. Especially, as the density of flash is increasing, where more layers of NAND is stacked on top of each other, resulting in a decrease in the flash reliability~\cite{meza2015large}. While flash employs \as{ecc} to handle correcting of data, there are errors that are not fixable such as the \textit{uncorrectable bit corruption}~\cite{boboila2010write,belgal2002new,brand1993novel}, which can be caused by flash wear, read disturbance, and other factors~\cite{2020-Jaffer-SSD_Errors}. We do not go into detail of flash induced errors, for a detailed evaluation on flash errors recovery mechanisms consult \cite{2020-Jaffer-SSD_Errors,gatla2018towards}. Jaffer et al.~\cite{2020-Jaffer-SSD_Errors} provide several guidelines for file systems to enhance reliability with flash errors, including adding more sanity checks, especially of metadata, and finding better tradeoffs between checksums and the checksum granularity, where a large checksum granularity can result in significant data loss if it has an unrecoverable invalid checksum, and a small checksum adds overheads on the needed space and performance. While file system checkers aim to solve a degree of faults, they are no panacea to fixing corrupted file systems~\cite{gatla2018towards} and require better failure handling in the file system itself.


==> flash_challenges.tex <==
\section{Challenges of Flash Storage Integration}\label{sec:flash_challenges} 
While \as{ssd} uses the same block interface that is used with \as{hdd}, flash has different characteristics that software must account for to better integrate flash storage. This section details the challenges that arise from integrating flash storage into systems, providing the guidelines along which we dictate the bottom up view of changes in the host storage software stack, up to the file system. We define the challenges to account for the characteristics of flash storage, as well as enhance its integration into host systems. In the case of \as{ssd} devices, these challenges often largely depend on the underlying \as{ftl}, as it is making the final decision, independent of what data placement the host implements, however aiding the \as{ftl} can increase the performance. Embedded devices provide a higher level of host data placement by eliminating the \as{ftl} and directly attaching flash chips to the motherboard. Each challenge is assigned a specific identifier with the \af{fic}, in order to refer back to the specific challenge throughout this literature review.

\noindent \textbf{\as{fic}1: Asymmetric Read and Write Performance.} On flash storage write operations require more time than read operations~\cite{stoica2009evaluating,2022-intel-p,chen2009understanding}, making it important for software to limit write operations. Particularly, frequent small writes that are smaller than the allocation unit, referred to as \textit{microwrites} incur significant performance penalties, and should be avoided where possible.

\noindent \textbf{\as{fic}2: Garbage Collection (GC).} While the \as{ftl} hides the flash access constraints from host applications, providing seemingly in-place data updates, it adds the cost of performing garbage collection to free up space. \as{gc} overheads have unpredictable performance penalties for the host system~\cite{2015-Kim-SLO_complying_ssds,2014-yang-dont_stack_log_on_log}, resulting in large tail latency~\cite{2013-Dean-tail_at_scale}. Dealing with, and aiming to minimize required garbage collection for the flash device is a key challenge in integrating flash storage.

\noindent \textbf{\as{fic}3: \as{io} Amplification.} Due to the characteristics of flash avoiding in-place updates of flash pages, writes often encounter \af{wa}. With this the amount of data that is written on the flash storage is larger than the write that is issued by the host system. For example a 4KiB issued write may increase to 16KiB being written on the device, due to possible garbage collection requiring to copy data, resulting in a \as{wa} factor of 4x. \as{wa} furthermore adds to an increase in wear on the flash cells~\cite{2013-Lu-SSD_WA_Lifetime}. \af{ra} similarly is caused by requiring to read a larger amount of data than is issued in the read \as{io} request. \as{ra} most commonly happens when reading metadata in order to locate data, thus requiring an additional read of metadata on top of the request read \as{io} request for the data. This is most often inevitable, as all data requires metadata for management, however this should be kept to a minimum at application-level. Furthermore, minimization of \as{wa} is more important than \as{ra}, since write requests have a higher latency than read requests, and writing has a more significant impact on the flash storage, resulting in increased flash wear. While read requests also incur wear on the flash cell, called read disturbance~\cite{2015-Liu-Read_leveling}, it is not as significant as for write requests. 

% \textbf{\as{fic}2.} \textit{Auxiliary Write Amplification (AWA):} Similar to on-device write amplification, applications can also encounter write amplification, which is referred to as auxiliary write amplification~\cite{2014-Leonardo-NVMKV}. An example of this happens when the application is writing more data than was intended, when for instance required to run application-level garbage collection.

% \textbf{\as{fic}4.} \textit{Auxiliary Read Amplification (ARA):} Similar to read amplification and auxiliary write amplification, when an application is required to read more data than the read size issued. Such an amplification is not caused by the FTL but rather represents application introduced amplification. An example of this is an application required to issue more read requests to locate data, in for instance a file system required to read inodes prior to locating valid data blocks. Therefore, a 4KiB read for a data block requires multiple inode (data directory and file inode) to be located.

\noindent \textbf{\as{fic}4: Flash Parallelism.} With the various possible levels of parallelism on flash storage devices (discussed in \cref{sec:bg_flash_ssds}), exploiting of the various possibilities requires software design consideration to aligning with these. Although the \as{io} scheduling of on-device parallelism, such for channel-level parallelism, is responsibility of the \as{ftl} (on devices at \as{ssd} integration level), the \as{ftl} implements particular parallelism, given that the host \as{io} requests aligning with the possibility of parallelizing the request, such as with large enough \as{io}s to stripe across channels and dies. Embedded device and custom flash integrations have more possibility to manage flash device parallelism at the host software level.

\noindent \textbf{\as{fic}5: Wear Leveling (WL).} Given limited program/erase cycles for flash cells, even wear over the entire device is required to ensures that no specific areas of the device are burnt out faster than others. Similar to flash parallelism, this largely depends on the flash integration level, as the \as{ftl} at the \as{ssd} integration level ensures \as{wl}, however embedded flash integration and custom flash integration is required to place more significance on ensuring even wear across the flash cells. Strongly related to prior flash integration challenges, wear is commonly a result of \as{gc}, which in turn increases the \as{io} amplification, and particularly the  \as{wa} and \as{ra}~\cite{2014-Desnoyers-Analytic_Models_SSD,2009-Hu-WA_SSD}. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/storage_stack.pdf}
    \caption{Visual overview of the storage stack in the Linux Kernel. Adapted from~\cite{mishra2017BigDataStorage,fischer2017linux}.}
    \label{fig:storage_stack}
\end{figure}

\noindent \textbf{\as{fic}6: \as{io} Scheduling.} As \as{ssd} ships with integrated firmware to expose the flash storage as a block/sector addressable storage device, integration into the current software stack is seamless. \cref{fig:storage_stack} shows the integration of a flash \as{ssd} into the Linux Kernel storage stack. Since flash storage devices are significantly faster than prior storage technologies, such as \as{hdd}, the storage software stack becomes the dominating factor in \as{io} latency~\cite{2010-Caulfield-Moneta,2012-Caulfield-Fast_User_Space_Access}. As is visible in \cref{fig:storage_stack}, the block \as{io} layer implements various schedulers with different functionality. Providing a ranging degree of optimizations for \as{io} requests, such as varying scheduling policies and merging of \as{io} requests, or possible reordering, specific configurations are favorable to increase performance with flash storage. Particularly the utilization of multiple queues, with multiple software and hardware dispatch queues (visible in the blk-mq configuration of the block \as{io} layer), allows better exploitation of flash storage capabilities, and avoids certain Linux Kernel overheads. Furthermore, evaluating mechanisms that reduce the latency of \as{io} operations, and particularly write \as{io} operations.

\subsection{Log-Structured File System - F2FS}\label{sec:bg_lfs}
A ubiquitous approach of managing persistent storage devices is with file systems, providing the familiar file and directory interface for organizing storage. The lack of in-place updates on flash pages, enforcing sequential writes, makes \af{lfs}~\cite{1992-Rosenblum-LFS,2006-Konishi-Linux_LFS,seltzer1993implementation} a suitable file system design. The design of \as{lfs} revolves around writing data as a log, appending new data sequentially on the storage device. Similar to the \as{ftl}, as data is being updated in a \as{lfs}, the log contains an increasing amount of no longer needed data, requiring \as{gc} to free occupied space. In this section, we describe the de-facto standard \as{lfs} for flash-based storage devices, \af{f2fs}~\cite{2015-Changman-f2fs}. A plethora of additional flash-based file systems exists, however these are commonly based on top of \as{f2fs} or adapt \as{f2fs} mechanisms.

\begin{figure*}[!ht]
    \centering
    \subfloat[]{\includegraphics[width=0.4\textwidth]{figs/f2fs-zone-blind-allocation.pdf}\label{fig:f2fs-zone-blind-allocation}}\hfill
    \subfloat[]{\includegraphics[width=0.59\textwidth]{figs/f2fs-zone-aware-allocation.pdf}\label{fig:f2fs-zone-aware-allocation}}
    % \vspace{-0.3cm}
    \caption{(a) \textit{zone-blind allocation} suffering from inadequate physical data separation, (b) \textit{zone-aware allocation} utilizing larger zones to ensure physical data separation.}
    \label{fig:f2fs-erase-unit-align}
\end{figure*}

With \as{f2fs} being a \as{lfs}, it writes data sequentially, in several different logs. \as{f2fs} maintains six concurrently writable logs, of which three are for data of different lifetime classifications (hot/warm/cold), and the remaining three are for node data of different lifetime classifications. Internally, \as{f2fs} utilizes a data allocation unit referred to as a \textit{block}, of 4KiB, in which blocks are allocated in the different logs. Consecutive blocks are collected into a 2MiB \textit{segment}, of which one or multiple segments are further grouped into a \textit{section}, and sections are combined into a \textit{zone}. The goal of sections is to align with the \as{gc} unit of the underlying \as{ftl}, whereas a zone is utilized in order to avoid sections in different zones to be mapped into the same on-device erase unit by the \as{ftl}, which would defeat the purpose of section grouping. Such mapping is illustrated in \cref{fig:f2fs-zone-blind-allocation}, which depicts an example of \textit{zone-blind allocation}, where data for different files, with different lifetime classification, are mapped into different sections, however align to the same zone. As a result the data mapping may not be far enough, resulting in the \as{ftl} to write the data to flash pages within the same erase unit. With \textit{zone-aware allocation}, illustrated in \cref{fig:f2fs-zone-aware-allocation}, the zone serves the purpose to provide a large enough separation between particular sections, such that the \as{ftl} similarly separates the written flash pages for the different file data into different erase units. 

Such a mapping is provided by \as{f2fs}, with the option of configuring the number of sections in a zone, which depending on the erase unit of the device ensures adequate physical data separation. However, by default \as{f2fs} is configured to contain a single segment in each section and a single section in a zone. As \as{f2fs} is log-structured, over time it contains valid and invalid blocks, similar to the \as{ftl}, and must therefore also run \as{gc}. In \as{f2fs} the process of \as{gc} is done at the unit of a section, where valid blocks in the containing segments are read and written to a free space, prior to the segments in the section being freed. \cref{fig:f2fs-layout} shows the layout of segments, sections, and zones (on the right half of the figure), alongside the metadata structures which \as{f2fs} requires. We discuss each of the essential structures throughout this section, except the superblock which is similar to other file system superblocks and contains essential file system metadata for the host system to be able to mount the file system.

\begin{figure}[!t] 
    \centering
    \includegraphics[width=0.49\textwidth]{figs/f2fs-layout.pdf}
    \caption{On-device layout of \as{f2fs} data. Adapted from F2FS~\cite{2015-Changman-f2fs}.}
    \label{fig:f2fs-layout}
\end{figure}

Similar to other file systems, a file in \as{f2fs} is managed through an \af{inode}, and contains all the file information, including the file specific metadata on creation time, access permissions, file name, and more. \cref{fig:f2fs-inode} shows the inode of F2FS. For identifying the data blocks of the associated file, inodes contain a fixed number of direct pointers to the addresses of the file data. Since inodes are allocated in blocks, they can often contain inline data of the file, if the file data fits in the available space of the inode. To be able to locate larger files, inodes utilize \textit{multi-level indexing}, where indirect pointers point to blocks containing further pointers to more data blocks. There are several levels of indirection, where a \textit{single indirect} pointer points to one block containing pointers to the blocks which contain the data. For example, with a block size of 4KiB and 4B addresses, a single indirect pointer can store 1024 addresses, which each point to 4KiB of data, giving an addressable space of $4KiB*1024=4MiB$ (plus the number of direct pointers in the inode). Increasing the level of indirection further increases the maximum file size of the file system, where nowadays file systems most commonly provide up to three levels of indirect pointers, allowing in the example of 4KiB block size and 4B addresses, a maximum file size of $4KiB*(1024+1024^2+1024^3)=4TiB$ (plus the number of direct pointers). While multi-level indexing is a popular implementation in file systems, other solutions such as \textit{extents} exist, utilizing a single pointer to a contiguous number of blocks for the file. This approach decreases the metadata size by requiring only a single pointer, however it is more difficult of finding a contiguous number of blocks for allocating space for the file.

\begin{figure}[!t] 
    \centering
    \includegraphics[width=0.4\textwidth]{figs/f2fs-inode.pdf}
    \caption{The \as{inode} structure of \as{f2fs}. Retrieved from F2FS~\cite{2015-Changman-f2fs}.}
    \label{fig:f2fs-inode}
\end{figure}

File systems commonly utilize tree-based indexing data structures in order to achieve a worst case time complexity of $\mathcal{O}(\log{}n)$ for locating of inodes or other metadata, compared to a log based approach requiring to scan the entire log, corresponding to $\mathcal{O}(n)$ worst case time complexity. However, a tree-based data structure introduces the Wandering Tree Problem~\cite{bityutskiy2005jffs3}, where if a leaf node is modified, its new block is written at the end of the log, giving it a new block address. Its parent node must also be modified to point to this new address, requiring a new block to be written for it at the end of the log, giving it a new block address. These changes to the parent node are propagated all the way up the tree to the root node. Therefore, F2FS manages metadata for segment allocations in a \af{nat}. It divides allocated blocks into three types; \textit{inode blocks} that contain the metadata for the file from the \as{inode}, \textit{direct pointer node blocks} containing the \as{lba} of the data, and \textit{indirect node blocks} holding unique identifiers to the direct node blocks. Therefore, a change in a data block requires the direct node block to be updated, to point to the new \as{lba} of the data, and a change in the \as{nat} to point the identifiers of the direct node blocks to the new direct node block address. The indirect node block does not require any changes, as it stores identifies of the direct node blocks, which are modified in the \as{nat}, therefore solving the wandering tree problem. To avoid metadata updates being written directly after a change, F2FS uses the \af{lmu} to buffer metadata and node block updates in memory before being flushed to the flash storage. Additional data structures for metadata in F2FS include the \af{sit} for information on the segment usage and the bitmap to identify valid and invalid blocks, and a \af{ssa} which includes further information on segments such as the information on owners of data and node blocks. Note that F2FS requires randomly writable space for metadata, as it is not written in the log, delegating data management to the \as{ftl}. 

Given that file systems are written in units of blocks, smaller \as{io}s arising from minor file challenges, such as microwrites, are undesirable due to the added \as{wa}. Therefore, file systems employ \textit{write buffering} by caching the changes in memory, and writing to storage when needed. However, this comes at the drawback that if the system crashes, the data cached in memory is lost. For this file systems provide the possibility to directly write to storage with \textit{direct \as{io}} or to explicitly flush caches to the storage device with an \textit{fsync()} call. To provide failure recovery in the case of system crashes or power loss, file systems commonly employ methods such as \textit{journaling}, in which operations are logged in a journal in addition to being written to the storage. Therefore, if the system crashes replaying the journal will result in reaching the prior valid file system before the system failure. File systems with this journaling feature are referred to as \textit{journaling file systems}. 

A similar approach with fewer overheads is using \af{cow}, commonly also referred to as \textit{shadow paging}, in which a copy of the original data is made on writing, and the copy is modified. Only upon successful completion is the metadata, pointing to the valid data block, changed to present the new copy. This can additionally be done atomically and simplifies the crash recovery, as the metadata state will always be valid, such that if the copy was written but the metadata points to the old data, the write did not complete successfully and thus the original data is the valid data. While there exist more implementations for ensuring crash recovery and consistency, journaling and \as{cow} are among the most utilized approaches. F2FS however utilizes \textit{checkpointing}, in which metadata including the file system status, bitmaps, inode lists, and the segment summary, are periodically written to the \af{cp} region. During a checkpoint, all data in page cache is flushed to storage and a \textit{checkpoint pack} is written, containing the metadata (\as{nat} and segment information bitmaps). In the case of a system crash or power loss, the file system can recover the state from the latest checkpoint, referred to as \textit{roll-back recovery} since the latest changes which are not in the checkpoint are reverted. In order to recover the latest changes, the host must call \textit{fsync()} to ensure that metadata and data are flushed from memory to the device. This recovery is referred \textit{roll-forward recovery} since it recovers the state past the latest stable checkpoint. F2FS can only guarantee roll-forward recovery with \textit{fsync()}.

To minimize the file system \as{gc} overheads, \as{f2fs} groups data based on the modification frequency. It achieves this by assigning a temperature (hold/warm/cold), and pre-defines classifications for direct node blocks, as these are frequently modified, and indirect node blocks are classified as cold, as these are not frequently modified. To further extend this mechanism, F2FS maintains six different logging zones for the different temperature assignments (hot/warm/cold for nodes and file data). In addition to node block classifications, data blocks are classified in several ways. Firstly, the host can provide a hint on the lifetime of a file, upon which the data blocks in the file are grouped according to this hint. The Linux Kernel provides five different lifetime hints, ranging from \textit{short} to \textit{extreme}, which \as{f2fs} reduces to the three groups it has. Secondly, \as{f2fs} by default assigns files with particular extensions, such as media data (e.g., .mp3, .mp4, .gif), with cold lifetime classification, as media is commonly written just once and then only read again. The default extensions to classify are written in the \as{f2fs} superblock as formatting time. \as{f2fs} reclassifies the lifetime based on the access frequency, where file data which is being moved during \as{gc}, meaning it has not been modified up to the time of \as{gc} and is therefore likely to not be modified frequently in the future, is classified as cold. Similarly, if the number of dirty blocks in a segment exceeds a threshold (16 by default), the corresponding inode is marked as hot. 

In F2FS \as{gc} is referred to as \textit{cleaning}, and is run periodically (called \textit{background cleaning}) or when space is needed (called \textit{foreground cleaning}). The cleaning policies implemented in F2FS are greedy~\cite{2010-Bux-Greedy_GC,kawaguchi1995flash}, \af{cb}~\cite{kawaguchi1995flash,1992-Rosenblum-LFS,wu1994envy}, which are used for foreground and background cleaning respectively, and \af{at}~\cite{2020-f2fs-age_threshold,menon1998age}. Greedy victim selection selects the segment with the lowest utilization, whereas the \as{cb} policy selects the segment with the best cost/benefit ratio, calculated as~\cite{1992-Rosenblum-LFS}, with $u$ being the utilization of the segment
\begin{equation*}
    \text{cost-benefit}=\frac{\text{free space generated}}{\text{cost}}=\frac{(1-u)*\text{age}}{1+u}
\end{equation*}
where the cost is based on reading the segment (depicted by the 1), plus writing the data in the segment (depicted by the utilization). \as{at} based \as{gc} is disabled by default and aims at avoiding that the same section is continuously being selected during \as{gc} if it always provides the best victim. To achieve this, a minimum lifetime is set (by default 7 days), which must be exceeded in order to be selected as the victim.

While F2FS utilizes a log-structured approach, under increased concurrency such a log becomes a bottleneck. Therefore, to provide increased performance, F2FS can switch between a single sequentially written log (\textit{normal logging}) to \textit{threaded logging}, where data is written in dirty segments instead of the log. However, while this approach provides increased logging capacity for concurrent access and avoids garbage collection, it incurs random writing. Similarly, \as{f2fs} provides the option for \af{ssr}, in which it uses invalid blocks in a segments instead of running foreground \as{gc}. While this approach avoid running \as{gc} it generates random write patterns. Given that during file system \as{gc}, block addresses are modified, as the cleaning moves still valid blocks to free space, however the metadata is not directly updated due to the \as{lmu} policy, F2FS is required to create a checkpoint after each segment cleaning.

\subsection{Flash Integration Organization}
With the different possible levels for integration of flash storage (recall \cref{fig:flash_integrations}), and while mechanisms for solving flash integration challenges are often applicable at various integration levels, several of the mechanisms we present require deeper integration of flash storage, levering increased control, in order to be implemented. For instance, the incorporation of the various levels of on-device parallelism is not directly possible at the \as{ssd} integration level, as the \as{ftl} controls the parallelism on the physical device. The custom and embedded level flash integration provide the host with more possibility to manage these. In order to separate the possibility of mechanisms to be implemented with a particular flash integration level, \cref{tab:integration_levels} provides a classification of each evaluated file system in this literature study to the respective integration level. During the evaluation we present the different mechanisms to solve a \as{fic}, and indicate which file systems utilize these. Therefore, when considering the feasibility of a mechanism for a particular flash integration consult this table to see its applicability. Note that file systems are not limited to the classification we provide, as for instance file systems designed for \as{ssd} flash integration also work on some embedded flash integration. However, we utilize only a single classification for each file system to avoid confusion. Exceptions are made only in specific cases where an existing file system is adapted for a different flash integration level.

\begin{table}[!t]
    \centering
    \begin{tabular}{||p{35mm}|p{35mm}||}
        \hline 
        Integration Level & File Systems \\
        \hline
        \hline
        \as{ssd} Flash Integration & \cite{2015-Changman-f2fs,2021-Gwak-SCJ,2012-Min-SFS,2014-Lu-ReconFS,2020-Tu-URFS,2019-Yoshimura-EvFS,2022-Jiao-BetrFS,jannen2015betrfs,huang2013improve,2019-Liu-fs_as_process,2018-Kannan-DevFS,2021-Liao-Max,2015-Kang-SpanFS,2022-Oh-exF2FS,rodeh2013btrfs} \\
        \hline
        Custom Flash Integration & \cite{kawaguchi1995flash,josephson2011direct,2020-Wu-DualFS,2018-Rho-Fstream,dubeyko2019ssdfs,lee2014refactored,2019-Lu-Sync_IO_OCSSD,2016-Lee-AMF,2018-Yoo-OrcFS,2016-Zhang-ParaFS,2021-Qin-Atomic_Writes} \\
        \hline
        Embedded Flash \newline Integration & \cite{2006-Lim-NAND_fs,hunter2008brief,2009-Sungjin-FlexFS,2008-Jung-ScaleFFS,woodhouse2001jffs,park2013enffis,nahill2015flogfs,schildt2012contiki,2015-Park-Suspend_Aware_cleaning-F2FS,2009-Zuck-NANDFS,2009-Park-Multimedia_NAND_Fs,2007-Hyun-LeCramFS,2021-Ji-F2FS_compression,2011-Park-Multi_NAND,manning2010yaffs,aleph2001yaffs,manning2002yaffs,engel2005logfs,2008-Kim-DFFS,park2006flash,2020-Yang-F2FS_Framentation,2022-Lee-F2FS_Address_Remapping,2011-Lim-DeFFS,2014-Hyunchan-O1FS,2022-Zhang-ELOFS,2020-Zhang-LOFFS,kim2006mnfs,2009-Tsiftes-Coffee_FS} \\
        \hline
    \end{tabular}
    \caption{Classification on the flash integration level utilised for the file systems evaluated in this literature study.}
    \label{tab:integration_levels}
\end{table}

We divide the discussion of mechanism by the \as{fic} for which the evaluated study presents a novel solution. This implies that mechanisms that solve multiple \as{fic} are discussed in detail in the first section they appear in, however are also mentioned in all latter sections for the \as{fic} that the mechanism solves. Therefore, each \as{fic} section contains a table of the respective mechanisms presented to solve that particular \as{fic}, along with a reference to the corresponding section of its detailed discussion.



==> flash_parallelism.tex <==
\section{Flash Parallelism}\label{sec:flash_parallelism}
With the capabilities of flash storage relying largely on increased parallelism, several existing mechanisms are leveraging these. Depending on the level of flash integration, different mechanisms are possible, where at the \as{ssd} integration the host has not control over the possible physical parallel utilization of flash, as the \as{ftl} controls this, however deeper flash integration at the custom and embedded levels provide more possibility. \cref{tab:flash_parallelism} depicts the various mechanisms to aid the utilization of flash parallelism and exploit the physical characteristics of flash.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        Aligning the Allocation Unit (\cref{sec:align_alloc}) & \cite{2020-Tu-URFS,2009-Park-Multimedia_NAND_Fs} \\
        \hline
        Clustered Allocation \& Striping (\cref{sec:clustered_alloc}) & \cite{2012-Min-SFS,dubeyko2019ssdfs,2018-Yoo-OrcFS,2016-Zhang-ParaFS,2011-Park-Multi_NAND,manning2010yaffs,aleph2001yaffs,manning2002yaffs} \\
        \hline
        Concurrency (\cref{sec:concurrency}) & \cite{2021-Liao-Max,2018-Kannan-DevFS,2015-Kang-SpanFS,2019-Lee-Parallel_LFS,2016-Lee-AMF,2016-Zhang-ParaFS} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Mechanisms for file systems to exploit flash parallelism capabilities, and the respective file systems that implement a particular mechanism.}
    \label{tab:flash_parallelism}
\end{table}

\subsection{Clustered Allocation \& Striping}\label{sec:clustered_alloc}
As host software has no direct access to flash storage with \as{ssd}, the \as{ftl} implements and manages all device-level parallelism. The possibility for the host to utilize flash parallelism comes from aiding the \as{ftl} in providing large enough \as{io}s such that the \as{ftl} can stripe data across flash chips and channels. This is achieved with \textit{clustered blocks/pages}~\cite{2012-Kim-clustered_blocks}, where blocks or pages on different units (such as blocks on different planes) are accessed in parallel. The \as{ftl} can possibly stripe data across these clustered blocks, given that the \as{io} request is large enough to fill the clustered unit. Such a mechanism aligns with prior discussed aligning of the allocation unit (\cref{sec:align_alloc}) to a physical unit to reduce \as{io} amplification, such as making the file system segment unit a multiple of the flash allocation unit. SFS~\cite{2012-Min-SFS} takes advantage of the achieved device-level parallelism with clustered blocks by aligning segments to a multiple of the clustered block size. During garbage collection SFS ensures that cleaning of segments, that do not have enough blocks to fill the clustered block size, is delayed until enough data is present.

SSDFS~\cite{dubeyko2019ssdfs} utilizes the custom flash integration to map data allocation of segments to the unit of a \af{peb}, where the \as{peb} is split over the parallel unit on the device, such as previously mentioned parallel erasing of flash blocks over channels. Therefore, utilizing \as{peb}s over the parallel unit allows striping writes into a segment over the varying channels, increasing the device parallelism. In order to achieve this, \as{io} requests have to be large enough such that they can be striped across the channel and fill the \as{peb}s mapped to the segment. For this, SSDFS utilizes aggressive merging of \as{io} requests to achieve the larger \as{io}s that can be striped across the parallel units (solving \textbf{\as{fic}7}). Instead of merging \as{io} requests, OrcFS~\cite{2018-Yoo-OrcFS} increases its file system allocation unit to a \textit{superblock} (not to be confused with the file system superblock), which represents a set of flash blocks. These flash blocks are then split over the parallel units of the flash storage for increased parallelism.

The large allocation unit however introduces increased \as{gc} overheads, and block-level striping has lower performance than page-level striping~\cite{2016-Zhang-ParaFS}. Therefore, ParaFS~\cite{2016-Zhang-ParaFS} implements a 2-D allocation scheme, with page-level striping over the flash channels, where striping is also based on the data hotness, hence having a 2-dimensional allocation scheme. Different groups are assigned for the hotness levels, where writes are issued to the corresponding hotness group striped over the flash channels. Several other file systems implement variations of striping across different parallel units on flash storage~\cite{2011-Park-Multi_NAND,manning2010yaffs,aleph2001yaffs,manning2002yaffs}. These mechanisms are also present in the design of storage applications, such as key-value stores~\cite{zhang2017flashkv,wang2014efficient}.

\subsection{Concurrency}\label{sec:concurrency}
Similar to increasing the data allocation unit, concurrency is a mechanism to exploit the flash parallelism. \as{lfs} design relies on a single append point at the head of the log, in the simplistic implementations, depending on methods such as locking to ensure only one write is issued at the log head. This has a significant impact on the performance where other \as{io}s are idle while a single \as{io} completes. F2FS however suffers from severe lock contention overheads, where the performance of the multi-headed logging is nearly fully deprecated due to the serialization of data updates~\cite{2021-Liao-Max}. In particular, as data has to be written persistently before inode and other metadata can be written. Furthermore, F2FS suffers from contention of the in-memory data structures, for which it uses reader-writer semaphores for read and write operations from the user (termed \textit{external \as{io} operations}), and reader-writer locks for writing of checkpoints and other metadata (termed \textit{internal operations}). As lock counters are shared among all cores, cache coherence adds a significant overhead that increases with more cores. Max~\cite{2021-Liao-Max} extends F2FS to increase the concurrency scalability with three main modifications.

Firstly, in order to eliminate cache coherence overheads, it introduces a \af{rps} that uses a per-process counter. Coordination between external and internal operations are ensured by the scheduler with a scheduler assisted \as{io} consensus. Secondly, the shared data structures in memory are partitioned by the inode, such that concurrent accessing does not require locking on parts of the radix tree, but instead on an \as{inode} basis. Lastly, it utilizes multiple independent logs, called a \af{mlog}, which are accessed concurrently. The different between \as{mlog} and multi-headed logging in F2FS is that atomic data blocks are mapped to the same \as{mlog}, eliminating the need to ensure concurrency control across different logs. Ordering for persistence, ensuring data blocks are written before metadata, is delegated to the recovery mechanism using a global versioning number in each inode to identify ordering across \as{mlog}s, and recover the most recent version number in case of a system crash. These mechanisms eliminate much of the needed concurrency control, which sequentialised major parts of operations and hindered multicore scalability.

With this increased concurrency capabilities, can the file system issue more \as{io} requests to the device, allowing to leverage a higher degree of on-device parallelism. Similarly, DevFS~\cite{2018-Kannan-DevFS} utilizes the parallel capabilities by exploiting the high number of \as{io} queues supported by \as{nvme}. It maps \as{io} queues to individual files, allowing single file operations to submit \as{io}s concurrently without interfering on the \as{io} queue, therefore increasing the per-file concurrency as well. Likewise to the concept of \as{mlog}, SpanFS~\cite{2015-Kang-SpanFS} maps files and directories to different \textit{domains}, such that individual domains can be accessed in parallel. Such methods have a higher lock granularity, where concurrency below the lock granularity is not possible, as a single process is holding the lock. Therefore, instead of holding locks for individual inodes or files, preventing concurrent writing to the same inode or file, Lee et al.~\cite{2019-Lee-Parallel_LFS} extend F2FS to utilize \af{rl}, in which ranges of a file are locked, and different ranges can be written concurrently. Therefore, it provides the possibility for intra-file parallelism. 

ALFS~\cite{2016-Lee-AMF}, exploits the flash parallelism by mapping consecutive file system segments to the flash channels and utilizing different \as{io} queues for each flash channel. Similarly, ParaFS~\cite{2016-Zhang-ParaFS} implements \textit{parallelism-aware scheduling}, which also maintains different \as{io} queues for each channel. However, it extends this concept by using a \textit{dispatching phase} and a \textit{request scheduling phase}. The dispatching phase optimizes write \as{io}s with a scheduling to the respective channels based on the utilization of the channel, such that the least utilised channels receives more requests. All requests are assigned a weight, which indicates their priority in the queue, where read requests weight is lower than that of write requests, because of the asymmetric performance of flash storage. During the request scheduling phase the scheduler assigns slices to the read and write/erase operations in the individual queues, such that if the time from the slice of a read operation is up and the queue contains no other read requests, a write or erase is scheduled, based on a fairness formula that incorporates the amount of free space in the block and concurrently active erase operations on other channels. This allows to minimize the erase operations on the flash, giving always free channels to utilize and maintain a fair schedule between write and erase operations.



==> gc.tex <==
\section{Garbage Collection}\label{sec:gc}
A significant challenge of flash storage is \as{gc} overheads having unpredictable performance penalties for the host system~\cite{2015-Kim-SLO_complying_ssds,2014-yang-dont_stack_log_on_log}, resulting in large tail latency~\cite{2013-Dean-tail_at_scale}. Dealing with, and aiming to minimize required garbage collection for the flash device is a key challenge in integrating flash storage. Naturally, as flash storage does not provide in-place updates, data is written in a log-based fashion, sequentially in the flash blocks. Therefore, over time as data is overwritten, the blocks contain an increasing number of invalid pages that must be erased to free space. However, as the block also contains valid data, and the erase unit is a block, the still valid pages are moved to a new block, such that the old black can be erased. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.55\textwidth]{figs/fragmentation.pdf}
    \caption{Illustration of single file fragmentation on the storage over time, as parts of file data are overwritten and, due to the \as{lfs} design new data is appended at the head of the log.}
    \label{fig:fragmentation}
\end{figure}

In a \as{lfs} updates to file data are written at the head of the log, resulting in the parts of the file that are updated to be located in a different flash block than the parts of the original file data. Furthermore, \as{gc} causes file data to moved around the storage space as well, resulting in scattering of parts of files, referred to as \textit{fragmentation}. Figure~\ref{fig:fragmentation} shows the resulting fragmentation for several files that occurs over time from file updates and \as{gc}. Fragmentation results in increased read time, due to files being in non-contiguous regions, and introduces increased garbage collection overheads due to the failed grouping of data. Ji et al.~\cite{2016-Ji-Framgentation_empirical_study} show an empirical study on fragmentation in mobile devices, identifying that fragmentation introduces performance degradation due to increased \as{io} requests, and it further produces increased pressure on caching. The effects on caching are due to increased difficulty of prefetching data, since it no longer is in contiguous physical ranges, but scattered throughout the physical space. Therefore, prefetching cannot bring correct data into the caches, resulting in an increase in cache misses. 

In addition to increased \as{io} requests for reading and rising cache pressure, increased garbage collection is caused when frequently modified files or file fragments, referred to as the \textit{hot data}, are in the same block as rarely accessed files, referred to as the \textit{cold data}. When hot data is modified, its flash pages are invalidated. Once enough flash pages in a block are invalidated, it can be erased. However, if it is co-located with cold data, the cold must be copied to a free space, as it is still valid. If this cold data is then again co-located with hot data, the modifications of the hot data cause the block to be cleared during \as{gc}, which requires the cold data to be moved again. Therefore, co-locating hot and cold data in the same physical erase unit results in significant \as{gc} increase due to the unnecessary moving of the cold data.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        Reducing Write Traffic (\cref{sec:reduce_write_traffic}) & \cite{huang2013improve,2011-Lim-DeFFS,woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,ning2011design,2009-Zuck-NANDFS,2022-Lee-F2FS_Address_Remapping} \\
        \hline
        Aligning the Allocation Unit (\cref{sec:align_alloc}) & \cite{2020-Tu-URFS,2009-Park-Multimedia_NAND_Fs} \\
        \hline
        Data Grouping (\cref{sec:data_grouping}) & \cite{2006-Lim-NAND_fs,2022-Zhang-ELOFS,2020-Zhang-LOFFS,2015-Changman-f2fs,2018-Rho-Fstream} \\
        \hline
        \as{gc} Policies (\cref{sec:gc_policy}) & \cite{2012-Min-SFS,2018-Yoo-OrcFS,2021-Gwak-SCJ,2015-Park-Suspend_Aware_cleaning-F2FS} \\
        \hline
        Coordinating the Software Stack Layers (\cref{sec:software_stack}) & \cite{2020-Wu-DualFS,2016-Zhang-ParaFS,2016-Lee-AMF,lee2014refactored} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Mechanisms for file systems to deal with \as{gc} overheads from flash storage, and the respective file systems that implement a particular mechanism.}
    \label{tab:gc}
\end{table}

Reducing the write traffic to the storage device, an effective method to handle the asymmetric flash performance (see \cref{sec:reduce_write_traffic}), is a solution to minimize fragmentation and reduce possible future \as{gc} overheads. However, additional mechanisms are required for effective \as{gc} management. With fragmentation being a significant contribution to increased garbage collection, avoiding it is a key objective to reducing garbage collection overheads. Fragmentation is classified into three different types~\cite{2007-Sato-defrag}. Firstly, \textit{single file fragmentation}, where data in a single file is dispersed over the storage (as is shown in Figure~\ref{fig:fragmentation}). Secondly, \textit{relevant file fragmentation}, where files that are relevant to each other and should be grouped together are split over the storage, such as co-locating hot and cold data in the same erase unit. Lastly, \textit{free space fragmentation}, where the file system has a large amount of small free space, because of deletion of dispersed small files. The cause of fragmentation occurring over time is referred to as \textit{file system aging}~\cite{smith1997file}. While several tools exist that implement \textit{defragmentation}~\cite{hahn2017improving,f2fs_defrag_tool,park2021fragpicker}, additional mechanism can be utilized to avoid fragmentation and \as{gc} overheads. \cref{tab:gc} depicts the mechanisms for file systems to deal with and minimize garbage collection overheads. The process of countering the different types of fragmentation is commonly referred to as \textit{storage gardening}~\cite{2020-Kesavan-Fragmentation,2019-Kesavan-Storage_Gardening}, and for file system development various aging tools exist in order to generate real-world file system workloads and simulate file system aging~\cite{2019-Conway-FS_aging,2018-Kadekodi-Geriatrix}. 

\subsection{Aligning the Allocation Unit}\label{sec:align_alloc}
\as{gc} is a result of having to move valid blocks in the erase unit to a free space, in order erase the flash block. While data grouping allows to align the validity inside the block, such that blocks are likely to be updated within close proximity, multiple files may be co-located in the same block. Therefore, a similar method is to align the allocation unit of data blocks for a single file to the erase unit, resulting in only a single file being located in a block. Such a mechanism is implemented in URFS~\cite{2020-Tu-URFS}, which aligns the data allocation unit for large files to the flash erase unit, allowing files to be erased as a single unit, limiting required \as{gc}. However, as the erase unit of flash can be several hundreds MBs, resulting in significant over-allocation for small files, it makes such a mechanism only beneficial with large files. NAMU~\cite{2009-Park-Multimedia_NAND_Fs} similarly showcases a file system that aligns its content with the requirement of large files. Focused on the multimedia domain, where files have the particular characteristics of rarely being modified, and if removed all file data blocks are erased in one unit, \as{gc} in NAMU is done at the granularity of a file. In addition to improving on \as{gc}, the memory requirements for mapping tables are also minimized. For generic file systems that vary in file characteristics, \af{ars}~\cite{2020-Yang-F2FS_Framentation} minimizes the issue of over-allocating space by allocating in a smaller unit of 2MB (a single segment). File data is written to the space until it is exhausted, upon which a new segment is allocated. While this does not map entire files to the flash erase unit, it allows writing of file data sequentially for each segment, eliminating fragmentation to a degree. 

\subsection{Data Grouping}\label{sec:data_grouping}
A key circumvention method for fragmentation relies on grouping of related data. Most commonly this is applied in the type grouping data by its access and modification frequency into hot and cold data, however other less commonly used groupings based on \textit{death-time prediction} exist~\cite{2021-Chakraborttii-DT_LBA}. Commonly more classifications than simply hot and cold are utilized for more effective grouping. A plethora of methods for grouping data in such a way have been proposed, which we split by its application type into several groups.

\subsubsection{Data Type Grouping}
Common write patterns in storage systems follow a bi-modal distribution, where many very small write requests and a numerous very large write requests are issued~\cite{chang2008hybrid}. This stems from the fact that small changes are caused by metadata updates, which occur the most frequently, whereas large changes are file updates. Given that metadata is more likely to be updated frequently, separating metadata from data improves on required garbage collection. Specifically, since metadata is often updated even if the data is not updated, for example in scenarios where the file attributes (access time, permissions, etc.) are updated, or the file is moved. Therefore, based on the request size, the data can be classified to be metadata and be grouped accordingly. F2FS also groups based on the data type, where metadata is considered to be always hot data, which is implemented by similar file systems~\cite{2006-Lim-NAND_fs}.

Dividing of file system data is similarly applied in ELOFS~\cite{2022-Zhang-ELOFS,2020-Zhang-LOFFS}, which splits the flash storage two partitions, where a directory partition contains the data of directory entries, and a data partition contains the file system data, which is compacted with the inodes. Jung et al.~\cite{jung2010process} propose the addition of classifying data based on the \af{pid}, as a process is likely to generate similar access patterns and data types throughout its lifetime, classifying by the \as{pid} allows to indirectly infer a data type. A similar data type separation is implemented by Fstream~\cite{2018-Rho-Fstream}, for which the authors modify ext4~\cite{cao2007ext4} and xfs~\cite{sweeney1996scalability} to map different operations to different streams on a stream \as{ssd}. Ext4Stream, the modified ext4 to support streams, maps different metadata operations to different streams, including the journal writes for consistency, the inode writes, as well as different streams for the directory blocks and the bitmaps (inode and block). Furthermore, it utilizes different streams that can be created for different files and for different file extensions. The goal of such streams is to map particular files, such as LOG files for key-value stores for example to a particular stream, separating its access patterns from that of other files and file system data. Similarly, the modified XFStream utilizes different streams for the log, inodes, and specific files.

\subsubsection{Dynamic Grouping}\label{sec:dynamic_grouping}
While grouping is an effective method for minimizing \as{gc}, they rely on static definition on classification targets for the number of hot/cold degrees to classify to. Shafaei et al.~\cite{2016-Shafaei-WA_extent_temp} identify that the majority of hot/cold data grouping methods fail to account for the accuracy in the hot/cold grouping mechanism, as well as relying on an individual classification of each LBA, making the management of increasingly larger flash storage difficult. Therefore, Shafaei et al.~\cite{2016-Shafaei-WA_extent_temp} propose an extent-based temperature identification mechanism. It is based on the density stream clustering problem~\cite{jia2008grid,chen2007density,forestiero2013single,isaksson2012sostream}, which is a common approach of classification in artificial intelligence and stream processing, however has not been applied to storage before. The density-based stream clustering groups data in a one dimensional space as the data arrives, hence its applicability for stream processing. 

Applying this method to storage, the one-dimensional space is the range of \as{lba}s, and extent-based clustering splits the available space into a number of extents to group by. Initially, the entire space is a single extent and as writes occur the extent is split into smaller extents with different classifications. Over time as more writes are issued, extents are expanded and merged (merging of extents with the same classification). Such a grouping allows a more detailed grouping due to the increase in classification targets, compared to binary hot/cold grouping. However, an evaluation by Yang and Zhu~\cite{2015-Yang-algebric_WA_modeling} on a configurable garbage collection policy, where the number of hotness classification targets is evaluated, shows that various hotness classification targets can significantly increase the write amplification during garbage collection. 

\subsubsection{\as{lba} Hotness Classification}\label{sec:lba_classification}
Different to grouping data based on its type, hotness can be classified on the \as{lba} based on its access frequency. The naive approach at modeling hotness for each \as{lba} is with table-based classification model~\cite{hsieh2005efficient}. This however comes at a high overhead cost, as an entry for each LBA is needed, which becomes increasingly expensive as flash storage grows.  Therefore, a more non-trivial method is based on two-level \as{lru} classification~\cite{chang2002adaptive}, with two LRU lists. Upon an initial \as{lba} access, the \as{lba} is stored in the first list, and a subsequent access moves it to the next list, which is referred to as the \textit{hot list}. Therefore, if an \as{lba} is in the hot list, it is considered to be frequently accessed. 

A different approach is implemented by \af{mbf}~\cite{jagmohan2010write,park2011hot}, which uses bloom filters to identify if an \as{lba} is hot. Bloom filters rely on a hash function that, given an input such as the \as{lba}, provide an output which is mapped to a bit array, and sets the bit to true. Therefore, if an \as{lba} is accessed, applying the hash function sets the respective bit in the array to true, and checking if an \as{lba} is hot simply applies the hash function and checks if the bit is set. However, depending on the length of the array, multiple \as{lba}s can map to the same bit location, as proven by the pigeonhole principle~\cite{ajtai1994complexity}, resulting in false positive hotness classifications for an \as{lba}. To avoid frequent false positive classifications, \as{mbf} utilizes multiple bloom filters at the same time. With multiple bloom filters, the same amount of arrays exist, applying all bloom filter hash functions to the \as{lba}, and setting the respective bit in each of the arrays. As a result, collisions on all bloom filter hash functions are less likely, minimizing the possibility for false positives.

Similar to \as{mbf}, Kuo et al.~\cite{kuo2006configurability} present a hot data identification method by using multiple hash functions and a hash table. Upon a write, the \as{lba} is hashed by multiple hash functions, and a counter for each hash function is incremented in a hash table. To check if an \as{lba} is hot, the \as{lba} is hashed and a configured $H$ most significant bits of the resulting hash table indicate if the \as{lba} is hot if they are non-zero, as the counter is increased on accesses the most significant bits are only non-zero if the \as{lba} is frequently accessed. Multiple hash functions are used for the same reason multiple bloom filters are used in \as{mbf}, to avoid false positive classifications. Lee and Kim~\cite{2013-Lee-data_grouping_empirical_study} provide a study into comparing performance of two-level \as{lru}, \as{mbf}, and \af{dac}, which are similar to the density-based stream clustering by Shafaei et al.~\cite{2016-Shafaei-WA_extent_temp} (discussed in the prior \cref{sec:dynamic_grouping}). The authors show that on the evaluated synthetic workloads \as{dac} provides the highest reduction in write amplification factor, which in turn leads to a decrease in \as{gc} overheads.

Unlike all prior approaches basing classification on the access frequency directly to identify hotness, Chakraborttii and Litz~\cite{2021-Chakraborttii-DT_LBA} propose a temporal convolutional network that predicts the \textit{death-time} of an \as{lba}, based on modification history. This allows to more optimally group data based on the death-time of individual \as{lba}, which has been shown to be an effective grouping mechanism~\cite{2017-He-SSD-Unwritten-Contract}. Grouping related death-time LBA reduces the required garbage collection, as blocks containing \as{lba}s with similar death-times are erased together, which in turn reduces the write amplification (solving \textbf{\as{fic}3}).

\subsection{Garbage Collection Policies}\label{sec:gc_policy}
While data grouping provides benefits of co-locating data based on their update likelihood, an additional essential part of garbage collection is the policy of victim selection for segments to clean. Since during garbage collection a segment to clean is required to be selected, where all still valid data in the segment is moved to a free space, selecting a victim becomes non-trivial. With the importance of data grouping with hotness for effective \as{gc}, conventional \as{gc} policies, such as greedy and cost-benefit lack their inclusion. SFS~\cite{2012-Min-SFS} proposes the \textit{cost-hotness} policy to account for the hotness of segments instead of the segment age, better incorporating the data grouping into victim selection. Similar to the cost-benefit policy (recall \cref{sec:bg_lfs}), the cost-hotness is calculated as
\begin{equation*}
    \text{cost-hotness}=\frac{\text{free space generated}}{\text{cost}*\text{segment hotness}}=\frac{(1-u)*\text{age}}{2u*h}
\end{equation*}
where the cost considers reading and writing the valid blocks (equivalent to $2u$) with the segment hotness. A further \as{gc} policy that is based on the cost-benefit policy, is the \af{cat} policy~\cite{chiang1999cleaning}. It extends cost-benefit by including an erase count for each block, improving wear leveling (solving \textbf{\as{fic}5}).

The majority of \as{gc} policies have a fixed algorithm, limiting configuration possibility. The \textit{$d$-Choice} algorithm~\cite{van2013mean} is a configurable \as{gc} policy that combines greedy selection with random selection. The tunable parameter $d$ defines the number of blocks to be selected randomly out of the $N$ total blocks. Therefore, configuring $d=1$ results in fully random victim selection, as a single block is randomly selected from the total blocks, providing effective wear leveling through randomness~\cite{2015-Yang-algebric_WA_modeling} (solving \textbf{\as{fic}5}). Configuring $d\rightarrow \infty$ selects a larger subset of blocks to use greedy selection on, such that $d=N$ is equivalent to fully greedy victim selection, allowing to provide the lowest cleaning latency. Configuration of $d$ thus allows to define the tradeoff between wear leveling and performance. 

An evaluation by Yang and Zhu~\cite{2015-Yang-algebric_WA_modeling} of the algorithm shows the significance of the number of hotness classification targets that are utilized, and the configuration of the $d$ parameter, where various hotness classification targets can significantly increase the \as{wa} during \as{gc}. Similarly, \af{fagc}~\cite{yan2014efficient} is a \as{gc} policy that maintains an \af{uft} for each \as{lba} of a file, in order to group valid pages in the victim block based on the access frequency when these are copied to a new block during \as{gc}. This is similar to grouping hot and cold data, but at the level of \as{gc} for each \as{lba} in a file. SFS~\cite{2012-Min-SFS} implements a \as{gc} policy that accounts for data grouping, with a lower overhead of having maintaining a \as{uft} for each file. It maintains a hotness classification for each block, and combines blocks with k-means clustering~\cite{hartigan1979algorithm}, into groups with similar hotness classification. 

The \as{gc} cost of foreground cleaning in F2FS can take up to several seconds~\cite{2018-Yoo-OrcFS}, as it is not a preemptive task. Implementing preemptive scheduling in Kernel file systems is challenging, as during the preemption the Kernel has to store the file system state to continue after higher priority tasks have finished, and the state being restored when returning depicts possibly outdated data. Due to the continued writing on the file system, restoring the prior state may no longer be valid, as ongoing writes may have changed file system metadata. OrcFS~\cite{2018-Yoo-OrcFS} implements \af{qpsc}, which sets a maximum time interval $T_{max}$ (default of 100ms). After cleaning a segment it checks if the timer has expired, and if so it checks if outstanding writes are present from the host. If there are outstanding writes, the locks are released and the write is executed, and if there are no outstanding writes the next segment can be cleaned and the timer is reset. This allows any host write command to not encounter a segment cleaning overhead higher than $T_{max}$.

A further drawback of segment cleaning with \as{lfs}, in particular F2FS, is that the modification of metadata during segment cleaning requires a checkpoint to be created after each segment clean. This constitutes to a significant overhead for the segment cleaning process. To avoid the excessive checkpointing after segment cleaning, \af{scj}~\cite{2021-Gwak-SCJ} adds support to F2FS to journal metadata updates made during segment cleaning, instead of creating a checkpoint. This journal is stored in a journal area, which delays the updating of the original metadata until the journal becomes large enough or the checkpointing time interval is reached. However, metadata still points to old invalid data blocks (referred to as \textit{pre-invalid blocks}), which requires that data only be invalidated once the metadata is updated by the \as{scj}. Therefore, \as{scj} implements an adaptive checkpointing that evaluates the cost of checkpointing to flush the metadata updates and the accumulation of pre-invalid blocks, and checkpoints if its cost is lower. 

In addition to utilizing \as{gc} policies to reduce its overheads, the policy can further be used to incorporate management of fragmentation. Park el at.~\cite{2016-Park-LFS_Defragmentation} propose to use a \af{vbq} in which valid blocks are sorted during garbage collection. Typically, a victim segment in the \as{lfs} is selected for cleaning, valid data is copied to the free space at the log head, and the old segment is erased. The \as{vbq} is added such that after a victim segment is selected, it is copied into the \as{vbq}, where the blocks it contains are sorted by the \as{inode} number. Then are the valid blocks written to a new segment and the old one is erased. This sorting allows to maintain file associated blocks together based on their \as{inode} number. 

A different approach to mitigate \as{gc} overheads is to design the \as{gc} procedure such that accesses do not suffer from high tail latency when \as{gc} is running. TTFlash~\cite{2017-Yan-Tiny_tail} achieves this through several mechanisms. It implements \textit{plane-blocking GC}, which limits any resources that are blocking \as{io}s to only the affected planes on the flash. However, this leads to blocking of requests to the \as{gc} affected planes. Therefore, TTFlash implements \textit{rotating \as{gc}} that only runs at most one \as{gc} operation on a \textit{plane group}. The plane group assignment is based on the possible parallelism of the device, such as plane- and channel-level parallelism. This ensures that a plane group is never blocked for more than a single \as{gc} operation, implying that any request will not be blocked for more than one \as{gc} operation. 

On embedded devices, and in particular mobile devices, in order to save energy the device suspends all threads when not needed (e.g., when the mobile screen is turned off). This implies that all file system threads are also suspended, which means the file system cannot run the background \as{gc} during these inactive sessions. Therefore, \af{sac}~\cite{2015-Park-Suspend_Aware_cleaning-F2FS} is an addition to \as{lfs}, which is the time between the suspend initiation and the suspending of the file system threads, also referred to as the \textit{slack time}. It uses this slack time to run background \as{gc}, however it does not write any data on the flash storage, but instead selects a victim block and brings the still valid pages in the page cache and marks these as dirty. As a result, all pages in the victim block to be dirty, which allows it to be erased. This process is referred to as \textit{virtual segment cleaning}, which however is not run every time the screen is turned off, but rather based on the device utilization, which is called \textit{utilization based segment cleaning}. 

\subsection{Coordinating the Software Stack Layers}\label{sec:software_stack}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/software_stack.pdf}
    \caption{Layers in the storage software stack across which data specific knowledge decreases as \as{io} is passed downwards to the \as{ftl}, representing the semantic gap~\cite{zhang2017flashkv} with flash storage.}
    \label{fig:software_stack}
\end{figure}

The various layers in the storage software stack introduces several redundant operations, such as \as{gc} that is run in the \as{lfs} and \as{gc} run on the storage device. This duplicate work leads to significant performance impacts~\cite{2014-yang-dont_stack_log_on_log}, requiring a co-design of the storage device software and the file system. Qiu et al.~\cite{2013-Qiu-Codesign_FTL_FS} show that the co-design of \as{ftl} and the file system show benefits of reduced memory requirements for \as{l2p} mappings, and increased device parallelism that can be exploited with better file system knowledge of the storage characteristics. In addition to duplicated work, information about data characteristics are lost across the various, since in order to integrate communication across the layers, each utilizes an interface for the other layers to communicate with. However, the expressiveness of the interfaces limits the capability to communicate data characteristics across the layers, as \cref{fig:software_stack} illustrates. Applications have the highest knowledge of data characteristics, how it is best allocated on the flash and managed in order to reduce \as{gc}, however cannot forward all of this information to the file system. Similarly, the file system may group specific data together, however cannot forward this information to the block layer, and similarly the \as{ftl} may take the submitted \as{io} requests and organize these different on the flash storage. This \textit{semantic gap} between the storage device and storage software is a result of the device integrating into the existing block \as{io} interface~\cite{zhang2017flashkv}, however failing to represent the flash-specific characteristics. Such mismatch between storage device and its accessing interface, requires storage software to enhance capabilities to pass information across the layers to avoid increasing the semantic gap across the layers.

DualFS~\cite{2020-Wu-DualFS} utilizes the custom integration with \as{ocssd} to merge the garbage collection of the file system with that of the \as{ftl}, and present this scheme as \textit{global garbage collection}. ParaFS~\cite{2016-Zhang-ParaFS} implements a similar coordination of file system \as{gc} and \as{ftl} \as{gc}. A different approach taken by Lee at al.~\cite{2016-Lee-AMF} is to modify the block interface with the flash characteristics, moving responsibility directly to the file system, or other application built on top of it. The resulting interface called \af{amf} exposes a block interface that does not allow overwriting unless an explicit erase is issued for the blocks. This matches the flash requirement that prior to overwriting data it has to be erased. The interface is implemented as a custom \as{ftl}, called AFTL, on top of which the ALFS file system is built. This avoids the duplicate garbage collection of the \as{ftl} and the file system, as the garbage collection of the ALFS erases blocks during garbage collection, informing the \as{ftl} to erase the physical block.

Co-designing the FTL and the file system allows removing uncoordinated duplicate work, and coordinate the flash management. To this end, Lee et al.~\cite{lee2014refactored} present a redesigned \as{io} architecture, called REDO, which avoids the duplicate operations from file system and \as{ftl} by implemented the new framework directly as the storage controller, and building the \af{rfs} on top of the new controller interface. By combining the file system operations with the storage controller, the file system is responsible for running \as{gc} and managing the storage by maintaining the \as{l2p} mappings.



==> io_amplification.tex <==
\section{\as{io} Amplification}\label{sec:io_amplification}
Several of the applied mechanisms for dealing with asymmetric flash performance and garbage collection are key mechanisms to eliminate \as{io} amplification. \cref{tab:io_amplification} shows the different mechanisms that can be applied to lower the various types of \as{io} amplification, including \af{wa}, \af{ra}, and \af{sa}. These include the benefit of write buffering, which in the case of write requests that are smaller than the flash allocation unit, avoids the unnecessary \as{wa} to fill the flash allocation unit. Similar buffering as is employed in \as{wods}, such as the $\text{B}^\varepsilon$-trees, allows decreasing the \as{wa}. Another key mechanism is reducing the generated write traffic, which minimizes \as{wa}, \as{ra}, and \as{sa} through deduplication, compression, delta-encoding, and virtualization. Similarly, the discussed methods of grouping data, avoiding fragmentation, allows reducing the \as{ra} to locate data, and furthermore limits \as{gc} overheads and \as{gc} caused \as{wa}. Throughout this section we evaluate the additional methods for limiting the various types of \as{io} amplification.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{30mm}|p{18mm}|p{23mm}||}
        \hline 
        Mechanism & Amplification Type & File Systems \\
        \hline
        Write \newline Optimized Data Structures (\cref{sec:wods}) & \as{wa} & \cite{2020-Tu-URFS,hunter2008brief,rodeh2013btrfs,2022-Jiao-BetrFS,dubeyko2019ssdfs} \\
        \hline
        Write Buffering (\cref{sec:write_buffering}) & \as{wa} & \cite{park2006cflru,jo2006fab,park2013enffis,2018-Kannan-DevFS,josephson2011direct,2019-Lu-Sync_IO_OCSSD,2010-Josephson-DFS,2011-Park-Multi_NAND} \\
        \hline
        Reducing Write Traffic (\cref{sec:reduce_write_traffic}) & \as{wa}, \as{ra}, \as{sa} & \cite{huang2013improve,2011-Lim-DeFFS,woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,ning2011design,2009-Zuck-NANDFS,2022-Lee-F2FS_Address_Remapping} \\
        \hline
        Data Grouping (\cref{sec:data_grouping}) & \as{wa}, \as{ra} & \cite{2006-Lim-NAND_fs,2022-Zhang-ELOFS,2020-Zhang-LOFFS,2015-Changman-f2fs,2018-Rho-Fstream} \\
        \hline
        \as{gc} Policies (\cref{sec:gc_policy}) & \as{wa}, \as{ra} & \cite{2012-Min-SFS,2018-Yoo-OrcFS,2021-Gwak-SCJ,2015-Park-Suspend_Aware_cleaning-F2FS} \\
        \hline
        Space Optimized Data Structure (\cref{sec:space_optimized_ds}) & SA & \cite{2014-Lu-ReconFS,2015-Changman-f2fs,2021-Liao-Max} \\
        \hline
        \as{wa} with Coarse Granularity Flash Mappings (\cref{sec:coarse_gran}) & \as{wa} & \cite{2018-Yoo-OrcFS,kim2006mnfs,2018-Yoo-OrcFS,lee2007log} \\
        \hline
        Reverse Indexing (\cref{sec:reverse_indexing}) & \as{wa} & \cite{2014-Lu-ReconFS}\\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Mechanisms for file systems to deal with \as{io} amplification caused by flash storage integration, and the respective file systems that implement a particular mechanism.}
    \label{tab:io_amplification}
\end{table}

\subsection{Space Optimized Data Structures}\label{sec:space_optimized_ds}
Similar to the design of a \as{wods}, data structures with particular focus on optimally utilizing available space are a mechanism to deal with \as{sa}. A commonly applied method for file systems to optimize space utilization is to possibly embed file data in the \as{inode}. Commonly the allocation of the file system \as{inode} occupies at least a block, such as 4KiB in F2FS, which however is more space than file metadata requires. Therefore, several bytes (~3.4KB in F2FS) are free, which are used to inline file data in the inode. This particularly allows for small files to entirely fit into the \as{inode}, avoiding to write the \as{inode} and leave the unused space empty, and additionally write an additional data block, which also has free space. Different to inline data, ReconFS~\cite{2014-Lu-ReconFS} uses an \as{inode} with a size of 128B, allowing to place numerous inodes in a single flash page. With such an \as{inode} size, writing each \as{inode} change directly requires to fill the flash page with unnecessary data. Therefore, ReconFS implements a \textit{metadata persistent log}, in which metadata changes are logged and compacted to align with pages, and are only written back to the storage when evicted or checkpointed, in order for the file system to remain consistent.

Similar to effective tree-based \as{wods}, the radix tree is a space optimized tree variant, that is commonly used as the directory and inode tree for file systems~\cite{2015-Changman-f2fs,2021-Liao-Max}. The directory tree is commonly constructed and maintained in memory and written to the persistent flash storage. Its space optimization revolves around merging of nodes that have a single child with that child node. This eliminates the need for an individual node that is assigned to each child, lowering the space requirement. As a result, the radix tree is also referred to as a compressed tree, due to the compression of single child nodes.

\subsection{Coarse Granularity Flash Mappings}\label{sec:coarse_gran}
A similar goal of file systems is to reduce the amount of memory that is required for the mapping table to maintain the \as{l2p} mappings. A common solution is to increase the granularity of the mapping table (e.g., block-level mapping instead of page-level mapping), requiring fewer mappings. MNFS~\cite{kim2006mnfs} manages flash storage with page-level and block-level mapping, depending on the update frequency. Metadata is updated more frequently and therefore utilizes a page-level mapping compared to larger mapping granularity for data. OrcFS~\cite{2018-Yoo-OrcFS} similarly utilizes a page-level for metadata, and a superblock-level mapping for data, which represents several flash blocks. The allocation unit is called a superblock as it consists of multiple blocks (not to be confused with the file system superblock). Furthermore, logical addresses are mapped to the same physical addresses in the data partition, requiring no mapping table, and file system sections are aligned to the superblock unit. Therefore, OrcFS only requires a block allocation information for each file in the superblock, which are stored in the inode block in the metadata area. 

However, this comes at the cost of having a larger allocation unit, and if a host write is smaller than the allocation unit it causes \as{wa}, due to the partial flash page write when the flash page size and the allocation unit are not aligned~\cite{2018-Yoo-OrcFS,lee2007log}. OrcFS~\cite{2018-Yoo-OrcFS,lee2007log} implements \textit{block patching} to solve this issue. It takes write requests that are smaller than the flash page size and pads the remaining space with dummy data to align the write request to flash page size. This mechanism avoids copying data if a flash page is partially written, and the next \as{lba} in the same flash page is written, which triggers a copy of all \as{lba}s in the flash page followed by writing the \as{lba} for the new write. For instance, for a flash page containing 4 \as{lba}s, if \as{lba}s 1-3 are written by one request, the first 3 \as{lba}s are mapped to the data and the fourth holds dummy data, such that the page is fully filled. If a second request to \as{lba} 4 is issued, it cannot fill the flash page as it has already been written. Therefore, to write the newly written data after the already written \as{lba}s, it must copy \as{lba}s 1-3, append the new write to \as{lba} 4, and write the 4 \as{lba}s to a new flash page. Adding of dummy data to fill pages reduces the \as{wa}, which would be caused by copying of all data in the flash page, as it now avoids copying the added dummy data on consecutive writes. While reduction in \as{wa} are presented, the adding of dummy data nonetheless adds \as{wa} to fill the flash page. However, as latter updates require less data written, and the importance of data grouping indicates, maintaining related data in the same flash page is more beneficial and possibly decreases future \as{wa}. Related data remains in the same flash page, as only the valid data in flash pages is copied on writes, as opposed to copying the entire flash page, introducing copied dummy data.

\subsection{Reverse Indexing}\label{sec:reverse_indexing}
As file system metadata is commonly maintained in a tree-based data structure, updates to metadata in the leaf nodes can propagate changes to the root node, known as the Wandering Tree Problem~\cite{bityutskiy2005jffs3}. Due to the update of leaf metadata, such that when file data is modified, the metadata points to the new location of the file data, causing new metadata to be written, which in turn requires its parent to be updated to point to the new location of the metadata. This propagates up to the root note, causing significant \as{wa}. F2FS utilizes a table based indexing, with the \as{nat}, such that only a table entry is required to change to update the data location, and metadata points to the table entry to locate the data. ReconFS~\cite{2014-Lu-ReconFS} utilizes an inverted indexing tree, which also avoids the wandering tree problem. With such a tree, each node points to its parent node, instead of the parent node pointing to a child node. Therefore, upon address change of a child node, the parent does not need to be modified, since the child node points upwards to the parent node. Similar mechanisms are utilized in \as{ftl} design~\cite{2013-Lu-Flash_Lifetime_Reduce_With_WA}, where indexing data is written in the \as{oob} space of the flash page from the data, in order to locate its metadata. In order to avoid increased scan times on failure recovery, which can no longer traverse the tree from the root, the updated pages are tracked to locate the most recently updated valid page, which is then periodically included in the checkpointing to ensure consistency. 


==> io_sched.tex <==
\section{\as{io} Scheduling}\label{sec:io_sched}
Given that flash storage has the capabilities to achieve single digit $\mu$-second latency, whereas overheads in the software stack, such as context switching in the Kernel caused by system calls, can already require $\mu$-seconds to complete~\cite{soares2010flexsc}, making software the dominating factor in overheads~\cite{2010-Caulfield-Moneta,2012-Caulfield-Fast_User_Space_Access,foong2010towards,seppanen2010high,vasudevan2012using}. In addition, \textit{interrupts} cause significant overheads for systems. Aimed at slow storage devices, the \as{io} request is submitted to the device, the context is switched, such that the process can continue with other work, and upon completion of the \as{io}, the host is interrupted, and the context is switched again. Any added interrupt on the \as{io} path can cause significant delays~\cite{2014-Shin-OS_IO_Path}. Cache effects are another drawback of context switching, since other work is continued, replacing data in the caches, it requires bringing the replaced data back into the caches after the interrupt and resuming of the prior context. Similarly, it also causes \af{tlb} pollution on the host system. A different approach to submitting \as{io} requests is with \textit{polling}, which eliminates the need for context switches. With polling, the \as{io} request is submitted and instead of continuing other work, the process regularly checks the \as{io} for completion. Using polling for \as{io} requests has been shown to be a favored method of building application for fast storage devices~\cite{kourtis2019reaping,yang2012poll,didona2022understanding}.

Modern systems largely rely on \textit{asynchronous \as{io}} over \textit{synchronous \as{io}}. With synchronous \as{io}, a process submits a single \as{io} request and waits for its completion. In order to saturate the storage device performance, additional threads are required, which submit \as{io} requests to the numerous \as{io} queues in the of the storage device. However, this mechanism does not scale efficiently, where each thread must wait until the \as{io} request is completed. Therefore, with asynchronous \as{io} the threads do not wait for completion, but instead submit a larger number of \as{io} requests each, allowing to fill the device \as{io} queues more effectively. The \as{io} requests for which a thread as submitted a request, but have not completed, are referred to as \textit{outstanding} or \textit{in-flight} \as{io} requests. \cref{tab:io_sched} shows the mechanisms for host systems to better leverage the flash storage performance and minimize overheads. In addition to file systems implementing particular mechanisms, we discuss more general methods applicable to all applications for benefiting from flash storage and enhancing performance.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        \as{io} Operations (\cref{sec:io_ops}) & \cite{2020-Tu-URFS} \\
        \hline
        \as{io} Scheduler (\cref{sec:io_scheduler}) & \cite{2021-Qin-Atomic_Writes} \\
        \hline
        \as{io} Path - User-Space File Systems & \cite{2020-Tu-URFS,2019-Yoshimura-EvFS,2018-Kannan-DevFS,2019-Liu-fs_as_process} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{\as{io} scheduling mechanisms to exploit performance capabilities of flash storage, and the respective file systems that implement a particular mechanism.}
    \label{tab:io_sched}
\end{table}

\subsection{\as{io} Operations}\label{sec:io_ops}
Given that particular \as{io} patterns can have degrading affects on the \as{ssd} performance, such as mixing read and write operations, as they share resources on the device, including the mapping table and \as{ecc} engine, and furthermore possibly invalidating the cached data in the \as{ssd} \as{ram}. Similarly, mixing \as{io} operations with different block sizes can result in increased fragmentation~\cite{2020-Tu-URFS}. As the Linux Kernel relies on a submission and completion queue for \as{io}, user-space frameworks such as \as{spdk} and NVMeDirect provide more flexibility for user-space file systems to design different queues, depending on the requirements. URFS~\cite{2020-Tu-URFS} utilizes this possibility to create adaptive queues that can better optimize \as{io} submissions to the device. Based on the workload characteristics URFS dynamically creates flexible \as{io} queues (e.g., group by size, read/write operation) to increase \as{ssd} performance. Similarly, Borge et al.~\cite{2019-Borge-SSD_read_variability} show with a case study on HDFS performance with \as{ssd}, that in order to leverage the capabilities of flash \as{ssd}, direct \as{io}, and increased parallel requests with buffered \as{io} are needed. 

\subsection{\as{io} Scheduler}\label{sec:io_scheduler}
With the possibility for asynchronous \as{io} to merge and reorder requests, the Linux Kernel implements several schedulers, such as \textit{NOOP}, \textit{deadline}, and \textit{CFQ}~\cite{sun2014exploring,pratt2004workload,moallem2008study,heger2010linux}. NOOP being the least intrusive scheduler only merges \as{io} request, but does not reorder them, which is beneficial on devices such as \as{ocssd}, that require consecutive LBAs. Son et al.~\cite{2015-Son-Optimizing_FS} showcase the benefits of merging random write requests, regardless of contiguity of the LBAs, in order to better enhance performance with fast storage devices. The deadline scheduler adds to NOOP by utilizing merging and reordering, however also applies a deadline for each \as{io} request to ensure requests are submitted to the device eventually. Two separate queues, one for read requests and an additional one for write requests are utilized, which are both ordered by the deadline of the request. Another scheduler variant of deadline exists, called \textit{mq-deadline}, which is aimed at multi-queue devices, such as \as{nvme} \as{ssd}. \af{cfq} implements a round-robin based queue that assigns time slices to each in order to prevent starvation and provide fairness. While these are the common schedulers in the Linux Kernel, to see details on all schedulers present in the Linux Kernel consult~\cite{2019-ubuntu_wiki_io_schedulers}. Such scheduling configuration begs the question on which scheduler is best suited for file systems on flash storage. Several studies into performance of the schedulers exist~\cite{sun2014exploring,yu2014optimizing}, showcasing that merging of read \as{io} requests in synchronous \as{io} provides beneficial performance gains, and similarly the merging of write \as{io}s in asynchronous \as{io} shows performance gains.

Qin et al.~\cite{2021-Qin-Atomic_Writes} argue that \as{io} ordering limits exploiting the parallelism of flash devices. Especially as the Linux block layer does not guarantee particular ordering, flags such as \af{fua}, indicating that \as{io} completion is signaled upon arrival of data on the storage, and \textit{PREFLUSH}, which before completing the request flushes the volatile caches, have to be set in order to ensure a specific ordering~\cite{2021-Qin-Atomic_Writes}. With file systems, the \as{io} of metadata and data has a particular ordering, such that metadata can only point to data that exists, needing to ensure that data is written prior to metadata. Removing of \as{io} ordering allows eliminating this need and better utilize the flash parallelism. Utilizing the \as{oob} area on flash pages, the file system developed by Qin et al., called NBFS, maintains versioning in order to identify out of order updates. Furthermore, updates are done using atomic writes (discussed in Section~\ref{sec:failure_consistency}). The issuing of \as{fua} requests further implies that its \as{io}s cannot be merged in the scheduler~\cite{2021-Qin-Atomic_Writes}, implying that if a smaller than flash page size \as{fua} \as{io} request is issued, it is padded to the page size, causing \as{wa}. NBFS solves this with its atomic writes that imply that the \as{fua} request does not immediately have to be written to the flash, but instead wait for all data blocks to arrive, which are then used to fill the pages, allowing to reduce the \as{wa} (solving \textbf{\as{fic}3}).

\subsection{\as{io} Path - User-Space File Systems}\label{sec:user_space_fs}
A mechanism that is gaining significant attention in the research community is the utilization of user-space file systems, bypassing the Kernel layers and avoid its associated overheads. These file systems run only in the user-space, as opposed to commonly used file systems (e.g., F2FS) running in Kernel space. In addition to the benefit of avoiding Kernel overheads, user-space file systems are easier to develop, have increased reliability and security by avoiding Kernel bugs and vulnerabilities, and provide increased portability~\cite{2015-Tarasov-User_space_fs_practicality}. A widely adopted framework for building user-space storage applications is \af{fuse}~\cite{szeredi2010fuse}. It is implemented over a Kernel module with which it exports a virtual file system from the Kernel, where data and metadata are provided by a user-space process, hence allowing user-space applications to interact with it. Since \as{fuse} is implemented with a Kernel module, \as{fuse} based file systems suffer significant performance penalties, requiring more \as{cpu} cycles than file systems in Kernel space. Particularly contributing to overheads is the need to copy memory between user-space and kernel-space, caused by the way \as{fuse} handles \as{io} requests~\cite{2019-Vangoor-Fuse_performance,vangoor2017fuse}. Furthermore, \as{fuse} still suffers from context switching~\cite{vangoor2017fuse,2019-Vangoor-Fuse_performance,rajgarhia2010performance} overheads and \af{ipc} between the \as{fuse} kernel module and \as{fuse} user-space daemon~\cite{zhu2018direct}. 

A similar framework for building user-space applications with direct storage access is \as{nvme}Direct~\cite{2016-Kim-NVMe_Direct}. However, it also relies on a Kernel driver to provide enhanced \as{io} policies. \as{spdk}~\cite{2017-Yang-SPDK} is another framework for building user-space storage applications, however it provides the mechanisms to bypass the Kernel and submit \as{io} directly to the device, by implementing a user-space driver for the storage device. Such a framework allows building high performance storage applications in user-space, which eliminate the overheads coming from the Kernel \as{io} stack. 

URFS~\cite{2020-Tu-URFS} provides increased concurrency performance by implementing a multi-process shared cache in memory, in order to avoid the Kernel overheads of copying data as is present in \as{fuse}. It furthermore helps avoid contention on the storage device. Eliminating of data copy is also addressed in ZUFS (zero-copy user-mode file system)~\cite{2019-Harrosh-zufs}, which is a
user-space file system for persistent memory, which completes \as{io} requests by requesting exact data locations instead of copying data into the own address space. A similar user-space file system that implements a shared cache for process is EvFS~\cite{2019-Yoshimura-EvFS}, which is \as{spdk}-based. While this file system can also support multiple readers/writers in the page cache, it only supports these for a single user process. User-space frameworks often provide capabilities to either expose the storage device as a block device, which the user-space application then accesses, or build a custom block device module (e.g., with \as{spdk}, which also has default driver modules such as \as{nvme}). For \as{nvme} devices that support \as{nvme} controller memory buffer management, the file system can manage parts of the device memory. DevFS~\cite{2018-Kannan-DevFS} utilize such an integration to manage the device memory for file metadata and \as{io} queues.

Different from prior discussed development frameworks, \af{fsp}~\cite{2019-Liu-fs_as_process} provides a storage architecture design for user-space file systems. The emphasis of \as{fsp} is to scale with the arrival of faster storage, and similarly to other user-space frameworks, minimize the software stack. For this it bases development on running file systems as processes, providing safer metadata integrity, data sharing coordination, and consistency control, as the process running the file system is in control of everything, instead of trusting libraries. Furthermore, \as{fsp} relies on \as{ipc} for fast communication, which unlike FUSE has a low overhead since it does not require context switching. Inter-core message passing comes at a low overhead and cache-to-cache transfers on multi-core systems can complete in double-digit cycles~\cite{soares2010flexsc}. DashFS~\cite{2019-Liu-fs_as_process} is built with \as{fsp}, providing a safe user-space file system with isolation of different user processes, and efficient \as{ipc}.


==> methodology.tex <==
\section{Literate Study Research Methodology}\label{sec:lit_methodology}
Several methodologies for conducting literature studies exist such as an unguided traversal of the
literature~\cite{2018-Hegeman-Survey_Graph_Analysis} and using
\textit{snowballing}~\cite{Webster2002AnalyzingTP,2014-Wohlin-Snowballing}. However, we find that said methods lack
systematic mechanisms in their evaluation, where the search space of relevant literature with unguided is not clearly
defined and can become incomprehensibly large. Snowballing on the other hand allows limiting the search space by
evaluation going forward, studies that reference the seed paper, and backwards, studies that the seed paper references,
in the citations from a set of seed papers systematically. However, it can introduce possible bias from the seed paper
selection. Therefore, we utilize a combination of approaches and additionally apply the \af{slr} presented by Kitchenham
et al.~\cite{kitchenham2007guidelines}. The \as{slr} approach relies on three separate stages to construct a systematic
literature review, depicted in \cref{tab:SLR_process}. As we do not inclusively apply every possible stage of the
\as{slr} method, the table additionally depicts which methods we apply in this study (indicated with a \cmark), and
where relevant information can be found in this survey.

\begin{table}[t]
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \centering
    \begin{tabular}{c c c}
        \hline
        & \textbf{Planning the review} & \\
        \hline
        \cmark & Identification of the need for a review & (\cref{sec:introduction}) \\
        \xmark & Commissioning a review & - \\
        \cmark & Specifying the research question(s) & (\cref{sec:introduction}) \\
        \cmark & Developing a review protocol & (\cref{sec:review_protocol}) \\
        \xmark & Evaluating the review protocol & - \\
        \hline \hline
        & \textbf{Conducting the review} & \\
        \hline
        \cmark & Identification of research & (\cref{sec:search_space_selection}) \\
        \cmark & Selection of primary studies & (\cref{sec:study_selection}) \\
        \xmark & Study quality assessment & - \\
        \cmark & Data extraction and monitoring & (\cref{sec:study_analysis}) \\
        \cmark & Data synthesis & (\cref{sec:study_analysis}) \\
        \hline \hline
        & \textbf{Reporting the review} & \\
        \hline
        \xmark & Specifying dissemination mechanism & - \\
        \cmark & Formatting the main report & - \\
        \xmark & Evaluating the report & - \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \caption{Outline of the Systematic Literature Review approach presented by Kitchenham et al.~\cite{kitchenham2007guidelines}, inspired by the structure of the literature study on Graph Analysis by Hegeman and Iosup~\cite{2018-Hegeman-Survey_Graph_Analysis}.}
    \label{tab:SLR_process}
\end{table}

With these three stages, clear protocol and process definitions are established prior to conducting the review, limiting
possible reviewer bias and additionally enhancing reproducibility. The initial stage consists of planning the review,
which includes establishing the need for this certain review and developing the review protocol. The protocol
encompasses the inclusion and exclusion criteria, as well as research question definition, and the establishment of the
review process. Based on an established protocol we conduct the review, establish the selection of studies to evaluate,
and proceed to extract and analyze the studies. Lastly, with all collected data on selected studies, we format this
literature study to present the review in a comprehensible manner.

\subsection{Review Protocol}\label{sec:review_protocol}
By making use of the \as{slr} process, we initially define a review protocol and review processes that we detail for this study. With emphasis on making this study reproducible, we provide detailed descriptions of each phase in the review process. A visual representation of the application of the review protocol phases is depicted in \cref{fig:review_protocol}. It revolves around three phases, firstly establishing the search space from which we extract relevant studies for this literature study. In the second phase we collect the studies and apply the defined selection criteria (explained in \cref{sec:study_selection}). Lastly, we analyze the collected relevant studies. The following sections explain each of the phases in detail, \cref{sec:search_space_selection} explains methods used for establishing the search space of literature. Next, \cref{sec:study_selection} depicts the selection criteria for extracting relevant studies from the defined search space. Lastly, \cref{sec:study_analysis} provides the methods of data extraction from studies and gives the organization of studies for this literature review.

\input{figs/review_protocol.tex}

\subsection{Search Space Selection}\label{sec:search_space_selection}
The first stage of our review protocol defines the definition of the search space from which relevant studies are extracted. We make use of several approaches for identifying relevant studies. Firstly, we apply the snowballing method on a set of seed papers. Seed papers selected for this literature review are depicted in \cref{tab:seed_papers}. With these seed papers, we analyze the studies from forward and backward citations of the seed paper. To further expand the search space of relevant studies, we examine the publications of numerous conferences, workshops, and journals which are focused on the area of systems and storage research. These conferences are analyzed in the range of 2010-2022, if present, as some are bi-annual or may not have been established in the given time range. The following venues are checked in this literature review: 

\begin{itemize}
    \item USENIX Annual Technical Conference (\textit{USENIX ATC})
    \item USENIX Conference on File and Storage Technologies (\textit{FAST})
    \item Networked Systems Design \& Implementation (\textit{NSDI})
    \item European Conference on Computer Systems (\textit{EuroSys})
    \item USENIX Symposium on Operating Systems Design and Implementation (\textit{OSDI})
    \item Symposium on Operating Systems Principles (\textit{SOSP})
    \item ACM International Systems and Storage Conference (\textit{SYSTOR})
    \item ACM Workshop on Hot Topics in Storage and File Systems (\textit{HotStorage})
    \item Architectural Support for Programming Languages and Operating Systems (\textit{ASPLOS})
    \item ACM Special Interest Group on Management of Data (\textit{SIGMOD})
    \item International Conference on Very Large Data Bases (\textit{VLDB})
    \item IEEE International System-on-Chip Conference (\textit{SOCC})
    \item International Conference on Distributed Computing Systems (\textit{ICDCS})
    \item ACM/IFIP Middleware Conference (\textit{Middleware})
    \item ACM Transactions on Storage (\textit{TOS})
    \item International Conference for High Performance Computing, Networking, Storage, and Analysis (\textit{SC})
    \item International Conference on Massive Storage Systems and Technology (\textit{MSST})
    \item IEEE International Conference on Computer Design (\textit{ICCD})
\end{itemize}

\begin{table}[!t]
    \centering
    \begin{tabular}{||c c c||}
        \hline
        Title & Venue & Publication Year \\
        \hline
        \hline
        F2FS~\cite{2015-Changman-f2fs} & FAST & 2016 \\
        JFFS~\cite{woodhouse2001jffs} & OLS & 2001 \\
        LogFS~\cite{engel2005logfs} & Linux Kongress & 2005 \\
        \hline
    \end{tabular}
    \caption{Seed papers used for this literature review. Titles are shortened.}
    \label{tab:seed_papers}
\end{table}

Lastly, we run individual queries on academic search engines for scholarly literature; Google Scholar, Semantic Scholar, and dblp. We utilize two types of queries; \af{rsq} for finding of relevant studies for this literature study, and \af{rlsq} for finding related work to this literature review. Related work encompasses surveys on file systems for flash, flash specific algorithms and data structures, and additional studies of flash related application and system integration. For each query, with each search engine, we analyze the 100 most relevant results (or less if there are fewer query results). The keyword queries for finding relevant studies and relevant related literature studies are, respectively:

\begin{itemize}[align=left,leftmargin=1.3cm]
    \item[\textbf{RSQ1.}] Flash File System
    \item[\textbf{RSQ2.}] NVM File System
    \item[\textbf{RSQ3.}] SSD File System
    \item[\textbf{RSQ4.}] File System \as{spdk}~\footnote{\af{spdk}~\cite{2017-Yang-SPDK} provides a number of tools and libraries for building high performant user-level storage software over NVMe, making it applicable to file system development on flash SSDs.}
\end{itemize}
\begin{itemize}[align=left,leftmargin=1.3cm]
    \item[\textbf{RLSQ1.}] Flash File System Survey
    \item[\textbf{RLSQ2.}] NVM File System Survey
    \item[\textbf{RLSQ3.}] SSD File System Survey
\end{itemize}

\noindent Finding of related surveys is not limited to the established queries, but additionally during the snowballing and synthesis of conference, workshop, and journal publications we identify related work based on the prior defined classifications. Inclusion of relevant studies outside of the time range from 2010-2022 is only applicable when the study is retrieved using snowballing from seed papers, or the study is present in one of the respective query results. The timing constraint is thus only applied to the extraction of relevant studies by analyzing publications at conferences, workshops, and journals.

\subsection{Study Selection Criteria}\label{sec:study_selection}
The second phase of the review protocol defines the study selection, which extracts the relevant studies from the defined search space with a set of established criteria. We define a specific Inclusion/Exclusion criteria, with which studies are selected for this literature review based on the appropriateness for the criteria. These criteria are based on the defined research questions and are aimed to narrow down the search space to a particular set of studies of interest in this review, and enforce only relevant work is included. While studies do not have to exclusively meet all the inclusion requirements to be included in this review, any if any of the exclusion criteria is present, the study is not included in this review.

\begin{itemize}
    \item[\textbf{I1.}] The work is novel.
    \item[\textbf{I2.}] The work designs a file system specifically for NAND flash storage.
    \item[\textbf{I3.}] The work adapts an existing file system to integrate with NAND flash storage.
    \item[\textbf{E1.}] The work designs or adapts a file system not specifically for NAND flash storage.
    \item[\textbf{E2.}] The work designs or adapts a hybrid/tiered file system that utilizes various storage technologies, not focusing file system design to NAND flash storage.
    \item[\textbf{E3.}] The work designs or adapts a file system which is evaluated on NAND flash storage, but not particularly built for NAND flash storage.
    \item[\textbf{E4.}] The work designs or adapts a file system for \as{ssd}, but not specifically for NAND flash storage.
\end{itemize}

While meeting inclusion requirements does not mean a study is guaranteed to be included, it is more likely to be included. In the case of exclusion criteria, exceptions are made in cases of using papers to establish background knowledge or building context, however they are not the core focus of the respective section where its content is discussed.

Furthermore, there has been a plethora of flash-based file systems which utilize hybrid/tiered storage devices, including NOR-based flash~\cite{2008-Chul-Hybrid_NOR_NAND_FS}, \af{scm}~\cite{2013-Sheng-NVMFS,2008-Youngwoo-PFFS,2010-Jaemin-Frash,2016-Mazumder-WSN_FS,2014-Li-PCM_NAND_Fusion}, byte addressable \gls{nvm}~\cite{2019-Lee-Parallel_LFS}, and methods that expose byte addressable NVRAM on SSDs with custom firmware for metadata placement~\cite{2021-Zhou-Remap_SSD,2017-Jin-Byte_Adressable_SSD}. As several of these technologies are byte addressable, they shift integration and file system design focus away from flash storage. Additionally, combining of multiple storage technologies, such as \as{ssd} and \as{hdd}, commonly utilize \as{ssd} as a cache for the file system on the \as{hdd}, similarly shifting focus away from flash storage integration for the file system. For this reason we exclude such file system designs from the core study of this literature review. Similarly, file systems that are not designed specifically for flash storage, but have flash-friendly characteristics are also excluded. This mainly includes log-structured file systems that are intended for HDD, with a focus on writing sequentially to minimize arm movement on the disk, which coincidentally matches the sequential write requirement of flash.

\subsection{Study Analysis}\label{sec:study_analysis}
The last stage of the review protocol defines the extraction of data from the relevant studies, and establishing the final report. During evaluation of the different studies selected for this literature review, we disseminate the information presented based on their answering of the defined research questions. For this, we define the various key integration challenges of flash storage integration (\cref{sec:flash_challenges}), based on the hardware and software characteristics of flash storage. Using the defined integration challenges, we divide the contributions of the studies evaluated in this literature study into the respective challenge, and discuss its mechanisms for solving the particular flash integration challenge. These challenges are evaluated in \cref{sec:ssd_rw_asym,sec:gc,sec:io_amplification,sec:flash_parallelism,sec:wear_leveling,sec:io_sched,sec:failure_consistency}. Lastly, we discuss on the findings of the main findings from this literature study, followed by the relevant related literature studies for flash storage in \cref{sec:related_work}.

\subsection{Limitations}
Albeit this literature study being extensively defined and established through clear protocol definitions, there are several limitations that remain. Firstly, the search space selection is only based on studies that have scientific literature. Therefore, file systems for flash which may be in the mainline Linux Kernel, are not guaranteed to be included in this survey, if no scientific literature on it exists. Secondly, the search space is limited to only scientific literature written in English. This additionally limits the inclusion of conferences, workshops, and journals to venues with proceedings in English. Lastly, as the resulting queries on the selected literature search engines produces several hundred thousand results, and we select to evaluate the first 100 results, we rely on the sorting of results based on relevance that each search engine provides. While we utilize multiple search engines in an effort to avoid bias from each search engine, it does not completely eliminate it.



==> related.tex <==
\section{Related Work}\label{sec:related_work}
With the growing adoption of flash based storage systems~\cite{daim2008forecasting,2008-Lee-Flash_in_enterprise_db}, there has been a plethora of proposed systems to optimize for flash characteristics. We focus on the existing file systems for flash storage, but other aspects such as key-value stores are another popular use case for flash storage.

\noindent \textbf{Flash Optimized File Systems.} Egger~\cite{egger2010file} provide a survey on the file systems for flash storage at the time (2010), comparing the file systems in key features important for flash storage. This includes the feature set of the file system, time complexity of operations such as mount time, and space requirements for memory. However, evaluated file systems are not limited to flash specific file systems. While the survey presents an insightful summary of flash file systems, it was published in 2010, thus limiting the number of available file systems significantly. Similarly, Gal and Toledo~\cite{gal2005algorithms} present a survey of algorithms and data structures for flash storage, which encompasses flash mappings and flash-specific file systems.

Jaffer~\cite{jafferevolution} provide a comparison of five file systems for flash storage, analyzing the feature set of each and discussing limitations. In particular, the author focuses on the evolution of design trends for flash storage over the past decades, where the earliest file system included in the comparison was presented in 1994. The author additionally includes a discussion on file system optimizations for data management with Streams~\cite{kang2014multi} and \as{ocssd}~\cite{picoli2020open,bjorling2017lightnvm}. While the author presents an insightful analysis into design trends for flash storage, the literature review is limited to only the five discussed file systems and does not differentiate in the file system application domain.

Dubeyko~\cite{dubeyko2019ssdfs} presents SSDFS, a file system designed for SSDs. Albeit not being a literature review of flash file systems, the author presents an extensive comparison of related work that proposes flash file systems. Including a discussion on flash-friendly and flash-oriented file systems, and summarizing the available methods for optimizing flash specific operations and storage management. While the discussion of flash file systems provides a comparison of flash file systems, it is similarly not differentiating between application domain of the file system. Munegowda et al.~\cite{munegowda2014evaluation} showcase a study into several file systems on Windows and Linux for SSD and flash devices. Furthermore, the authors present a comparison of features for the varying file systems, including flash support and FTL integration, as well as a high level performance comparison. However, the study is focused on the main adopted file systems, lacking the inclusion of less adopted flash file systems.

Ramasamy and Karantharaj~\cite{2014-Ramasamy-Flash_FS_Challenges} survey the challenges of building file systems for flash storage, including the performance implications, caching techniques, and implications of the FTL. The authors additionally discuss available solutions to the presented design challenges for storage systems on flash memory. Similarly, Di Carlo et al.~\cite{2011-DiCarlo-Design_Issues_FS_Flash} present a study into the design issues and challenges of flash memory file systems. The authors analyze the inherent implications of the flash storage from the type of cell type used and required wear leveling, error correction, and bad block management. A comparison of several available flash file systems at the time of publication (2011) is presented, with focus on the discussed design challenges.

\noindent \textbf{Flash Optimized Applications.} Not focusing of file systems for flash storage, there have been several surveys into flash characteristics. Luo and Carey~\cite{2018-Luo-LSM_Survey} present a survey into log-structured merge-tree (LSM-tree) design techniques for storage systems. With LSM-trees being a widely adopted and popular choice of database and key-value store design to optimize for flash storage, the presented survey showcases relevant flash storage optimizations for data management. Similarly, Doekemeijer and Trivedi~\cite{2022-Doekemeijer-KV_Flash_Survey} present a study into key-value stores optimized for flash storage, showcasing several techniques that can likewise be applied to file system design for flash storage.

\noindent \textbf{Flash Translation Layer.} Chung et al.~\cite{chung2009FTL_survey} provide a survey into the various FTL algorithms, discussing the design issues of various algorithms. Flash file system performance will largely depend on the FTL implementation for SSDs, making optimal FTL design an important aspect of optimizing file system performance. A similar survey on FTL algorithms is presented by Kwon et al.~\cite{kwon2011ftl}. As embedded devices and possible custom integrations require management of flash at the file system level, the concepts for efficient and performant FTL algorithms are applicable to file system level management of flash storage.


==> rw_asym.tex <==
\section{Asymmetric Read and Write Performance}\label{sec:ssd_rw_asym}
Given that read and write performance on flash storage is asymmetric~\cite{stoica2009evaluating,2022-intel-p,chen2009understanding}, this section provides the various mechanisms to handle the asymmetric performance. \cref{tab:rw_asym} shows the various methods for dealing with asymmetric performance, and how to increase file system performance. A particularly important mechanism for improving lower write performance of flash is to utilize write-optimized data structures, such as log-based data structures, where write operations are always written to the end of the log. Further mechanisms for improving write performance involve efficient methods of data caching, and effective organization of data on the storage device.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        Write Optimized Data Structures (\cref{sec:wods}) & \cite{2020-Tu-URFS,hunter2008brief,rodeh2013btrfs,2022-Jiao-BetrFS,dubeyko2019ssdfs} \\
        \hline
        Write Buffering (\cref{sec:write_buffering}) & \cite{park2006cflru,jo2006fab,park2013enffis,2018-Kannan-DevFS,josephson2011direct,2019-Lu-Sync_IO_OCSSD,2010-Josephson-DFS,2011-Park-Multi_NAND} \\
        \hline
        Deduplication (\cref{sec:deduplication}) & \cite{huang2013improve,dubeyko2019ssdfs,2011-Lim-DeFFS} \\
        \hline
        Compression (\cref{sec:compression}) & \cite{woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,ning2011design} \\
        \hline
        Delta-Encoding (\cref{sec:delta_encoding}) & \cite{huang2013improve,dubeyko2019ssdfs} \\
        \hline
        Virtualization (\cref{sec:virtualization}) & \cite{2009-Zuck-NANDFS,2022-Lee-F2FS_Address_Remapping} \\
        \hline
        Flash Dual Mode Switching (\cref{sec:flash_dual_mode}) & \cite{2020-Wu-DualFS,2009-Sungjin-FlexFS} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Mechanisms for file systems to deal with \textbf{\as{fic}1}, asymmetric read and write performance of flash storage, and the respective file systems that implement a particular mechanism.}
    \label{tab:rw_asym}
\end{table}

\subsection{Write Optimized Data Structures}\label{sec:wods}
The characteristic of flash having lower write than read performance requires that data structures for flash are write optimized. Such data structures which are optimized for write operations are referred to as \af{wods}~\cite{bender2015introduction}. With the addition of the missing support for in-place updates on flash, the best suiting data structure for flash-based file systems is a log-based structure. As a result, all file systems discussed in this section are \as{lfs}. The nature of a \as{lfs} being append only writes accounts for the lower write performance on flash, which matches the write updates to the operations more optimal for flash, which are smaller fine-fine grained updates~\cite{2013-Lu-Flash_Lifetime_Reduce_With_WA} in a log structured fashion~\cite{2015-Changman-f2fs}. 

However, while the log provides increased write performance, metadata is scattered throughout the log, requiring a full scan of the log to locate metadata. Therefore, file systems commonly employ tree-based data structures for metadata, decreasing the worst case time complexity from $\mathcal{O}(n)$ to $\mathcal{O}(\log{}n)$. B-tree is a commonly used data structure for storage systems, including databases~\cite{comer1979ubiquitous,graefe2011modern} and file systems~\cite{rodeh2013btrfs}. Nodes in a B-tree can be larger than in conventional binary search trees, allowing the node to align to a unit of the underlying storage. B-trees furthermore are maximizing the breadth of the tree, instead of its height, in order to minimize the \as{io} requests in order to locate data, since each traversal to a child node requires an \as{io} request. The tree itself is sorted and self-balancing, making the worst case complexity for search relative to the tree height, however also requiring to balance the tree. The B+tree further reduce required \as{io} by only having data in the leaf nodes, such that higher nodes only contain keys, increasing the number of keys that fit inside a block. Leaf nodes are linked in a linked list, for faster node traversal, which in turn speeds up searching. 

In order to write optimize these trees, $\text{B}^\varepsilon$-trees~\cite{bender2015introduction,brodal2003lower} adapt the node structure of the B-tree to include a buffer to which updates to its children nodes are written. As node updates are initially written in memory, this allows to gather a larger number of small writes, encode these in the added buffer of the respective nodes, and write these as a larger unit, avoiding frequent small updates to nodes. The most recent version of BetrFS~\cite{2022-Jiao-BetrFS} (published in 2022) implements such a $\text{B}^\varepsilon$ as the metadata storage for indexing data. It is implemented in the Linux Kernel as a key-value store, based on TokuDB~\cite{tokudb}, which exposes a key-value addressable interface. The benefit of this $\text{B}^\varepsilon$-tree is that the nodes have a larger (2-4MiB) sequentially written log, batching updates into larger units and thus avoiding small updates. Initially all updates go into the root node message log, which when full gets flushed to its child nodes. While \as{wods} provide optimized write performance by batching updates, read requests require reading an entire node (2-4MiB), causing small read requests to suffer from significant read amplification.

SSDFS~\cite{dubeyko2019ssdfs} adapts the tree design to utilize hybrid nodes, since the node allocation uses blocks, which are several KB in size, and may not directly be filled directly. Therefore, hybrid nodes in the tree adapt the size of the node, such that if a hybrid node is allocated and filled, it allocates an additional hybrid node, which upon being filled is merged with the first hybrid node and becomes a leaf node. This allows to reduce write amplification (solving \textbf{\as{fic}3}) if a node is not filled enough. An additional optimization to B-trees is the \af{piobt}~\cite{2011-Roh-Bp_tree_optimizations}, which implements a parallel flash-optimized B-Tree variant (solving \textbf{\as{fic}4}), utilizing a larger \as{io} granularity to exploit package-level parallelism, maintain a high number of outstanding \as{io} requests to utilize the channel-level parallelism, and avoid mixed read and write operations.

\subsection{Write Buffering}\label{sec:write_buffering}
In addition to \as{wods} optimizing write operations file systems need to also avoid small writes, referred to as \textit{microwrites}. Particularly, as file systems write in units of blocks, which commonly are 4KiB, small writes require a full unit to be filled. The majority of file systems provide the possibility for inline data in inodes, such that the inode data, which is written regardless, has a small capacity to include data. However, this still requires that for small files inodes are directly written to flash. Therefore, several schemes that involve buffering and caching of data in memory, before flushing to the flash storage, provide increased write performance, and additionally increase overall performance.

While buffering of \as{io} prior to flushing to flash storage provides performance gains, buffers are often limited in size and are much smaller than the persistent storage. Furthermore, in addition to buffering write requests for new data, accessing or updating existing data is also cached in the buffer. Therefore, the caches utilize effective methods that minimize the cache misses by optimizing the eviction policy. \af{lru}~\cite{tanenbaum2016structured-LRU} is a common caching policy that maintains the items in the cache in the order of usage, where the least recently used item is selected for eviction. This mechanism is extended by DFS~\cite{2010-Josephson-DFS,josephson2011direct}, which utilizes \textit{lazy \as{lru}}, which does not insert accessed data into the buffer upon a cache miss, but rather inserts the data into the buffer only on an additional cache. Requiring of two cache misses implies that the cache only contains data that is frequently accessed, instead of caching all data from a cache miss.

\af{cflru}~\cite{park2006cflru} is another extension on the \as{lru} algorithm, which splits the buffer into two segments, one as the working region in which recently accessed pages reside, which are managed in \af{mru} fashion, therefore depicting the frequently accessed pages. The second region, called the clean-first region contains the less commonly accessed pages in \as{lru} fashion. On eviction (e.g., when writing a new page and freeing space in the buffer), it first attempts to evict a clean page, rather than a dirty page from the clean-first region, as this does not require a flush of the dirty data to the flash storage, and only resorts to evicting dirty pages as last resort. \af{fab}~\cite{jo2006fab} optimizes the caching policy to align with the flash characteristics by organizing pages in the cache in a larger unit, called \textit{block}, and upon eviction flushes entire blocks to the flash storage, issuing larger \as{io}s and aligning better to the flash erase unit. 

Similarly, NAFS~\cite{2011-Park-Multi_NAND} implements a \textit{double list cache}, containing a clean list with only clean pages for caching of data, and a second dirty list for writing of modified pages and to prefetch of pages based on the access patters, only containing dirty pages. The benefit of two separate lists is that firstly it allows caching write operations and avoid small writes to the flash device, and secondly it prefetches data into the clean list in order to minimize cache misses. EnFFiS~\cite{park2013enffis} presents the \textit{dirty-last cache} policy, which considers the flash characteristics by utilizing a \textit{delay region} and a \textit{replacement region}, which correspond to a multiple of the flash memory blocks. By using a multiple of the flash blocks, the data written is sequentialized and written to the flash as a larger unit, where dirty pages are initially moved from the replacement region to the delay region, before being flushed to the flash. This buffering in the delay region allows collecting more dirty pages, improving performance and avoiding smaller writes to flash. 

StageFS~\cite{2019-Lu-Sync_IO_OCSSD} likewise utilizes two stages, where write operations are initially written into the first stage, called the \textit{file system staging area}. The issued writes to the staging area are completed in a \textit{persistence-efficient} way, which utilizes a log to account for asymmetric flash performance for the staging area. Subsequently, writes are then regrouped, based on the file system structure and hot/cold identification, and are written to the second stage, based on the group assignment. The staging area allows writing synchronous \as{io} directly to the staging log with optimal flash write characteristics, lowering completion latency, followed by better grouping of data when writing from the staging to the second stage file system area.

In an effort to limit the required memory for data caching, DevFS~\cite{2018-Kannan-DevFS} proposes the \textit{reverse caching} mechanism for effectively managing host memory and device memory. Reverse caching aims at keeping only active files in the device memory, which is limited in size, and upon closing of a file migrates the metadata to the host memory. Reopening a file migrates it back to the device memory, and consistency of metadata is not violated as any actively modified metadata is in the device memory, and only inactive metadata is in the host memory. To efficiently utilize reverse caching, DevFS uses a host-memory cache that is able to use \af{dma} to move metadata between itself and the device memory, additionally minimizing host overheads.

\subsection{Reducing Write Traffic}\label{sec:reduce_write_traffic}
In order to avoid the slower write performance of flash storage another mechanisms aims at minimizing the amount of data that is written to the storage device. Whenever data is updated on the flash storage, updating all metadata and writing the new data incurs a significant amount of write traffic, in addition to causing \as{wa}. Therefore, reducing the amount of data being written through mechanisms such as deduplication, compression, and delta-encoding helps at avoiding the increased \as{wa}.

\subsubsection{Deduplication}\label{sec:deduplication}
File systems commonly contain duplicate data, from backups or archival copies made and general work. Therefore, file systems often aim to avoid creating duplicates of existing data, which is referred to as \textit{deduplication}. Evaluations show that in high-performance computing centers on average about 20-30\%, with peaks of 70\%, of the stored data can be removed through deduplication~\cite{meister2012study}. Deduplication avoids writing the same data multiple times, which in turn helps reduce the write traffic and minimizes write and space amplification (solving \textbf{\as{fic}2}). Effective deduplication relies on hash functions, which provide a deterministic output, called the \textit{digest} or commonly referred to as the \textit{fingerprint} of the data, based on which duplicates can be identified. The utilized hash functions for deduplication are \textit{one way hash functions}~\cite{merkle1989one}, which calculate a fingerprint of the data, or digest, but given the digest or fingerprint, the data cannot be generated. Given data from a file for instance, hashing the data provides a digest, and if the same data is to be written again, the same digest is generated. By identifying if a digest already exists in the file system, can it identify if the data is being duplicated, and avoid writing the duplicate by making the metadata of the newly written data point to the existing data. 

In order to apply deduplication on file system data, two methods exits. \textbf{(1)} Deduplication with fixed-sized chunks, where hashes are generated based on the entire file or a pre-determined chunk size, and \textbf{(2)} variable-sized chunks where the chunk size that is hashed depends on the file and content. The effectiveness of deduplication with fixed-sized chunks is limited and highly dependent on the chunk size and modification sequences in the chunks~\cite{2011-Lim-DeFFS}, as for example a small change in a large file, where the chunk size is the entire file, results in a completely different hash, even if much of the data is duplicated. While variable-sized chunks reduces the configuration dependability it is significantly more complex to implement. DeFFS~\cite{2011-Lim-DeFFS} implements a duplicate elimination algorithm that reduces the complexity of identifying duplicates. As comparing duplicates of every byte is not possible, the algorithm finds the smallest modified region in a file adapting the chunk size, which is initially assigned the default value that corresponds to the flash page size.

The idea of eliminating duplication through fingerprints is not new for \as{ssd}, as existing \as{ftl} implementations implement such mechanism. \af{caftl}~\cite{chen2011caftl} generates collision-free fingerprints of write requests and maintains fingerprints of all flash resident data in order to avoid writing the same data twice. Flash Saver~\cite{li2012flash} is a similar architecture running between the SSD and the file system, which manages the file system \as{io} requests and ensures deduplication using SHA-1 fingerprints~\cite{wang2005finding}. A plethora of similar hash-based deduplication mechanisms exist~\cite{fu2011aa,ha2013deduplication,kim2012deduplication,xia2014combining}, which may not be particular to file systems, but can be adopted by a wide range of storage systems. File systems with deduplication are CSA-FS~\cite{huang2013improve}, which implements deduplication by calculating the MD5 digest~\cite{rivest1992md5} (MD5 is a hash function applied to the input) and looks up the result in a hash table which provides the corresponding LBA of the block. If it already exists and the user requested a new file with it, the new inode simply uses the given LBA from the hash table, instead of duplicating the data again. Similarly, SSDFS~\cite{dubeyko2019ssdfs} maintains fingerprints with its metadata B-Tree, and DeFFS~\cite{2011-Lim-DeFFS} stores hash keys with all inodes for their data to avoid duplicates. 

\subsubsection{Compression}\label{sec:compression}
An effective method for reducing the required storage space for data is to utilize \textit{compression}. While there exist lossy compression algorithms~\cite{iverson2012fast,kavitha2016survey}, which discard parts of the data, and lossless compression algorithms~\cite{kavitha2016survey,sharma2010compression}, which maintain all data, lossy compression is very application dependent, and in the case of file systems we assume a lossless data storage and therefore focus on lossless compression algorithms. Lossless compression methods rely on three methods. \textbf{(1)} \af{rle} which minimizes size by taking the repeating characters, referred to as the run, and replacing them with a 2 byte sequence of the number of repetitions of the character, called the run count, followed by the replaced character. For example the sequence of ``aaabbccc`` is represented as ``a3b2c3`` with \as{rle}. \textbf{(2)} \af{lz}~\cite{ziv1977universal,ziv1978compression} which utilizes a dictionary to replace strings with their dictionary value. Variations of the \as{lz} algorithm exist, such as LZ77~\cite{ziv1977universal}, LZ78~\cite{ziv1978compression}, and LZW~\cite{welch1984technique}. The dictionary is constructed at the compression time and used a decompression time~\cite{kapoor2013review}. A well-known compression algorithm GZIP~\cite{deutsch1996gzip} is based on two \as{lz} algorithms. \textbf{(3)} Huffman Coding~\cite{huffman1952method} which creates a full binary tree based the frequency of occurring characters and generating code of the character and the frequency. 

JFFS~\cite{woodhouse2001jffs} and several other file systems~\cite{woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,goyal2005energy,cramfs,ning2011design} provide a data compression, however metadata compression has shown to cause decompression overheads~\cite{kang2022pr}. Applying compression at the file system level allows reducing the utilized storage space, especially on flash this reduces the space and write amplification factors (solving \textbf{\as{fic}3}), and in turn prolonging the flash lifetime as shown by Li et al.~\cite{2015-Li-SSD_lifetime_compression} on the benefits of different compression algorithms for NAND flash lifetime. SSDFS~\cite{dubeyko2019ssdfs} utilizes LZO compression~\cite{oberhumer2008lzo}, a library for data compression with LZ algorithms, for data and metadata. Given that different data benefits from different compression mechanisms, where for instance data is less frequently read can be compressed more efficiently than frequently read data, which may require more simplistic decompression to minimize overheads, or embed metadata in the compressed data to avoid decrypting data and metadata separately. Adaptive compression selection is employed in an extension of F2FS~\cite{2021-Ji-F2FS_compression}, where \af{fpc} selects the compression method for files based on how compressible they are.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/pba_decompression.pdf}
    \caption{The benefit of \af{pbal} during decompression arises from the elimination of copying associated file data.}
    \label{fig:pba_decompression}
\end{figure}

An issue of compression is that it must be aligned to the flash unit, in order to avoid unnecessary read amplification and required data copying. \cref{fig:pba_decompression} shows that if the compressed data is not aligned to the flash unit of a page, such that compressed data can span across pages, the decompression process becomes more complex. This is due to first having to read all the associated flash pages into the device memory. However, if compressed data can span across flash pages, this implies that non-associated data can be included. Therefore, only the associated data must be copied to a \textit{decompression buffer} (step 2a), from which the data can be decompressed (step 3). LeCramFS~\cite{2007-Hyun-LeCramFS} (short for less crammed FS) implements a read-only file system with compression for embedded devices, that avoids this additional copy of data by using \as{pbal}. Any compressed data will not span across page boundaries, implying that no additional pages with non-associated data are read, and the data can be decompressed directly (step 2). Therefore, it avoids the additional copy of data and reduces the read amplification (solving \textbf{\as{fic}}3). In order to avoid wasting space if the page is not fully utilized from a single compression, LeCramFS extends the compression implementation with a \textit{partial compression}, which splits the data into parts that fit into the available space. These parts are then compressed separately, allowing to utilize all available space.

\subsubsection{Delta-Encoding}\label{sec:delta_encoding}
Similar to deduplication, delta-encoding lowers the write traffic, further limiting the space and write amplification (solving \textbf{\as{fic}2}) by instead of writing out entire data when updated, with delta-encoding the new data is compared to the old data and only the differences, called the \textit{delta}, are written. This is especially beneficial in the case of small changes in large files, where it avoids writing the entire file again and writes only the changes in the data. While delta-encoding provides a similar space reduction to compression, particular file characteristics of what is being encoded can affect resulting performance. For instance, data sets that have a significant redundancy across them, such as email data sets, require significantly less space than being compressed~\cite{douglis2003application}. However, non-textual data, such as pdf documents, will have large deltas for even small changes, where compression is likely to be a better choice. Therefore, the application of delta-encoding depends on the data characteristics and what type of content is being encoded, in order to achieve better utilization of delta-encoding compared to simpler compression. CSA-FS~\cite{huang2013improve} implements delta encoding on its file system metadata (superblock, descriptor, bitmaps, and tables), allowing minor updates such as the access time of metadata and bitmaps to only write the new changes. Similarly, SSDFS~\cite{dubeyko2019ssdfs} uses delta-encoding for user data.

\subsubsection{Virtualization}\label{sec:virtualization}
As Butler Lampson mentioned in his famous quote from 1972 (which was originally stated by David Wheeler), ``Any problem in computer science can be solved with another level of indirection``~\cite{lampson1993principles}. By adding an additional layer on flash storage the write traffic can be reduced as a result of avoiding metadata update propagation (as with the wandering tree problem~\cite{bityutskiy2005jffs3}). Adding a virtual layer is conceptually identical to \af{lba} on top of \as{pba}. \cref{fig:virtualization} shows an example of how virtualization maintains the same \af{vba} when file data is updated, eliminating a need for metadata updates. Note, for simplicity we assume the virtual layer to be on top of the physical layer, providing \as{pba}s, however it can be directly on the physical layer of the flash storage, depending on the flash integration level, and would therefore be using \af{l2p} mappings. In the illustrated scenario, three blocks are mapped to \as{pba}0, \as{pba}1, and \as{pba}2, respectively. Assuming these are part of a file, metadata points to these respective virtual block addresses. If the first block of the file is modified, a new data block is written at \as{pba}3. With virtualization, the \as{vba} remains unchanged, only the \as{v2p} mapping table is modified to depict the new mapping of \as{pba}3. As a result, file metadata remains unchanged, avoiding write amplification for updating file metadata. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/virtualization.pdf}
    \caption{A simplified example scenario of virtualization on top of the physical storage.}
    \label{fig:virtualization}
\end{figure}

A similar mechanism is implemented in NANDFS~\cite{2009-Zuck-NANDFS}, using a \textit{sequencing layer} that implements the block allocation as immutable storage on the logical layer. Therefore, when file system data is updated, it cannot overwrite and simply marks the data as obsolete, and the new updated data is written in a newly allocated block. The sequencing layer implements the \as{l2p} mapping,  such that the \as{lba} of the new data is the same as the old \as{lba}, avoiding the updating of data addresses in the file system metadata. This implies that the file system does less writing by eliminating metadata updates, which in turn also reduces the required \as{gc}.

The concept of virtualization can similarly be applied through \af{ar}. With \as{ar} only the \as{l2p} mapping table of the storage device is modified, which similar to virtualization avoids rewriting of metadata. \as{ar} is an effective mechanism for solving additional overheads in file systems, such as file system garbage collection~\cite{kang2018address}, journaling~\cite{choi2009jftl,kang2018address,weiss2015anvil}, and data duplication~\cite{2021-Zhou-Remap_SSD}. Lee et al~\cite{2022-Lee-F2FS_Address_Remapping} propose \af{rmipu}, an address remapping scheme implemented in F2FS to solve issues of out-of-place updates. Instead of applying \as{ar} into a single file system operation, \as{rmipu} includes all write operations to utilize \as{ar}. All updated data is first stored in the log, followed by \as{ar} to update data pointers, thus avoiding metadata updates for file overwrite operations. File write operations to new files are appended to the log as usual, and the contiguity in \as{lba}s for files is maintained.

\subsection{Flash Dual Mode Switching}\label{sec:flash_dual_mode}
Some modern flash devices allow the host to switch the cell level of underlying flash blocks (e.g., switching \as{mlc} to \as{slc})~\cite{2020-Wu-DualFS,li2019accelerating}. This provides the benefit that a lower cell level, representing fewer bits, has a lower read, write, and erase latency, thus providing the flash with a higher performance than with a larger cell level configuration~\cite{2020-Wu-DualFS}. This switching between flash modes is referred to as \textit{flash dual mode}, which however comes at the cost of being able to store less data in the same amount of flash, as the block is only able to store half the data in the example of switching from \as{mlc} to \as{slc}. DualFS~\cite{2020-Wu-DualFS} utilizes the flash dual mode feature to provide a dynamically sized \as{slc} area, alongside the remaining \as{mlc} area, to accelerate the performance of critical \as{io} requests. By evaluating the \as{io} queue depth of \as{io} requests, DualFS determines the criticality of the incoming request, and maps it to the \as{slc} area for increased performance. It further profiles incoming request based on the hotness and allocates hot data into the \as{slc} mode for lower request latency.

FlexFS\cite{2009-Sungjin-FlexFS} implements a similar mechanism for increased performance on the \as{slc} area. The drawback of such a design is that data is required to be moved from the \as{slc} area to the \as{mlc} area as it has a lower write lifetime, and is aimed at the for critical \as{io} requests that require lower completion latency, which in turn causes \textit{data migration overheads}. To solve this, FlexFS implements several migration techniques that aim to hide the overheads for the data migration from the host. The first technique revolves around \textit{background migration}, which pushes the migration to happen when the system is idle. The second technique is \textit{dynamic allocation}, which writes non-critical requests to the \as{mlc} area, saving on flash degradation in the \as{slc} area, as well as avoiding future data migration. The dynamic allocator functions based on measurements of prior system idle times from \as{io} requests, to predict current idle time, and if sufficient idle time is predicted in order to complete data migration, the data is written to the \as{slc}, and otherwise part of the data, depending on required migration and idle time, is written to the \as{mlc} area. The last technique, \textit{locality-aware data management}, takes into account the hotness of data, and the dynamic allocator attempts to migrate only cold data from the \as{slc} area.


==> sections/rqs.tex <==
\section{Research Questions}\label{sec:lit_study_rqs}
In order to evaluate the various work on flash storage implications for file system design, we devise three key \af{srq} that aim at analyzing past, current, and future trends.

\begin{itemize}
    \item [\textbf{SRQ1.}] \textbf{What are the main challenges arising from NAND flash characteristics and its integration into file system design?} \\
        Flash storage has particular characteristics, such as sequential writing, no in-place updates, and requiring erasing of flash blocks. This \as{srq} aims at analyzing what particular challenges arise for storage software from the flash-specific constraints and resulting effects of on-device operations. Devising a list of key challenges provides the foundation based on which relevant work in this literature study is selected, and the final report is structured.
    \item[\textbf{SRQ2.}] \textbf{How has NAND flash storage influenced the design and development of file system and the storage software stack?} \\
        Using the identified challenges in \textbf{\as{srq}1}, this \as{srq} evaluates for each of the challenges, how file system design has changed to integrate with it. As file systems are commonly built on top of existing storage software layers, such as the Linux Block \as{io} layer, we include methods and mechanisms in the storage software stack particularly devised for file systems and flash storage integration. As a result, this \as{srq} evaluates how the depicted challenges are addressed throughout the various software stack layers, up to the file system.
    \item [\textbf{SRQ3.}] \textbf{How will NAND flash storage and newly introduced NAND flash-based storage devices and interfaces affect future file system design and development?} \\
        With a particular goal of this literature study being to evaluate the validity of data structures, algorithms, and mechanisms of flash, and understanding the applicability to \as{zns}, a newly arising storage technology, this research question furthermore aims at evaluating future challenges that may arise from new technology.
\end{itemize}


==> wear_leveling.tex <==
\section{Asymmetric Read and Write Performance}\label{sec:ssd_rw_asym}
Given that read and write performance on flash storage is asymmetric~\cite{stoica2009evaluating,2022-intel-p,chen2009understanding}, this section provides the various mechanisms to handle the asymmetric performance. \cref{tab:rw_asym} shows the various methods for dealing with asymmetric performance, and how to increase file system performance. A particularly important mechanism for improving lower write performance of flash is to utilize write-optimized data structures, such as log-based data structures, where write operations are always written to the end of the log. Further mechanisms for improving write performance involve efficient methods of data caching, and effective organization of data on the storage device.

\begin{table}[!t]
    \centering
    % Update reference format to fit table into column
    \crefformat{section}{\S#2#1#3}
    \crefformat{subsection}{\S#2#1#3}
    \crefformat{subsubsection}{\S#2#1#3}
    \begin{tabular}{||p{40mm}|p{35mm}||}
        \hline 
        Mechanism & File Systems \\
        \hline
        \hline
        Write Optimized Data Structures (\cref{sec:wods}) & \cite{2020-Tu-URFS,hunter2008brief,rodeh2013btrfs,2022-Jiao-BetrFS,dubeyko2019ssdfs} \\
        \hline
        Write Buffering (\cref{sec:write_buffering}) & \cite{park2006cflru,jo2006fab,park2013enffis,2018-Kannan-DevFS,josephson2011direct,2019-Lu-Sync_IO_OCSSD,2010-Josephson-DFS,2011-Park-Multi_NAND} \\
        \hline
        Deduplication (\cref{sec:deduplication}) & \cite{huang2013improve,dubeyko2019ssdfs,2011-Lim-DeFFS} \\
        \hline
        Compression (\cref{sec:compression}) & \cite{woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,ning2011design} \\
        \hline
        Delta-Encoding (\cref{sec:delta_encoding}) & \cite{huang2013improve,dubeyko2019ssdfs} \\
        \hline
        Virtualization (\cref{sec:virtualization}) & \cite{2009-Zuck-NANDFS,2022-Lee-F2FS_Address_Remapping} \\
        \hline
        Flash Dual Mode Switching (\cref{sec:flash_dual_mode}) & \cite{2020-Wu-DualFS,2009-Sungjin-FlexFS} \\
        \hline
    \end{tabular}
    % Reset reference format to before
    \crefformat{section}{Section #2#1#3}
    \crefformat{subsection}{Section #2#1#3}
    \crefformat{subsubsection}{Section #2#1#3}
    \caption{Mechanisms for file systems to deal with \textbf{\as{fic}1}, asymmetric read and write performance of flash storage, and the respective file systems that implement a particular mechanism.}
    \label{tab:rw_asym}
\end{table}

\subsection{Write Optimized Data Structures}\label{sec:wods}
The characteristic of flash having lower write than read performance requires that data structures for flash are write optimized. Such data structures which are optimized for write operations are referred to as \af{wods}~\cite{bender2015introduction}. With the addition of the missing support for in-place updates on flash, the best suiting data structure for flash-based file systems is a log-based structure. As a result, all file systems discussed in this section are \as{lfs}. The nature of a \as{lfs} being append only writes accounts for the lower write performance on flash, which matches the write updates to the operations more optimal for flash, which are smaller fine-fine grained updates~\cite{2013-Lu-Flash_Lifetime_Reduce_With_WA} in a log structured fashion~\cite{2015-Changman-f2fs}. 

However, while the log provides increased write performance, metadata is scattered throughout the log, requiring a full scan of the log to locate metadata. Therefore, file systems commonly employ tree-based data structures for metadata, decreasing the worst case time complexity from $\mathcal{O}(n)$ to $\mathcal{O}(\log{}n)$. B-tree is a commonly used data structure for storage systems, including databases~\cite{comer1979ubiquitous,graefe2011modern} and file systems~\cite{rodeh2013btrfs}. Nodes in a B-tree can be larger than in conventional binary search trees, allowing the node to align to a unit of the underlying storage. B-trees furthermore are maximizing the breadth of the tree, instead of its height, in order to minimize the \as{io} requests in order to locate data, since each traversal to a child node requires an \as{io} request. The tree itself is sorted and self-balancing, making the worst case complexity for search relative to the tree height, however also requiring to balance the tree. The B+tree further reduce required \as{io} by only having data in the leaf nodes, such that higher nodes only contain keys, increasing the number of keys that fit inside a block. Leaf nodes are linked in a linked list, for faster node traversal, which in turn speeds up searching. 

In order to write optimize these trees, $\text{B}^\varepsilon$-trees~\cite{bender2015introduction,brodal2003lower} adapt the node structure of the B-tree to include a buffer to which updates to its children nodes are written. As node updates are initially written in memory, this allows to gather a larger number of small writes, encode these in the added buffer of the respective nodes, and write these as a larger unit, avoiding frequent small updates to nodes. The most recent version of BetrFS~\cite{2022-Jiao-BetrFS} (published in 2022) implements such a $\text{B}^\varepsilon$ as the metadata storage for indexing data. It is implemented in the Linux Kernel as a key-value store, based on TokuDB~\cite{tokudb}, which exposes a key-value addressable interface. The benefit of this $\text{B}^\varepsilon$-tree is that the nodes have a larger (2-4MiB) sequentially written log, batching updates into larger units and thus avoiding small updates. Initially all updates go into the root node message log, which when full gets flushed to its child nodes. While \as{wods} provide optimized write performance by batching updates, read requests require reading an entire node (2-4MiB), causing small read requests to suffer from significant read amplification.

SSDFS~\cite{dubeyko2019ssdfs} adapts the tree design to utilize hybrid nodes, since the node allocation uses blocks, which are several KB in size, and may not directly be filled directly. Therefore, hybrid nodes in the tree adapt the size of the node, such that if a hybrid node is allocated and filled, it allocates an additional hybrid node, which upon being filled is merged with the first hybrid node and becomes a leaf node. This allows to reduce write amplification (solving \textbf{\as{fic}3}) if a node is not filled enough. An additional optimization to B-trees is the \af{piobt}~\cite{2011-Roh-Bp_tree_optimizations}, which implements a parallel flash-optimized B-Tree variant (solving \textbf{\as{fic}4}), utilizing a larger \as{io} granularity to exploit package-level parallelism, maintain a high number of outstanding \as{io} requests to utilize the channel-level parallelism, and avoid mixed read and write operations.

\subsection{Write Buffering}\label{sec:write_buffering}
In addition to \as{wods} optimizing write operations file systems need to also avoid small writes, referred to as \textit{microwrites}. Particularly, as file systems write in units of blocks, which commonly are 4KiB, small writes require a full unit to be filled. The majority of file systems provide the possibility for inline data in inodes, such that the inode data, which is written regardless, has a small capacity to include data. However, this still requires that for small files inodes are directly written to flash. Therefore, several schemes that involve buffering and caching of data in memory, before flushing to the flash storage, provide increased write performance, and additionally increase overall performance.

While buffering of \as{io} prior to flushing to flash storage provides performance gains, buffers are often limited in size and are much smaller than the persistent storage. Furthermore, in addition to buffering write requests for new data, accessing or updating existing data is also cached in the buffer. Therefore, the caches utilize effective methods that minimize the cache misses by optimizing the eviction policy. \af{lru}~\cite{tanenbaum2016structured-LRU} is a common caching policy that maintains the items in the cache in the order of usage, where the least recently used item is selected for eviction. This mechanism is extended by DFS~\cite{2010-Josephson-DFS,josephson2011direct}, which utilizes \textit{lazy \as{lru}}, which does not insert accessed data into the buffer upon a cache miss, but rather inserts the data into the buffer only on an additional cache. Requiring of two cache misses implies that the cache only contains data that is frequently accessed, instead of caching all data from a cache miss.

\af{cflru}~\cite{park2006cflru} is another extension on the \as{lru} algorithm, which splits the buffer into two segments, one as the working region in which recently accessed pages reside, which are managed in \af{mru} fashion, therefore depicting the frequently accessed pages. The second region, called the clean-first region contains the less commonly accessed pages in \as{lru} fashion. On eviction (e.g., when writing a new page and freeing space in the buffer), it first attempts to evict a clean page, rather than a dirty page from the clean-first region, as this does not require a flush of the dirty data to the flash storage, and only resorts to evicting dirty pages as last resort. \af{fab}~\cite{jo2006fab} optimizes the caching policy to align with the flash characteristics by organizing pages in the cache in a larger unit, called \textit{block}, and upon eviction flushes entire blocks to the flash storage, issuing larger \as{io}s and aligning better to the flash erase unit. 

Similarly, NAFS~\cite{2011-Park-Multi_NAND} implements a \textit{double list cache}, containing a clean list with only clean pages for caching of data, and a second dirty list for writing of modified pages and to prefetch of pages based on the access patters, only containing dirty pages. The benefit of two separate lists is that firstly it allows caching write operations and avoid small writes to the flash device, and secondly it prefetches data into the clean list in order to minimize cache misses. EnFFiS~\cite{park2013enffis} presents the \textit{dirty-last cache} policy, which considers the flash characteristics by utilizing a \textit{delay region} and a \textit{replacement region}, which correspond to a multiple of the flash memory blocks. By using a multiple of the flash blocks, the data written is sequentialized and written to the flash as a larger unit, where dirty pages are initially moved from the replacement region to the delay region, before being flushed to the flash. This buffering in the delay region allows collecting more dirty pages, improving performance and avoiding smaller writes to flash. 

StageFS~\cite{2019-Lu-Sync_IO_OCSSD} likewise utilizes two stages, where write operations are initially written into the first stage, called the \textit{file system staging area}. The issued writes to the staging area are completed in a \textit{persistence-efficient} way, which utilizes a log to account for asymmetric flash performance for the staging area. Subsequently, writes are then regrouped, based on the file system structure and hot/cold identification, and are written to the second stage, based on the group assignment. The staging area allows writing synchronous \as{io} directly to the staging log with optimal flash write characteristics, lowering completion latency, followed by better grouping of data when writing from the staging to the second stage file system area.

In an effort to limit the required memory for data caching, DevFS~\cite{2018-Kannan-DevFS} proposes the \textit{reverse caching} mechanism for effectively managing host memory and device memory. Reverse caching aims at keeping only active files in the device memory, which is limited in size, and upon closing of a file migrates the metadata to the host memory. Reopening a file migrates it back to the device memory, and consistency of metadata is not violated as any actively modified metadata is in the device memory, and only inactive metadata is in the host memory. To efficiently utilize reverse caching, DevFS uses a host-memory cache that is able to use \af{dma} to move metadata between itself and the device memory, additionally minimizing host overheads.

\subsection{Reducing Write Traffic}\label{sec:reduce_write_traffic}
In order to avoid the slower write performance of flash storage another mechanisms aims at minimizing the amount of data that is written to the storage device. Whenever data is updated on the flash storage, updating all metadata and writing the new data incurs a significant amount of write traffic, in addition to causing \as{wa}. Therefore, reducing the amount of data being written through mechanisms such as deduplication, compression, and delta-encoding helps at avoiding the increased \as{wa}.

\subsubsection{Deduplication}\label{sec:deduplication}
File systems commonly contain duplicate data, from backups or archival copies made and general work. Therefore, file systems often aim to avoid creating duplicates of existing data, which is referred to as \textit{deduplication}. Evaluations show that in high-performance computing centers on average about 20-30\%, with peaks of 70\%, of the stored data can be removed through deduplication~\cite{meister2012study}. Deduplication avoids writing the same data multiple times, which in turn helps reduce the write traffic and minimizes write and space amplification (solving \textbf{\as{fic}2}). Effective deduplication relies on hash functions, which provide a deterministic output, called the \textit{digest} or commonly referred to as the \textit{fingerprint} of the data, based on which duplicates can be identified. The utilized hash functions for deduplication are \textit{one way hash functions}~\cite{merkle1989one}, which calculate a fingerprint of the data, or digest, but given the digest or fingerprint, the data cannot be generated. Given data from a file for instance, hashing the data provides a digest, and if the same data is to be written again, the same digest is generated. By identifying if a digest already exists in the file system, can it identify if the data is being duplicated, and avoid writing the duplicate by making the metadata of the newly written data point to the existing data. 

In order to apply deduplication on file system data, two methods exits. \textbf{(1)} Deduplication with fixed-sized chunks, where hashes are generated based on the entire file or a pre-determined chunk size, and \textbf{(2)} variable-sized chunks where the chunk size that is hashed depends on the file and content. The effectiveness of deduplication with fixed-sized chunks is limited and highly dependent on the chunk size and modification sequences in the chunks~\cite{2011-Lim-DeFFS}, as for example a small change in a large file, where the chunk size is the entire file, results in a completely different hash, even if much of the data is duplicated. While variable-sized chunks reduces the configuration dependability it is significantly more complex to implement. DeFFS~\cite{2011-Lim-DeFFS} implements a duplicate elimination algorithm that reduces the complexity of identifying duplicates. As comparing duplicates of every byte is not possible, the algorithm finds the smallest modified region in a file adapting the chunk size, which is initially assigned the default value that corresponds to the flash page size.

The idea of eliminating duplication through fingerprints is not new for \as{ssd}, as existing \as{ftl} implementations implement such mechanism. \af{caftl}~\cite{chen2011caftl} generates collision-free fingerprints of write requests and maintains fingerprints of all flash resident data in order to avoid writing the same data twice. Flash Saver~\cite{li2012flash} is a similar architecture running between the SSD and the file system, which manages the file system \as{io} requests and ensures deduplication using SHA-1 fingerprints~\cite{wang2005finding}. A plethora of similar hash-based deduplication mechanisms exist~\cite{fu2011aa,ha2013deduplication,kim2012deduplication,xia2014combining}, which may not be particular to file systems, but can be adopted by a wide range of storage systems. File systems with deduplication are CSA-FS~\cite{huang2013improve}, which implements deduplication by calculating the MD5 digest~\cite{rivest1992md5} (MD5 is a hash function applied to the input) and looks up the result in a hash table which provides the corresponding LBA of the block. If it already exists and the user requested a new file with it, the new inode simply uses the given LBA from the hash table, instead of duplicating the data again. Similarly, SSDFS~\cite{dubeyko2019ssdfs} maintains fingerprints with its metadata B-Tree, and DeFFS~\cite{2011-Lim-DeFFS} stores hash keys with all inodes for their data to avoid duplicates. 

\subsubsection{Compression}\label{sec:compression}
An effective method for reducing the required storage space for data is to utilize \textit{compression}. While there exist lossy compression algorithms~\cite{iverson2012fast,kavitha2016survey}, which discard parts of the data, and lossless compression algorithms~\cite{kavitha2016survey,sharma2010compression}, which maintain all data, lossy compression is very application dependent, and in the case of file systems we assume a lossless data storage and therefore focus on lossless compression algorithms. Lossless compression methods rely on three methods. \textbf{(1)} \af{rle} which minimizes size by taking the repeating characters, referred to as the run, and replacing them with a 2 byte sequence of the number of repetitions of the character, called the run count, followed by the replaced character. For example the sequence of ``aaabbccc`` is represented as ``a3b2c3`` with \as{rle}. \textbf{(2)} \af{lz}~\cite{ziv1977universal,ziv1978compression} which utilizes a dictionary to replace strings with their dictionary value. Variations of the \as{lz} algorithm exist, such as LZ77~\cite{ziv1977universal}, LZ78~\cite{ziv1978compression}, and LZW~\cite{welch1984technique}. The dictionary is constructed at the compression time and used a decompression time~\cite{kapoor2013review}. A well-known compression algorithm GZIP~\cite{deutsch1996gzip} is based on two \as{lz} algorithms. \textbf{(3)} Huffman Coding~\cite{huffman1952method} which creates a full binary tree based the frequency of occurring characters and generating code of the character and the frequency. 

JFFS~\cite{woodhouse2001jffs} and several other file systems~\cite{woodhouse2001jffs,dubeyko2019ssdfs,2021-Ji-F2FS_compression,2007-Hyun-LeCramFS,goyal2005energy,cramfs,ning2011design} provide a data compression, however metadata compression has shown to cause decompression overheads~\cite{kang2022pr}. Applying compression at the file system level allows reducing the utilized storage space, especially on flash this reduces the space and write amplification factors (solving \textbf{\as{fic}3}), and in turn prolonging the flash lifetime as shown by Li et al.~\cite{2015-Li-SSD_lifetime_compression} on the benefits of different compression algorithms for NAND flash lifetime. SSDFS~\cite{dubeyko2019ssdfs} utilizes LZO compression~\cite{oberhumer2008lzo}, a library for data compression with LZ algorithms, for data and metadata. Given that different data benefits from different compression mechanisms, where for instance data is less frequently read can be compressed more efficiently than frequently read data, which may require more simplistic decompression to minimize overheads, or embed metadata in the compressed data to avoid decrypting data and metadata separately. Adaptive compression selection is employed in an extension of F2FS~\cite{2021-Ji-F2FS_compression}, where \af{fpc} selects the compression method for files based on how compressible they are.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/pba_decompression.pdf}
    \caption{The benefit of \af{pbal} during decompression arises from the elimination of copying associated file data.}
    \label{fig:pba_decompression}
\end{figure}

An issue of compression is that it must be aligned to the flash unit, in order to avoid unnecessary read amplification and required data copying. \cref{fig:pba_decompression} shows that if the compressed data is not aligned to the flash unit of a page, such that compressed data can span across pages, the decompression process becomes more complex. This is due to first having to read all the associated flash pages into the device memory. However, if compressed data can span across flash pages, this implies that non-associated data can be included. Therefore, only the associated data must be copied to a \textit{decompression buffer} (step 2a), from which the data can be decompressed (step 3). LeCramFS~\cite{2007-Hyun-LeCramFS} (short for less crammed FS) implements a read-only file system with compression for embedded devices, that avoids this additional copy of data by using \as{pbal}. Any compressed data will not span across page boundaries, implying that no additional pages with non-associated data are read, and the data can be decompressed directly (step 2). Therefore, it avoids the additional copy of data and reduces the read amplification (solving \textbf{\as{fic}}3). In order to avoid wasting space if the page is not fully utilized from a single compression, LeCramFS extends the compression implementation with a \textit{partial compression}, which splits the data into parts that fit into the available space. These parts are then compressed separately, allowing to utilize all available space.

\subsubsection{Delta-Encoding}\label{sec:delta_encoding}
Similar to deduplication, delta-encoding lowers the write traffic, further limiting the space and write amplification (solving \textbf{\as{fic}2}) by instead of writing out entire data when updated, with delta-encoding the new data is compared to the old data and only the differences, called the \textit{delta}, are written. This is especially beneficial in the case of small changes in large files, where it avoids writing the entire file again and writes only the changes in the data. While delta-encoding provides a similar space reduction to compression, particular file characteristics of what is being encoded can affect resulting performance. For instance, data sets that have a significant redundancy across them, such as email data sets, require significantly less space than being compressed~\cite{douglis2003application}. However, non-textual data, such as pdf documents, will have large deltas for even small changes, where compression is likely to be a better choice. Therefore, the application of delta-encoding depends on the data characteristics and what type of content is being encoded, in order to achieve better utilization of delta-encoding compared to simpler compression. CSA-FS~\cite{huang2013improve} implements delta encoding on its file system metadata (superblock, descriptor, bitmaps, and tables), allowing minor updates such as the access time of metadata and bitmaps to only write the new changes. Similarly, SSDFS~\cite{dubeyko2019ssdfs} uses delta-encoding for user data.

\subsubsection{Virtualization}\label{sec:virtualization}
As Butler Lampson mentioned in his famous quote from 1972 (which was originally stated by David Wheeler), ``Any problem in computer science can be solved with another level of indirection``~\cite{lampson1993principles}. By adding an additional layer on flash storage the write traffic can be reduced as a result of avoiding metadata update propagation (as with the wandering tree problem~\cite{bityutskiy2005jffs3}). Adding a virtual layer is conceptually identical to \af{lba} on top of \as{pba}. \cref{fig:virtualization} shows an example of how virtualization maintains the same \af{vba} when file data is updated, eliminating a need for metadata updates. Note, for simplicity we assume the virtual layer to be on top of the physical layer, providing \as{pba}s, however it can be directly on the physical layer of the flash storage, depending on the flash integration level, and would therefore be using \af{l2p} mappings. In the illustrated scenario, three blocks are mapped to \as{pba}0, \as{pba}1, and \as{pba}2, respectively. Assuming these are part of a file, metadata points to these respective virtual block addresses. If the first block of the file is modified, a new data block is written at \as{pba}3. With virtualization, the \as{vba} remains unchanged, only the \as{v2p} mapping table is modified to depict the new mapping of \as{pba}3. As a result, file metadata remains unchanged, avoiding write amplification for updating file metadata. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/virtualization.pdf}
    \caption{A simplified example scenario of virtualization on top of the physical storage.}
    \label{fig:virtualization}
\end{figure}

A similar mechanism is implemented in NANDFS~\cite{2009-Zuck-NANDFS}, using a \textit{sequencing layer} that implements the block allocation as immutable storage on the logical layer. Therefore, when file system data is updated, it cannot overwrite and simply marks the data as obsolete, and the new updated data is written in a newly allocated block. The sequencing layer implements the \as{l2p} mapping,  such that the \as{lba} of the new data is the same as the old \as{lba}, avoiding the updating of data addresses in the file system metadata. This implies that the file system does less writing by eliminating metadata updates, which in turn also reduces the required \as{gc}.

The concept of virtualization can similarly be applied through \af{ar}. With \as{ar} only the \as{l2p} mapping table of the storage device is modified, which similar to virtualization avoids rewriting of metadata. \as{ar} is an effective mechanism for solving additional overheads in file systems, such as file system garbage collection~\cite{kang2018address}, journaling~\cite{choi2009jftl,kang2018address,weiss2015anvil}, and data duplication~\cite{2021-Zhou-Remap_SSD}. Lee et al~\cite{2022-Lee-F2FS_Address_Remapping} propose \af{rmipu}, an address remapping scheme implemented in F2FS to solve issues of out-of-place updates. Instead of applying \as{ar} into a single file system operation, \as{rmipu} includes all write operations to utilize \as{ar}. All updated data is first stored in the log, followed by \as{ar} to update data pointers, thus avoiding metadata updates for file overwrite operations. File write operations to new files are appended to the log as usual, and the contiguity in \as{lba}s for files is maintained.

\subsection{Flash Dual Mode Switching}\label{sec:flash_dual_mode}
Some modern flash devices allow the host to switch the cell level of underlying flash blocks (e.g., switching \as{mlc} to \as{slc})~\cite{2020-Wu-DualFS,li2019accelerating}. This provides the benefit that a lower cell level, representing fewer bits, has a lower read, write, and erase latency, thus providing the flash with a higher performance than with a larger cell level configuration~\cite{2020-Wu-DualFS}. This switching between flash modes is referred to as \textit{flash dual mode}, which however comes at the cost of being able to store less data in the same amount of flash, as the block is only able to store half the data in the example of switching from \as{mlc} to \as{slc}. DualFS~\cite{2020-Wu-DualFS} utilizes the flash dual mode feature to provide a dynamically sized \as{slc} area, alongside the remaining \as{mlc} area, to accelerate the performance of critical \as{io} requests. By evaluating the \as{io} queue depth of \as{io} requests, DualFS determines the criticality of the incoming request, and maps it to the \as{slc} area for increased performance. It further profiles incoming request based on the hotness and allocates hot data into the \as{slc} mode for lower request latency.

FlexFS\cite{2009-Sungjin-FlexFS} implements a similar mechanism for increased performance on the \as{slc} area. The drawback of such a design is that data is required to be moved from the \as{slc} area to the \as{mlc} area as it has a lower write lifetime, and is aimed at the for critical \as{io} requests that require lower completion latency, which in turn causes \textit{data migration overheads}. To solve this, FlexFS implements several migration techniques that aim to hide the overheads for the data migration from the host. The first technique revolves around \textit{background migration}, which pushes the migration to happen when the system is idle. The second technique is \textit{dynamic allocation}, which writes non-critical requests to the \as{mlc} area, saving on flash degradation in the \as{slc} area, as well as avoiding future data migration. The dynamic allocator functions based on measurements of prior system idle times from \as{io} requests, to predict current idle time, and if sufficient idle time is predicted in order to complete data migration, the data is written to the \as{slc}, and otherwise part of the data, depending on required migration and idle time, is written to the \as{mlc} area. The last technique, \textit{locality-aware data management}, takes into account the hotness of data, and the dynamic allocator attempts to migrate only cold data from the \as{slc} area.

